Dialogue Benchmark Generation from Knowledge Graphs with Cost-Effective Retrieval-Augmented LLMs

Dialogue benchmarks are crucial in training and evaluating chatbots engaging in domain-specific conversations. Knowledge graphs (KGs) represent semantically rich and well-organized data spanning various domains, such as DBLP, DBpedia, and YAGO. Traditionally, dialogue benchmarks have been manually created from documents, neglecting the potential of KGs in automating this process. Some question-answering benchmarks are automatically generated using extensive preprocessing from KGs, but they do not support dialogue generation. This paper introduces Chatty-Gen, a novel multi-stage retrieval-augmented generation platform for automatically generating high-quality dialogue benchmarks tailored to a specific domain using a KG. Chatty-Gen decomposes the generation process into manageable stages and uses assertion rules for automatic validation between stages. Our approach enables control over intermediate results to prevent time-consuming restarts due to hallucinations. It also reduces reliance on costly and more powerful commercial LLMs. Chatty-Gen eliminates upfront processing of the entire KG using efficient query-based retrieval to find representative subgraphs based on the dialogue context. Our experiments with several real and large KGs demonstrate that Chatty-Gen significantly outperforms state-of-the-art systems and ensures consistent model and system performance across multiple LLMs of diverse capabilities, such as GPT-4o, Gemini 1.5, Llama 3, and Mistral.

==> algorithms/approach.tex <==
\begin{algorithm}[t]
\caption{Independent Question-SPARQL Generation Algorithm}
\label{alg:approach}
\begin{flushleft}
\textbf{Input:} $SG$: Subgraph, $n$: Number of questions, $e$: Seed Entity
\textbf{Output:} $questions$: List of independent question on subgraph facts, $queries$: Corresponding SPARQL queries
\end{flushleft}

\begin{algorithmic}[1]
\State $p_u \gets getUniquePredicates(SG)$
\State $preds\_to\_triples \gets groupTriples(SG, p_u)$
\State $SSG, queries \gets []$
\For{every $\langle p, t_{list}\rangle \in \langle preds\_to\_triples\rangle  $}
\State $t' \gets modifyTriple(e, t_{list}[0])$
\State $SSG \gets ssg \cup t'$
\EndFor
\State $questions, triples \gets generateQuestions(SSG, n)$
\For{every $\langle q, t\rangle \in \langle questions, triples\rangle  $}
        \State $qu \gets generateQuery(q, t')$
        \State $queries \gets queries \cup qu$
\EndFor
\State \textbf{Return} questions, queries
\end{algorithmic}
\end{algorithm}

==> algorithms/generate_dialogue.tex <==
\begin{algorithm}[t]
	\caption{Zero-Shot Dialogue Generation}
	\label{alg:gen_dialogue}
	\begin{flushleft}
		\textbf{Input:} $[Q_{In}]$: List of Independent Questions , $e$: seed entity \\
		\textbf{Output:} $D(e)$: Dialogue
	\end{flushleft}
	
	\begin{algorithmic}[1]
		\State $D \gets []$
		\For{every $q \in Q_{In}$}
		 \State $pr \gets getPronoun(e, q)$
		 \State $u\_q \gets updateQuestion(q, pr)$
		 \State $D \gets D \cup u\_q$
		\EndFor
		\State $\textbf{Return D}$
	\end{algorithmic}

\end{algorithm}

==> algorithms/node_type_selection.tex <==

\begin{algorithm}[t]
\vspace*{2ex}
\caption{Node Type Selection}
\label{alg:node_selection}
\begin{flushleft}
\textbf{Input:} $endpoint$: SPARQL endpoint, $m$: number of Dialogues, $domain$: prefixes of KG, $r_{threshold}$: Rare types threshold, $s_{threshold}$: Shadowed parents threshold\\
\textbf{Output:} $dist$: Map of node type to the number of entities to sample
\end{flushleft}
\begin{algorithmic}[1]
% Get types, filter, and calculate percentage
\STATE $types \gets getKGNodeTypes(endpoint, domain)$
\STATE $types \gets removeRareTypes(types, r_{threshold})$
\STATE $types \gets removeShadowedTypes(types, s_{threshold})$
\STATE $ dist \gets getTypesDistribution(types, m)$
\STATE $\textbf{Return dist}$
\end{algorithmic}
\vspace*{2ex}
\end{algorithm}



==> algorithms/seed_entity.tex <==
\begin{algorithm}[t]
\caption{Entity Sampling}
\label{alg:seed_entity}
\begin{flushleft}
\textbf{Input:} $endpoint$: SPARQL endpoint, $m$: number of Dialogues \\
\textbf{Output:} $nodes$: list of entities
\end{flushleft}

\begin{algorithmic}[1]
\State $types_{kg} \gets getKGNodeTypes(endpoint)$
\State $types_{filter} \gets filterNodeTypes(types_{kg})$
\State $types_{precent} \gets calculatePercentage(types_{filter})$
\State $rare \gets getRareTypes(types_{precent})$
\State $types \gets types_{filter} - rare$
\State $dist \gets getTypesCount(types, m)$
\State $nodes \gets getSampleNodes(dist, endpoint)$
\State $\textbf{Return nodes}$
% \State $subgraphs \gets \{\}$
% \For{every $n$ in $nodes$}
%         \State $g \gets generateSubGraph(node)$
%         \If{$isValid(n, g)$}
%             \State $ subgraphs[n] \gets g $
%         \Else
%             \State $nodes \gets nodes \cup sampleNode(endpoint)$
%     \EndIf
% \EndFor
% \State $\textbf{Return subgraphs}$
\end{algorithmic}

\end{algorithm}


==> algorithms/seed_validator.tex <==
\begin{algorithm}[t]
\caption{Entity and Subgraph Validation}
\label{alg:seed_validation}
\begin{flushleft}
\textbf{Input:} $SG$: subgraph, $e$: seed entity, $length$: LLM context length \\
\textbf{Output:} $isValid$: indicates the validity of $<e, SG>$ pair
\end{flushleft}

\begin{algorithmic}[1]
\State $l_{max}, g_{limits}, p_{min} \gets getLimits(length)$
\State $l_{length} \gets getNumTokens(e_{label})$
\State $g_{size} \gets getGraphSize(SG)$
\State $p_{unique} \gets getNumUniquePredicates(SG)$
\State $isValid \gets l_{length} < l_{max} \& g_{size} \in g_{limits} \& p_{unique} > p_{min}$
\State $\textbf{Return isValid}$
\end{algorithmic}

\end{algorithm}

==> old_sections/abstract_june10.tex <==
\begin{abstract}
Conversational AI systems have gained significant attention due to their capabilities. These systems rely on information seen during their training process. They can benefit from integration with external sources to provide up-to-date information, especially for domains not included in their training data. Knowledge graphs (KGs) containing knowledge related to diverse domains can serve as an example of external source. However, there is a lack of a systematic way to evaluate such chatbots. Therefore, we need benchmarks for different domains to evaluate the chatbots. We propose {\sysName}, a framework that leverages large language models (LLMs) and KG SPARQL endpoints to automatically generate dialogue benchmarks for arbitrary KGs. {\sysName} selects representative entities and subgraphs as the context of dialogues using the KG endpoint at run time, eliminating the need for expensive pre-processing. We also design a multi-stage LLM-based approach to generate dialogues, allowing control over intermediate results and eliminating manual effort. Evaluated with various KGs from different domains, {\sysName} successfully generated dialogues spanning different question types and representative node types in each KG. Moreover, it demonstrates efficiency in terms of time needed to generate the benchmarks.

\end{abstract}

==> old_sections/background_april12.tex <==
\section{Background}

% \subsection{Benchmarking on KG}
%\begin{definition}[Knowledge Graph]
%A knowledge graph $KG = \{V\} \cup \{E\}$ is a directed graph composed of vertices and edges:
%\begin{itemize}
%    \item Vertices $V$: Each vertex $v \in V$, represents an entity and is associated with two attributes $v_{type}$ specifies the category of the entity (e.g., person, location, language) and $v_{label}$.
%    \item Edges $E$: Each edge  $e \in E$ represents a relationship between two entities and has a label ($e_{label}$)
%\end{itemize}
%The KG can be represented as a set of triples ($T$) containing subject ($s$), predicate ($p$), and object ($o$): $T = \{<s, p, o>\}$ such that $s,o \in V$ and $p \in E$.
%\end{definition}
The benchmark creation process on top of KGs can be divided into two main steps: \myNum{i} KG exploration, \myNum{ii} Questions generation. In this section, we discuss the two closest approaches to our work: CSQA\cite{csqa} and Maestro\cite{maestro}. CSQA is a semi-automatically created benchmark, built on top of the Wikidata knowledge graph. It contains around $200k$ conversations. Maestro is an automatic benchmark generation system for question answering on knowledge graphs. It tackles the issue of variation in existing benchmarks and their limited KG coverage.


\subsection{KG Exploration}
In The knowledge exploration step, the systems select the required components from the KG to generate the questions, e.g. entities, predicates, or subgraphs.

\textbf{CSQA} gather all $330$ Wikidata predicates with their connected subject and object. They are saved as subject-predicate-object triples for further processing. This manual step needs to be performed for any new KG. 

\textbf{Maestro} divides the KG exploration into three steps: \myNum{i} predicate lexicon table creation, \myNum{ii} seed entity selection, and \myNum{iii} subgraph shape generation. In predicate lexicon table creation the predicates from the KG are extracted, along with their labels, connected node types, and KG examples containing these predicates. An optional text corpus can be employed to extract natural language sentences with candidate phrases explaining the predicate. The extracted patterns are used to create the predicate lexicon, including the predicate, connected node types, and verb/noun phrases associated with different predicate directions. Maestro can function without this corpus but yields better benchmarks with its inclusion. This step is sensitive to the presence of types in the KG, i.e. if the predicate is connecting entities that do not have \textit{rdf:type} predicate, the predicate is not considered.
In seed entity selection, Entities are chosen from the KG using a class importance and entity popularity-based approach to mitigate bias towards famous entities or specific types. These entities also serve as answers to generated questions. In subgraph shape generation, subgraphs for the seed entities are extracted based on a set of predefined shapes. The shape selection process includes preparing the SPARQL template per shape. 


\subsection{Questions Generation}
In the question generation step, the systems use the extracted KG components to generate the questions. This includes both single and conversational questions. 

In \textbf{CSQA} workers are provided with the subject-predicate-object triples and tasked with formulating questions using the predicate and subject (the object being the answer) and vice versa. The created questions are independent, i.e., do not require context to be answered. Then, a group of in-house annotators provided templates for creating the conversation. These templates consist of connected question-answer pairs. A connected question-answer pair share a relation or an entity. Finally, workers further modified questions to increase context dependence, effectively transforming the set of questions into dialogue. Although CSQA semi-automated the question generation using templates, manual work is still required in defining connected pairs, designing the templates, and transforming the question into dialogue. 

\textbf{Maestro} uses the seed entity, subgraphs, and predicate lexicon, the question generation module produces natural language questions and queries. Some questions are transformed to change their type (e.g., converting to count or boolean). Each subgraph shape is associated with a manually created natural language template. The final transformation is biased to the boolean questions, ultimately creating a big percentage of boolean questions in the benchmark. 






==> old_sections/background_april22.tex <==
\section{Background and Limitations}

The process of automatically generating conversational benchmarks for Knowledge Graphs (KGs) can be divided into seven main steps: \myNum{1} \textit{Sample Entities}: Extract a set of entities that represent the different types within the target KG. These entities will serve as the topics of the dialogues. \myNum{2} \textit{Extract Context}: Extract subgraphs surrounding the extracted entities. These subgraphs must contain enough facts to create a conversation. Similar to passages in document benchmarks, the subgraphs represent the context provided by the KG. \myNum{3} \textit{Entity Representation}: Choose a natural language representation for the entities to be used in the generated questions instead of their URIs (which identify the entities in the KG). \myNum{4} \textit{Generate Questions}: Using the context and entity representation, this step generates a set of questions asking about facts within the given subgraph. \myNum{5} \textit{Maintain Dialogue Flow}: Ensure that the generated questions are relevant and connected, if the previous step generated conversational questions. Or convert questions to dialogues if the previous step generated independent questions. \myNum{6} \textit{Generate Answer}: Extract the answer to each generated question from the KG. This answer can be an entity or a literal value. Since we are dealing with KGs, this step may involve generating SPARQL queries. \myNum{7} \textit{KG-Agnostic Design:} Design all previous steps to work with any arbitrary KG, requiring minimal to no adjustments for different knowledge graphs.

Due to the lack of existing systems specifically designed to generate conversational benchmarks for KGs, we will discuss benchmarks and systems that perform similar tasks and explain why they are not applicable to our task. \autoref{tab:back} summarizes these systems. CoQA\cite{coqa} and QuAC\cite{quac} are well-known conversational question answering benchmarks on documents. Head-to-Tail\cite{head_to_tail} is a template-based generated benchmark for single questions on KGs. CSQA\cite{csqa} is a semi-automatically generated conversational benchmark specifically designed for the Wikidata KG. Maestro\cite{maestro} is an automatic single-question benchmark generation framework for KGs.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/Framework.pdf}
\caption{An overview of the framework of automatic generation of conversational benchmark for KGs. The KG is first used to select the seed entities, and then the subgraph of each seed entity is extracted and given to the independent question generation module. The independent questions are then provided to both the query generation module and the final dialogue generation module. }
\label{fig:framework}
\end{figure*}

\textbf{CoQA} and \textbf{QuAC} are manually generated, with slight variations in settings and answer formats. Their manual creation process limits their applicability to other data sources, such as KGs. Steps 1, 3, and 7 in the explained process (sampling entities, entity representation, and KG-agnostic design) are not applicable to CoQA and QuAC. Additionally, context extraction differs in these document-focused benchmarks, as they extract passages from the source documents not subgraphs. Finally, question generation, answer retrieval, and maintaining dialogue flow are all manual steps in CoQA and QuAC.

\textbf{CSQA} takes a predicate-centric approach for benchmark generation. This eliminates the need for a separate context extraction step. CSQA begins by extracting all $330$ Wikidata predicates along with their connected subjects and objects. These are stored as subject-predicate-object triples for further processing. The process of selecting entity representations remains unclear, but given the manual nature of predicate extraction, entity representation is likely manually chosen. Question generation in CSQA is a manual process that creates independent questions. Workers are tasked with formulating questions using the provided subject-predicate-object triples. Questions can be formulated using the predicate and subject (with the object serving as the answer) or vice versa. To maintain a conversational flow, CSQA utilizes pre-designed templates. In-house annotators design these templates, which consist of connected question-answer pairs that share a relation or entity. Then, workers manually modify the generated conversations to introduce complexities such as coreferences, ellipsis, incompleteness, and contextual dependence. Similar to Head-to-Tail, CSQA does not require a separate answer generation step, as the answer is predetermined before question generation. However, supporting new KGs with CSQA is labor-intensive. Users would need to manually extract predicates, generate independent questions and answers, define connected question-answer pairs, design templates, and transform question sets into dialogues.

\textbf{Head-to-Tail} employs a popularity-based approach for entity selection in its benchmark. Entities are first sorted by popularity and then bucketed into three categories: Head, Torso, and Tail. However, during sampling, node types are not considered; nodes are randomly chosen from each bucket. For context extraction, Head-to-Tail focuses on the attributes surrounding the sampled entity. The process of entity representation selection is unclear. Question generation relies on manually created templates for each attribute surrounding the entity. This approach becomes impractical for KGs with many node types, as users would need to define a vast number of templates for various attribute-node type combinations. While Head-to-Tail does not natively support dialogues, the questions focus on entity attributes allows grouping them to simulate a conversation. But this method leads to repetitive dialogues for entities of the same type due to the use of templates. Head-to-Tail does not require a separate answer generation step, as the answer to each question is directly retrieved from the object of the triple used to create the question template. Although Head-to-Tail considers multiple KGs, supporting a new KG would necessitate manually designing a significant number of templates to encompass all attributes across all node types within that KG.

\textbf{Maestro} requires a pre-processing step before the main process. During pre-processing, Maestro extracts predicates, their labels, connected node types, and (KG) examples. This step relies on the presence of types in the KG; predicates connecting entities without the "rdf:type" predicate are not considered. The pre-processing time is proportional to the number of classes in the KG ontology. Entity selection in Maestro utilizes a combined approach of class importance and entity popularity to reduce bias towards well-known entities or specific types. However, this approach might miss important seed node types. Context extraction in Maestro involves defining various subgraph shapes around entities and creating corresponding SPARQL templates. These shapes then represent the context surrounding the entity. For entity representation, Maestro offers flexibility by allowing users to specify the predicate for extracting the appropriate representation. However, this assumes a single predicate can be used for all node types, which is not always true in KGs where different predicates represent different node types e.g. \textit{name} for \textit{Person} and \textit{title} for \textit{Publication}. Question generation in Maestro relies on rules; each shape has a corresponding natural language template for generating questions from the subgraph. However, a subsequent transformation step modifies some question types (e.g., converting them to count or boolean). This final step exhibits a bias towards boolean questions, resulting in a high percentage of such questions in the generated benchmarks. Similar to explored systems, Maestro does not require a separate answer generation step, as the answer is predetermined before question generation. Additionally, Maestro lacks dialogue generation capabilities, and grouping questions from the generated benchmark will not create a dialogue because all questions for a seed entity share the same answer (the entity itself). While Maestro is the only system among those explored that can handle multiple KGs, this support is not user-friendly. Supporting a new KG necessitates writing three classes totaling around $600$ lines of code, making it a challenge for non-technical users.








==> old_sections/context_extraction_May15.tex <==
\section{Context Extraction}
This module efficiently identifies topics for dialogue generation using three steps: \myNum{i} relevant node type selection, \myNum{ii} textual entity representation, and \myNum{iii} seed node and subgraph extraction. We rely on a node type-based approach, that eliminates the need for a time-consuming, storage-intensive pre-processing step that retrieves all entities from the KG.

% \subsection{Entity Sampling}
\subsection{Node Types and Coverage}
\label{sec:seed}
Our approach starts by selecting relevant node types from the target KG to cover the different topics within its domain. This approach is efficient and scalable for large KGs. Relying on node types avoids performing a time-consuming and space-consuming pre-processing step that extracts all the entities from the KG and requires a storage proportional to the number of entities. We focus on node types relevant to the KG's domain, excluding metadata types. Then we calculate statistics on these types to determine the distribution of node types within the given number of seed entities to be sampled.

 
Algorithm \autoref{alg:node_selection} outlines the node type selection process in detail. It takes four inputs: KG SPARQL endpoint, number of dialogues, domain prefixes that specify the relevant domains in the KG, and rare type threshold. The number of entities corresponds to the number of dialogues, as each entity serves as a dialogue topic. Therefore, the selected seed entities should cover the KG's most important topics. We use the node types to identify these topics. Line 1 retrieves the domain-specific types. It uses the provided endpoint and domain prefixes to execute a SPARQL query. This query retrieves all KG types along with their entity counts, creating a comprehensive list. The list is then sorted by descending entity count. Then, the list is filtered to exclude irrelevant metadata and non-domain-specific types. By default, We use the KG's main ontology types, reflecting its core information. Users can specify additional types or prefixes for inclusion. 

% \input{algorithms/seed_entity}
\input{algorithms/node_type_selection}

Finally, we use the entity counts of the filtered list to calculate the percentage of coverage of each type. Line 2 identifies and removes rare types. These are highly specific types whose percentage falls below the user-defined threshold. The low percentages reflect that these types are not the KG’s main focus. Line 3 identifies and removes shadowed types. These are parent types whose entities primarily belong to a single child type. Removing shadowed parents improves time efficiency by avoiding redundant processing of both the parent and child entities. Additionally, it enables more diversity in the generated dialogues by focusing on only one of the two exact topics. Due to these removals, the remaining type percentages will no longer sum to $100\%$. Therefore, we recalculate the percentages for the included types only. Finally, Line 4 leverages the adjusted percentages and the required number of entities to determine the number of entities to sample from each type. This ensures the sampled entities reflect a distribution similar to the overall KG entity distribution.



\subsubsection{Complexity}
Let $\tau$ be the number of node types returned, and $q_{cost}$ denotes the cost of executing the query to retrieve types and their counts. $q_{cost}$ varies across RDF engines since it depends on the presence of the indices and built-in functions, especially an index between node types and entity counts. Line 1's execution cost is O($q_{cost}$ + $\tau$). This is because we first execute the query ($q_{cost}$) and then iterate through the returned list ($\tau$) to filter and calculate percentages. Lines 2-4 involve iterating through the type list ($\tau$), resulting in an individual cost of O($\tau$) for each line. Consequently, the overall time complexity of Algorithm \autoref{alg:node_selection} is $O(q_{cost}+\tau)$.

\subsection{Textual Entity representation}
\label{sec:entity_rep}
The second step is retrieving a textual representation for each entity. This representation significantly impacts how humans and LLMs understand the entity and their ability to generate meaningful questions using it. KGs represent entities using URIs, which are unsuitable for natural language questions. Therefore, we need a method to convert these URIs into a textual format to use in the generated questions.
One approach is to encode the entity using the final URI segment. This method assumes the human-readability of the final segment (e.g., \url{http://dbpedia.org/resource/The_Future_of_Freedom_Conference}). However, this does not generalize. In many URIs, the final segment contains IDs (e.g., \url{https://dblp.org/pid/00/10071}) or character-number combinations (e.g., \url{https://dblp.org/rec/conf/valuetools/Coppa14}). These formats hinder LLMs' ability to understand the entity's meaning, leading to ambiguous or low-quality questions.

URIs themselves are insufficient for generating meaningful textual representations. A more effective approach involves leveraging the entity's context within the KG. Each entity is connected to various predicates, some offer good representations (e.g., "\textit{name}" for Person entities or "\textit{title}" for Publication entities). However, identifying a single predicate for diverse KGs or node types within one KG is challenging. We need a mapping between node types and appropriate predicates for the KG to retrieve the correct representation. Users with sufficient technical knowledge can provide such mapping.  While this may be feasible for smaller KGs with limited node types (tens), it becomes impractical for large KGs like DBpedia or Yago, which contain hundreds or thousands of node types.  This necessitates the development of an automatic approach for extracting node-type description predicates from the KG.

We propose an LLM-based approach for automatically extracting a description predicate $p_l$ for each node type within a KG. First, for each node type($t$), we sample a random entity ($e$) belonging to that type from the KG. Next, we extract all outgoing predicates ($P_{list}$) connected to the sampled entity ($e$). Finally, we filter the extracted predicate list ($P_{list}$) to keep only predicates connecting the entity ($e$) to string literals. This ensures the extracted representation is a string suitable for usage within questions.

\begin{equation}
    \label{eq:entity}
    p_l = f(t, P_{list}, I)
\end{equation} 

\begin{lstlisting}[language=Python, caption=Choosing representative predicate for type prompt, escapechar=@, label=label_predicate]
# Instruction:
Given the specified node type and its
associated predicates, choose a suitable
predicate to serve as a label for this type.

# Input:
node type:
predicates: 

# Response:
\end{lstlisting}

Instruction $I$ is shown in \autoref{label_predicate}. We leverage zero-shot prompting to instruct the LLM to select the most representative predicate from the filtered list ($P_{list}$). This chosen predicate serves as the label extractor for the corresponding node type ($t$). This approach generates human-readable entity representations for all node types, regardless of the information encoded in the URIs. Furthermore, it eliminates the need for user input or specific technical expertise, leading to improved question quality and overall system usability.


\subsection{Seed Nodes and Subgraph Extraction}

\begin{definition}[Subgraph $SG$]
\label{def:subgraph}
Given a $KG$ containing a set of vertices $V$ ,and a set of relations $R$. Let $e$ be the target seed entity. The subgraph $SG(e) = \{T\}$ is a set of triples, where $T = \langle s, p, o \rangle$ such that $s, o \in V$, $p \in R$, and $s= e$ or $o = e$.      
\end{definition}

\input{algorithms/entiy_subgraph_extraction}
% \input{algorithms/seed_validator}
After the node types, entity counts to sample, and corresponding label predicates are identified, we proceed to extract seed entities and their associated subgraphs. These subgraphs serve as the context for our dialogues and are used to generate multiple questions. Algorithm \autoref{alg:seed_subgraph_extraction}  details the extraction process, including the validations performed. This process is repeated for each selected node type.

We iterate through the process until the required number of entity-subgraph pairs for the current node type are extracted. In Line 3, we use a SPARQL query to extract an entity belonging to the node type ($t$). This query utilizes the label predicate ($p_l$) to retrieve the entity's label concurrently with the entity. To optimize this step and reduce query overhead, we batch-retrieve entities from the endpoint and process them individually. We only execute a new SPARQL query if the entire batch is exhausted before reaching the required number of pairs ($n$). Lines 4-6 ensure the extracted entity has a reasonable length for LLM processing. This prevents the LLM from being overwhelmed by very long labels and allows it to focus on the information connected to the entity through predicates instead of getting distracted by details within the textual label. Examples of invalid entities include publications whose labels contain publication year or location. If the label exceeds the maximum input length, we move on to the next entity. For accepted labels, lines 7-8 calculate the graph size and the number of unique predicates surrounding the seed entity within the specified number of hops ($h$). We leverage count queries that utilize the RDF engine's built-in indices for faster response times. Line 9 validates that the graph size fits within the LLM's context length limit and that the number of unique predicates is sufficient to support rich dialogue generation. Unique predicates connect entities to diverse facts, providing a strong foundation for generating multiple distinct questions.

If the values meet the LLM's requirements, we proceed to the extraction. Line 13 extracts the subgraph around the seed entity based on the specified shape, the number of hops to traverse outward from the entity, and the direction of predicates (outgoing from the entity only, or including both incoming and outgoing predicates). The subgraph includes all entities and literals connected to the seed entity within these parameters. Line 14 filters the extracted subgraph by removing some triples. First, triples containing the predicate label are excluded, as the answer to any question using it is the label itself. Additionally, triples with non-domain specific predicates and triples containing very long string literals as objects are removed to avoid confusing the LLM. Examples of filtered triples include triples of entities linked to entire abstracts. These triples are removed since they have the potential to confuse the LLMs by asking about information in the abstract rather than information in the given subgraph.
Line 15 validates the filtered subgraph, ensuring it still contains enough information (number of triples) to facilitate generating meaningful conversation. If valid, the subgraph is added to the final list of entity-subgraph pairs. Otherwise, we proceed to process the next entity. The module outputs a list of these valid entity-subgraph pairs for each node type.


\subsubsection{Complexity}
Algorithm \autoref{alg:seed_subgraph_extraction} is executed $|\tau|$ times, where $|\tau|$ represents the number of node types selected in Algorithm \autoref{alg:node_selection}. The cost of this algorithm is dominated by the execution time of SPARQL queries in Lines 3, 7, 8, and 13. The exact cost of each query will vary depending on the specific RDF engine being used, as it relies on the engine's implementation and built-in indices. The count queries in Lines 7 and 8 are the fastest. They only involve counting triples and predicates, without retrieving data, resulting in minimal processing time. Counting unique predicates has a slightly higher cost because it requires checking for uniqueness within the counted set. The query in Line 3 that retrieves entities with their labels has a higher cost than count queries. It retrieves a batch of entities based on a specified size and uses specific predicates to optimize efficiency. However, it remains less expensive than the subgraph extraction query. Line 13's query for extracting the subgraph is the most expensive. This query retrieves all triples surrounding the entity within a specified number of hops and direction. Let's denote the cost of executing this query as $q2_{cost}$. All validations within the algorithm are performed in constant time. Filtering the subgraph has a complexity of O($K$), where $K$ signifies the number of triples in the extracted subgraph. The overall time complexity of Algorithm \autoref{alg:seed_subgraph_extraction} is $O(\tau(q2_{cost}+K))$.

This type-based context extraction approach offers significant advantages over a brute-force solution that does not consider entity types. The brute-force approach retrieves all KG entities in a pre-processing step, necessitating storage space proportional to the number of entities in the KG. Our approach achieves better space and time complexity compared to the brute-force solution. In terms of space complexity, the brute-force solution requires storing potentially billions of entities, whereas our type-based approach works on-the-fly, eliminating storage requirements. Time complexity analysis reveals that the dominant factor for Algorithms \autoref{alg:node_selection} and \autoref{alg:seed_subgraph_extraction} combined is $O(\tau(q2_{cost}+K))$, where $\tau$ represents the number of selected node types, $q2_{cost}$ denotes the cost of extracting the subgraph, and $K$ signifies the number of triples in the extracted subgraph. This complexity is significantly lower compared to the time required to extract all KG entities. While our technique prioritizes efficiency and guarantees a sufficient number of unique predicates to generate meaningful conversation, it may not necessarily select entities surrounded by the highest number of unique predicates, which might be achievable with the brute-force approach. 


==> old_sections/context_extraction_May7.tex <==
\section{Context Extraction}
This module identifies topics for dialogue generation in three steps: \myNum{i} Entity Sampling, \myNum{ii} Textual Entity Representation, and \myNum{ii} Subgraph Extraction and Validation.

\subsection{Entity Sampling}

\begin{definition}[Subgraph $SG$]
\label{def:subgraph}
Given a $KG$ containing a set of vertices $V$ ,and a set of relations $R$. Let $e$ be the target seed entity. The subgraph $SG(e) = \{T\}$ is a set of triples, where $T = \langle s, p, o \rangle$ such that $s, o \in V$, $p \in R$, and $s= e$ or $o = e$      
\end{definition}
\label{sec:seed}
\input{algorithms/seed_entity}

This module selects a representative set of entities from a KG that will be used as topics to generate dialogues. We propose a type-based entity sampling approach that is efficient and scalable for large KGs. By relying on node types, this approach eliminates the need to retrieve all entities and perform time-consuming pre-processing steps, which require storage proportional to the billions of entities found in large KGs. Eliminating the pre-processing requirement significantly improved our time performance. The approach selects node types relevant to the target KG's domain, excluding metadata types. Then we calculate statistics on these types to determine the distribution of node types within the given number of seed entities to be sampled. Finally, we sample entities from each type to create the final set. This approach targets entities with sufficient surrounding facts to create rich dialogues while fitting in the context length of LLMs.
  
Algorithm \autoref{alg:seed_entity}  explains the entity sampling process in detail. It takes two inputs: the SPARQL endpoint of the target KG and the required number of dialogues. The number of entities to be sampled corresponds to the number of dialogues, as each entity serves as a dialogue topic. Lines 1-2 identify domain-specific types. We first retrieve all KG types using a SPARQL query to have a comprehensive list of types. Then, we filter this list to exclude irrelevant metadata types. By default, we use the main types defined in the KG's ontology, as these represent the KG's core information. Users have the flexibility to specify additional types or type prefixes for inclusion. Line 3 calculates the number of entities belonging to each filtered type using SPARQL queries. These counts are then used to determine the percentage of entities within each type. We define rare types in the KG as types with very few entities (in tens), resulting in negligible percentages. These highly specific types are often not the KG's main focus, so lines 4-5 identify them using a percentage threshold and remove them from the list. This removal causes the remaining type percentages to no longer sum to $100\%$. Therefore, we adjust the percentages by recalculating them for the included types only. Line 6 leverages the calculated percentages and the required number of entities to determine the number of entities to be sampled from each type. This ensures the sampled entities reflect a distribution similar to the overall KG entity distribution. Finally, line 7 utilizes the entity distribution and the SPARQL endpoint to retrieve entities for each type. The labels of these sampled entities must have a reasonable length suitable for LLM processing.

\subsection{Subgraph Extraction}
\input{algorithms/seed_validator}
Following entity sampling, we extract a surrounding subgraph for each entity to serve as the dialogue context. This subgraph will be used to generate multiple questions rather than a single complex question, as followed by existing systems. Extracting the subgraph requires defining its shape, width, and direction. For shapes, we focus on shapes suitable for dialogues. Complex shapes often lead to complex questions, which shorten the conversation by asking for many facts at once. These kinds of shapes and questions make the conversation challenging to maintain. Therefore, we focus on star-based shapes, where the entity acts as the central node. The width measured in the number of hops, determines the number of connections traversed outward from the entity. The direction parameter specifies whether predicates are considered only when outgoing from the entity, or include both incoming and outgoing connections. The subgraph includes all entities and literals connected to the central entity within the specified width and direction.

To ensure meaningful dialogue generation, we validate each sampled entity and its corresponding subgraph against specific criteria. Algorithm \autoref{alg:seed_validation} details this validation process where we use the LLM context length to determine the maximum length of the entity textual representation, the maximum size of the subgraph, and the minimum number of unique predicates surrounding the entities. First, we validate the entity. The textual representation of the entity must fall within a defined length limit. This prevents confusing the LLM and allows it to focus on information connected to the entity through predicates, instead of getting distracted by details within the textual label itself. Examples of invalid entities include publication entities whose labels contain publication year, location, or abstracts. For the subgraph, we start by measuring its size using the number of tokens it contains. This size must fit in the context length of the LLM. The subgraph needs to contain a sufficient number of unique predicates to facilitate the generation of rich dialogues. Because unique predicates connect the entities to different facts, which provide a strong foundation for generating multiple, distinct questions. Any invalid entity-subgraph pair is replaced with a new sample from the same entity node type. The module outputs a list of validated $\langle$entity, subgraph$\rangle$ pairs.

\subsection{Entity Representation}


The way an entity $e$ is represented affects both human's and LLM's understanding of this entity and subsequently generating meaningful questions. As explained in \autoref{sec:subgraph_approach}, entities are encoded using the final URI segment, this encoding function assumes the human-readability of this segment (e.g., \url{http://dbpedia.org/resource/The_Future_of_Freedom_Conference}).
However, this is not always the case as some in URIS this segment contains IDs (e.g., \url{https://dblp.org/pid/00/10071}) or character-number combinations (e.g., \url{https://dblp.org/rec/conf/valuetools/Coppa14}). In these instances, the LLM struggles to understand the entity's meaning, resulting in ambiguous or low-quality questions.

To overcome this, meaningful string representations for entities within triples are essential. Each entity in the knowledge graph (KG) is connected to multiple predicates; some, like "\textit{name}" for a Person or "\textit{title}" for a Publication, offer good representation. However, It is challenging to find a single predicate suitable for diverse KGs or node types. We need a mapping between node types and appropriate predicates for the target KG to retrieve the correct representation. One can assume that users creating KG benchmarks has the sufficient technical knowledge to provide this mapping. While this may be true for some cases, this is feasible only for small KGs with tens of node types. It becomes impractical for large KGs like DBpedia or Yago with hundreds or thousands of node types. This necessitates the automatic extraction of node type description labels within a given KG.

We propose an LLM-based approach to automatically extract description predicate $p_l$ for all node types within a KG. Let the node type be $t$, we extract all outgoing predicates $P_{list}$ connected to entities of type $t$. We filter $P_{list}$ to keep predicates connecting entities of type $t$ to string literals, this ensures that the entity representation is a string, not another entity. 

\begin{equation}
    \label{eq:entity}
    p_l = f(t, P_{list}, I)
\end{equation} 
In the instruction $I$, we prompt the LLM using zero-shot to choose from $P_{list}$, the most representative predicate that can serve as a label for node type $t$. This approach provides human-readable entity representation for all node types, regardless of the information type in the URI. It also eliminates the need for user input or technical expertise. This leads to better generated question quality and system usability.

% \begin{tcolorbox}
% Given the specified node type $<node type>$  and its associated predicates $<predicates>$, choose a suitable predicate to serve as a label for this type.
% \end{tcolorbox}
\begin{lstlisting}[language=Python, caption=Choosing representative predicate for type prompt, escapechar=@]
# Instruction:
Given the specified node type and its
associated predicates, choose a suitable
predicate to serve as a label for this type.

# Input:
node type:
predicates: 

# Response:
\end{lstlisting}


==> old_sections/context_extraction_april29.tex <==
\section{Context Extraction}
\subsection{Subgraph Extraction}
\begin{definition}[Subgraph $SG$]
\label{def:subgraph}
Given a $KG = (V,P)$ where $V$ is a set of vertices and $P$ is a set of predicates. Let $e$ be the target seed entity. The subgraph $SG(e) = \{T\}$ is a set of triples, where $T = \langle v_i, p, v_j \rangle$ such that $v_i, v_j \in V$, $p \in P$, and $v_i = e$ or $v_j = e$      
\end{definition}
\label{sec:seed}


This module identifies topics for dialogue generation in two steps: \myNum{i} Entity Sampling and \myNum{ii} Subgraph Extraction and Validation.

%% omij - didn't understood the first line
To guarantee diverse topics, we select a representative set of entities from various knowledge graph (KG) types.  Algorithm \autoref{alg:seed_entity} explains the entity sampling procedure. The inputs are the required number of dialogues which represents the number of subgraphs to extract and the $KG$ SPARQL endpoint. Line 1 extracts all types existing in the KG. In line 2, We filter for domain-specific types by keeping only those matching a pre-defined prefix and discarding metadata types. {\sysName} gives the user the flexibility to use the prefix of the target KG (e.g., "dblp" for DBLP graph) or to provide a prefix. In line 3, we calculate the percentage of entities belonging to each filtered type. In lines 4,5 we detect the rare types with minimal impact and eliminate them, some KGs contain thousands of rare types. We define rare types as types whose percentage is less than $1\%$. In line 6, based on adjusted percentages, we determine the number of nodes to sample from each remaining type. Leveraging the distribution and SPARQL endpoint, we retrieve entities following the adjusted distribution in line 7.
For each sampled node, we extract surrounding subgraphs which serve as the dialogue context.  Each subgraph includes all entities and literals connected to the seed node within a single hop. Extracting the subgraph operates in two steps, the first when the sampled node is the subject and the second when it is the object.

Both seed node and subgraph undergo validation as explained in Algorithm \autoref{alg:seed_validation}. The validations performed are: \myNum{i} Ensure that the seed node label length is within a specific limit to avoid confusing the LLM, \myNum{ii}
the subgraph size must fit within the LLM's context length, and \myNum{iii} the subgraph contains numerous unique predicates for richer dialogue generation. Since unique predicates serve as a good base for generating multiple different questions.
 We replace any invalid pairs with new samples. Ultimately, the module outputs a list of valid $\langle$entity, subgraph$\rangle$ pairs.

 
\input{algorithms/seed_entity}

\input{algorithms/seed_validator}


\subsection{Entity Representation}


The way an entity $e$ is represented affects both human's and LLM's understanding of this entity and subsequently generating meaningful questions. As explained in \autoref{sec:subgraph_approach}, entities are encoded using the final URI segment, this encoding function assumes the human-readability of this segment (e.g., \url{http://dbpedia.org/resource/The_Future_of_Freedom_Conference}).
However, this is not always the case as some in URIS this segment contains IDs (e.g., \url{https://dblp.org/pid/00/10071}) or character-number combinations (e.g., \url{https://dblp.org/rec/conf/valuetools/Coppa14}). In these instances, the LLM struggles to understand the entity's meaning, resulting in ambiguous or low-quality questions.

To overcome this, meaningful string representations for entities within triples are essential. Each entity in the knowledge graph (KG) is connected to multiple predicates; some, like "\textit{name}" for a Person or "\textit{title}" for a Publication, offer good representation. However, It is challenging to find a single predicate suitable for diverse KGs or node types. We need a mapping between node types and appropriate predicates for the target KG to retrieve the correct representation. One can assume that users creating KG benchmarks has the sufficient technical knowledge to provide this mapping. While this may be true for some cases, this is feasible only for small KGs with tens of node types. It becomes impractical for large KGs like DBpedia or Yago with hundreds or thousands of node types. This necessitates the automatic extraction of node type description labels within a given KG.

We propose an LLM-based approach to automatically extract description predicate $p_l$ for all node types within a KG. Let the node type be $t$, we extract all outgoing predicates $P_{list}$ connected to entities of type $t$. We filter $P_{list}$ to keep predicates connecting entities of type $t$ to string literals, this ensures that the entity representation is a string, not another entity. 

\begin{equation}
    \label{eq:entity}
    p_l = f(t, P_{list}, I)
\end{equation} 
In the instruction $I$, we prompt the LLM using zero-shot to choose from $P_{list}$, the most representative predicate that can serve as a label for node type $t$. This approach provides human-readable entity representation for all node types, regardless of the information type in the URI. It also eliminates the need for user input or technical expertise. This leads to better generated question quality and system usability.

% \begin{tcolorbox}
% Given the specified node type $<node type>$  and its associated predicates $<predicates>$, choose a suitable predicate to serve as a label for this type.
% \end{tcolorbox}
\begin{lstlisting}[language=Python, caption=Choosing representative predicate for type prompt, escapechar=@]
# Instruction:
Given the specified node type and its
associated predicates, choose a suitable
predicate to serve as a label for this type.

# Input:
node type:
predicates: 

# Response:
\end{lstlisting}


==> old_sections/evaluation_june28.tex <==
\section{Evaluation}
\subsection{{\sysName} Configuration}
{\sysName}  is a configurable benchmark generation framework. It empowers users to generate benchmarks tailored to their specific needs using different settings. Users can create benchmarks containing the required number of questions and targeting various KGs with minimal configuration. To initiate the benchmark generation, users specify the following key parameters: \myNum{i} the KG endpoint URL, \myNum{ii} the number of dialogues, \myNum{iii}  the maximum number of questions per dialogue, and \myNum{iv}  the LLM to use per module
% , and \myNum{v} the workflow type (complex or simplified).

\subsection{Evaluation Setup}
\subsubsection{Compared Systems}
We evaluate {\sysName} against Maestro \cite{maestro}, the state-of-the-art system for generating benchmarks for KGs. The code of Maestro\cite{maestro} is available. The results reported for Maestro are a result of our running of the system.
\subsubsection{Three Different Real KGs}
To evaluate the system's ability to run with KGs of different domains, We use three KGs: DBpedia, Yago, and DBLP. DBpedia and yago are general knowledge graphs. They contain information about people, places, and movies, … etc. DBLP is an academic graph that contains information about scientific publications, authors, and citations. 
\subsubsection{Computing Infrastructure}
We use two different settings for our experiments. In the first setting, We use a Linux machine with $180GB$ RAM and $16$ CPU cores. We use this setting for deploying KGs on virtuoso SPARQL endpoints, running {\sysName} with closed access models i.e. models accessed using APIs, and running Maestro. In the second setting, We use a Linux machine with one Nvidia A100 40GB GPU Card, 32 CPU cores and 64GB RAM. We use this setting to host Open source LLMs, and running {\sysName} with them.
\subsubsection{{\sysName} implementation and settings}
{\sysName} is implemented using Python $3.10$, Lang chain library v$0.1.4$, and OpenLLM library v$0.4.44$ \cite{Pham_OpenLLM_Operating_LLMs_2023} to host the open source LLMs. For SPARQL endpoints, we use Virtuoso v$7.2.5.2$, as it is widely adopted as an endpoint for big KGs. We prepare three different Virtuoso endpoints, one for each of the KGs. The standard, unmodified installation of the Virtuoso engine was used in all of our experiments. For node type selection, we use $1\%$ rare types' threshold, and $99\%$ shadowed parent threshold. For entity and subgraph extraction, we use entity batch size of $10,000$, number of hops is equal to $1$, and outgoing and incoming predicate direction. 
\subsubsection{LLMs}
We evaluated {\sysName} using different LLMs of different sizes. They can be divided into two categories: \myNum{i} Closed access models: GPT-3.5-turbo\cite{radford2018improving}\cite{instructgpt}, GPT-4\cite{gpt4}, GPT-4o\cite{gpt4o}, Gemini-1-pro\cite{geminiteam2024gemini1}, Gemini-1.5-pro\cite{geminiteam2024gemini15}, and \myNum{ii} Open source LLMs: LLAMA-2-7B \cite{llama2}, LLAMA-2-13B \cite{llama2}, LLAMA-3-8B \cite{llama3modelcard}, LLAMA-3-8B-instruct \cite{llama3modelcard}, CodeLLAMA-7B \cite{codellama}, CodeLLAMA-13B \cite{codellama}, Mistral-7B-v0.1 \cite{mistral}, Mistral-v0.1-instruct \cite{mistral}, Mistral-7B-v0.2 \cite{mistral}, Mistral-v0.2-instruct \cite{mistral}. The closed access models are used via sending requests to their APIs. Open source LLMs are used via sending requests to our server hosting these LLMs.

\subsection{Benchmark Quality}
We evaluated {\sysName}'s ability to generate human-like questions. \autoref{fig:independent_example} shows examples of the generated questions. The textual entity representation plays a crucial role. Disabling this module and relying on the URI's last segment significantly impacts question quality and clarity, as shown in \autoref{fig:independent_example}. This results in a significant increase in question validation errors, indicating the absence of the entity representation in the generated questions. This demonstrates the importance of a meaningful entity representation to the LLM to comprehend the entity and generate questions. Disabling the module resulted in a significant increase in question validation errors, from $1$ to $109$ for DBLP KG, from $1$ to $51$ for Yago KG, and from $0$ to $16$ for DBpedia KG. This highlights the effectiveness of textual representations, as a reduction in the number of errors suggests improved LLM understanding and question quality.

We compared the independent questions generated by {\sysName} and Maestro to determine which system produces more human-like questions. \autoref{fig:independent_example} illustrates examples generated by the two systems. All Maestro’s questions for the same seed entity have the same answer, the entity itself. This leads to similar questions asking about the same facts with different rephrasing.
In contrast, {\sysName} asks questions about various facts surrounding the chosen entity. This diversity in facts included in questions suggests {\sysName}'s superior performance. The same pattern persists for the other KGs: Yago and DBpedia. This improvement is attributed to the rich subgraphs with multiple facts used for question generation, and the entity representation module, which empowers the LLM to understand the entity's meaning and rely on its capabilities instead of rule-based approach followed by Maestro.

\begin{figure}[t]
	\begin{verbatim}
Maestro:
1. Who authored the Publication "baraki19"?
2. The authored by of the Publication "baraki19"?
3. Is the Person "8766" the authored by of
the  Publication "baraki19"?
4. What authored by the Person "11171"?
5. Who is the authored by of the Publication "daun18"?

Chatty-Gen using predicate label:
1. Who is the author of Cooperative Situation
Awareness in Transportation?
2. In which year was Cooperative Situation 
Awareness in Transportation published?
3. What is the primary affiliation of Jiaxin Pan?
4. Is Jiaxin Pan associated with any other affiliation?
5. In which journal was 'Trust-Region Methods
on Riemannian Manifolds.' published?

Chatty-Gen without predicate label
1. What is the bibtex Type of item Adler12?
2. Who is the author of Adler12?
3. When was the Phdthesis 'Bailer20' published?
4. Which school accepted the thesis in publication
Beck15?
5. In which year was publication Beck15 published?
	\end{verbatim}
	\caption{Examples of independent questions generated by Maestro and {\sysName} with and without using labels for DBLP KG.}
	\label{fig:independent_example}
\end{figure}

We evaluated {\sysName} and Maestro with respect to the question types covered in their generated benchmarks. \autoref{fig:coverage} illustrates the distribution of question types (question words) for both systems on the three KGs: DBLP, Yago, and DBpedia. We group questions that does not start with a question word into categories. Examples include Yes/No questions (We refer to it as Boolean) starting with \textit{is, did, …, etc.}, and questions starting with nouns (we refer to it as Noun) such as \textit{through, the, by, ..., etc.} As shown in Figures \ref{fig:yago_maestro_complexity} and \ref{fig:dblp_maestro_complexity}, Maestro has a bias towards boolean questions for YAGO and DBLP, whereas {\sysName} produces a less biased distribution. For DBpedia, we compared the benchmark question types generated by the two systems with the human generated QALD-9 dataset (\autoref{fig:maestro_complexity}). While QALD-9 offers a wider variety of question types than either system, {\sysName} still demonstrates a good variation, despite being automatically generated. Notably, Maestro's bias towards boolean questions persists, generating a higher percentage of boolean questions compared to the average in question answering benchmarks. For example, QALD-9 contains only $3\%$ boolean questions, while Maestro generates $34\%$. In contrast, {\sysName} produces a more typical percentage of boolean questions. {\sysName}’s consistency across the three KGs suggests its ability to work with different KGs from various domains.

\begin{figure*}[t]
\centering
   \begin{subfigure}{.3\textwidth}
   	\centering
   	\includegraphics[width=\columnwidth]{figures/maestro_complexity_yago.pdf}
   	\caption{YAGO KG}
   	\label{fig:yago_maestro_complexity}
   \end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dblp.pdf}
	\caption{DBLP KG}
	\label{fig:dblp_maestro_complexity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dbpedia.pdf}
	\caption{DBpedia KG}
	\label{fig:maestro_complexity}
	\end{subfigure}
	\caption{Comparison of the coverage of question types generated by Maestro and {\sysName} for the three KGs.}
	\label{fig:coverage}
\end{figure*}

{\sysName} effectively generates high-quality dialogues that mimic human conversations. \autoref{fig:example} shows examples of the generated dialogues for DBLP and YAGO KGs. The questions within the dialogue are relevant and form a coherent discussion about various facts related to one entity.\shorten

% \begin{figure}[t]
% 	\begin{verbatim}
% 		Example YAGO:
% 		1. What is the birth place of Charlie Chaplin?,
% 		2. What is his nationality?,
% 		3. What are his alternate names?,
% 		4. What awards did he receive?,
% 		5. When did he die?
		
% 		Example DBLP:
% 		1. What is the bibtex Type of 'An Adaptive Hierarchical
% 		Approach to the Extraction of High Resolution Medial
% 		Surfaces.'?,
% 		2. How many creators does it have?,
% 		3. Is it listed on the Toc Page?,
% 		4. What is the year of publication?,
% 		5. In which event was it published in 2012?
% 	\end{verbatim}
% 	\caption{Examples of generated questions by {\sysName} for the different KGs.}
% 	\label{fig:example}
% \end{figure}

% yago - gpt-4 example
% dblp - gpt-4 example
\begin{figure}[t]
	\begin{verbatim}
Example YAGO:
1. Where was Arthur Stuart-Menteth Hutchinson born?
2. What alternate names are known for him?
3. What was the occupation of him?
4. When did he die?
5. Where did he pass away?

Example DBLP:
1. What type of work is 'Systems of Logic Based on -
-Ordinals.' classified as in Bibtex?
2. Who authored it?
3. What is the DOI of it?",
4. In which year was it published?
5. How many creators were involved in it?
	\end{verbatim}
	\caption{Examples of generated questions by {\sysName} for the different KGs.}
	\label{fig:example}
\end{figure}


\subsection{Node type Distribution}
We evaluate the seed node selection module in {\sysName} and Maestro to ensure the chosen node types reflect the node type distribution in the KG. \autoref{fig:diversity2} illustrates how the KG node type distribution compare to {\sysName} and Maestro. We obtain node types by querying the KG endpoint for each chosen entity and calculating the percentage of each type. For {\sysName}, most types closely match the KG distribution. However, some differences exist because some nodes have multiple types, so a single seed contributes to multiple types. On the other hand, Maestro does not include many seeds from the most representative types in the KG. For instance, the Person type, constituting $18\%$of DBpedia KG entities, is absent from Maestro's benchmark. Maestro generates a high percentage of rare types, like Social Person ($26\%$ of its benchmark). To simplify the figure, we excluded KG types with less than $5\%$ 

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity.pdf}
% 		\caption{DBLP KG}
% 		\label{fig:dblp_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity.pdf}
% 		\caption{YAGO KG }
% 		\label{fig:yago_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity.pdf}
% 		\caption{DBpedia KG}
% 		\label{fig:dbpedia_diversity}
% 	\end{subfigure}
	 
% 	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
% 	\label{fig:diversity}	
% \end{figure*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity2.pdf}
		\caption{DBLP KG}
		\label{fig:dblp_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity2.pdf}
		\caption{YAGO KG }
		\label{fig:yago_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity2.pdf}
		\caption{DBpedia KG}
		\label{fig:dbpedia_diversity2}
	\end{subfigure}
	 
	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
	\label{fig:diversity2}	
\end{figure*}

\subsection{Systems Time Performance}
\input{tables/maestro_timev2}
This experiment analyzes the time taken by Maestro and {\sysName} to produce benchmarks of $100$ questions for different KGs, \autoref{tab:maestro_time} shows the time taken in hours by both systems. Maestro first needs to traverse the whole KG. It extracts all predicates with their context, a context defined as (predicate, subject\_type, object\_type).  All contexts are saved in PostgreSQL Database for subsequent access. Then, the required number of seed entities is retrieved from the Database and the benchmark generation process starts. In \autoref{tab:maestro_time}, we show the number of predicates processed by Maestro per KG, for DBLP and YAGO we included all predicates, while for DBpedia we stopped at $18,211$ out of $994,592$ predicates for memory limitations, but the whole process needs days to finish. Maestro time is dominated by this preprocessing, and it is proportional to the number of predicates. {\sysName} uses the information in the entire KG on the fly, and needs minutes to run the end-to-end generation process, regardless of the size of the target KG. This order of magnitude improvement in running time can be attributed to the seed sampling process explained in \autoref{sec:seed}. It eliminates the need to perform any pre-processing step, while the validation of the extracted seeds ensures that the seeds are good enough to create meaningful questions.

\subsection{Summarization}
In the following experiments, We evaluate the effect of subgraph summarization on the cost (number of tokens), time to complete benchmark generation, and percentage of correct SPARQL queries generated by LLMs.
\input{tables/subgraph_vs_summarized}

\subsubsection{Cost Efficiency}
The cost is defined as the number of tokens sent to and returned from the LLM in each end-to-end pipeline. To evaluate the cost of the two approaches, we report the average, minimum, maximum, and total number of tokens needed to generate benchmarks of 20 dialogues ( $\approx$ 100 questions) As shown in \autoref{tab:comp}, {\sysName} consistently has lower costs across the different KGs. This demonstrates the efficiency of summarizing the subgraph. There is a cost difference between YAGO and DBLP, although both are generated using the same number of dialogues. This can be attributed to the longer DBLP labels, e.g. paper titles.

\subsubsection{Answer Correctness}
We evaluate the subgraph and summarized approaches with respect to generating syntactically correct SPARQL queries that retrieve the answer to the questions. We validate the queries by executing them against the remote KG endpoint, and only correct question-query pairs exist in the benchmark. If a query fails to execute, it's considered a syntax error. If it executes but returns a different answer than the one stored in the subgraph, it's marked as incorrect. Otherwise, it's considered correct. \autoref{tab:comp} shows the percentage of correct queries generated by {\sysName}  and the subgraph approach across the three KGs. {\sysName}  outperforms the subgraph approach in all KGs. This improvement arises from removing the answer when creating the summarized subgraph, which reduced LLMs confusion. In general, both {\sysName}  and the subgraph approach perform better on YAGO compared to DBLP. This can be attributed to two factors: \myNum{i} YAGO's domain (general knowledge) is more similar to the data the LLMs were trained on, and \myNum{ii} the long labels for publication names in DBLP can confuse the LLM during processing the subgraph.

\subsubsection{Time Efficiency}
We compare the average time taken by {\sysName} and the subgraph approach to generate one dialogue with its SPARQL queries. This time is divided into processing time of the LLM and network latency if the LLM resides on a remote server.  \autoref{tab:comp} shows that both approaches needs comparable time to generate dialogues, as the network latency dominates the time.

\subsection{LLMs}

We evaluated {\sysName}'s ability to work with multiple LLMs of different sizes. We tested it with closed-access models (GPT-3.5, GPT-4, GPT-4o, Gemini-Pro-1) and open-source models (LLAMA-2 (7B/13B), LLAMA-3 (8B), LLAMA-3-instruct (8B), CodeLLAMA (7B/13B), Mistral-v0.1 (7B)). We analyzed the performance of the models to identify the best performing models. Then we tested {\sysName} with two variation of using different LLMs for each stage. Our first variation is using  LLAMA-3-instruct (8B) for Question-triple and Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. The second variation is using GPT-4 for Question-triple Generation, LLAMA-3-instruct (8B) for Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. To assess performance, we generated benchmarks consisting of $20$ dialogues, each containing a maximum of $5$ questions. We evaluated with two KGs of different domains: YAGO and DBLP. To ensure a finite evaluation process, we set a limit of $500$ seed entities. If this limit was reached before generating the $20$ dialogues, we stop the process.

\autoref{tab:openllm} shows the results of this experiment, Num\_seeds is the total number of seeds used to successfully generate the $20$ dialogues. Dialogues-S is the number of successfully generated dialogues, since some models reaches the limit of $500$ before generating all $20$ dialogues. Questions-E and Triples-E are the number of validation errors skipped for the question and triples generation, respectively. and Dialogue-E is the number of invalid dialogues. Parsing-E identifies the cases where LLMs failed to return a correctly structured response. Time is the total time taken by {\sysName} to generate the benchmark in minutes. Number of tokens is the sum total number of tokens sent to and returned from the LLMs in millions to generate the benchmarks. The table shows the performance of each LLM across domains (YAGO and DBLP), and across multi-stage (\autoref{sec:workflow}) and single-stage {\color{blue}{(???)}} workflows.
% we need section for single stage 

\autoref{tab:openllm} shows that GPT-3.5, GPT-4, and GPT-4o are not affected by changes in domain or task complexity. For Gemini-Pro-1 and open-source LLMs, performance is impacted by change of domain, with most models performing better on YAGO KG. This is due to similarity between YAGO data (general knowledge) to the LLMs’ training data, unlike DBLP (academic, domain-specific data). DBLP also contains long titles of papers and conferences (longer than average entity length in YAGO) which can confuse LLMs and reduce performance. These models are also affected by pipeline complexity change, they perform better with the complex pipeline which requires fewer prompts. This is likely because of the higher number of prompts, which increases the probability of LLM hallucinations. The complex pipeline requires $7$ prompts ($1$ question and triples, $5$ SPARQL, and $1$ dialogue) while the simplified requires $12$ prompt ($1$ question, $5$ triples, $5$ SPARQL, and $1$ dialogue). The simplification has the potential to improve the performance of LLMs, but it is preferred in single prompt solutions where a task can be broken down to minimal number of subtasks.  Overall, the top performing LLMs across both KGs are GPT-3.5, GPT-4, GPT-4o, CodeLLama (13b), and Gemini-Pro-1. These models require less than 100 seed entities to process before generating 20 dialogues. Using variations of LLMs for different stages can achieve comparable performance to the top performing models at a lower cost. For example, Multi-LLM-2 variation leverages the code generation ability of CodeLLama's (13b) for SPARQL queries and the natural language capabilities of LLAMA-3 instruct (8B) for dialogue generation, requiring GPT-4 only for the complex question-triples generation task.


% for the table we should say that multi-stage approach 

\autoref{tab:openllm} {\color{blue} {shows that the performance of the GPT-3.5, GPT-4, GPT-4o, Gemini-1-pro, CodeLLAMA-13b models are not affected by changes in the domain in our multi-stage approach, and it degrades from YAGO KG to DBLP KG for open-source models like LLAMA-2-13b, CodeLLAMA-7b, Mistral-7b-v0.1. This behaviour is likely due to change of domain, YAGO KG contains general knowledge data, unlike DBLP KG which contains academic, domain-specific data. DBLP KG also contains long titles of papers and conferences (longer than average entity length in YAGO KG) which can confuse LLMs and reduce performance. With single-stage approach GPT-4o's success rate ratio(number of seeds to successful dialogues) for YAGO KG and DBLP KG are 39\% and 7\% respectively, the same ratio is 95\% and 100\% for multi-stage approach. Overall only GPT-4o, Gemini-1.5-pro and LLAMA-3-8b-inst are able to generate 20 successful dialogues in one-stage approach, and all of the other open-source models failed to do it even after 1000 seeds. With multi-stage approach almost every model is able to generate 20 successful dialogues, except LLAMA-2-7b which failed to generate even single dialogue for both KGs. Overall, for our multi-stage approach the top performing LLMs across both KGs are GPT-3.5, GPT-4, GPT-4o, CodeLLama (13b), and Gemini-1-Pro. These models require less than 100 seed entities to process before generating 20 dialogues. Using variations of LLMs for different stages can achieve comparable performance to the top performing models at a lower cost. For example, Multi-LLM-2 variation leverages the code generation ability of CodeLLama's (13b) for SPARQL queries and the natural language capabilities of LLAMA-3 instruct (8B) for dialogue generation, requiring GPT-4 only for the complex question-triples generation task. The time taken and number of tokens is proportional to number of prompts or an api calls, in multi-stage approach the }}

==> old_sections/evaluation_may24.tex <==
\section{Evaluation}
\subsection{{\sysName} Configuration}
{\sysName} is a configurable benchmark generation framework, i.e. users have the flexibility to generate benchmarks using different settings. It empowers users to generate benchmarks tailored to their specific needs. Users can effortlessly create benchmarks containing any desired number of questions and targeting various KGs. Furthermore, the framework offers the flexibility to choose between two distinct approaches for question generation: the subgraph approach and the summarized approach. To initiate the benchmark generation, users need to provide five key parameters: \myNum{i} the KG endpoint URL, \myNum{ii} the desired number of dialogues, \myNum{iii}  the maximum number of questions per dialogue, \myNum{iv} the preferred approach (subgraph or summarized), and \myNum{v} the language model. With these parameters, the framework generates benchmarks that can be used to assess the strengths and weaknesses of different question-answering systems.  

\subsection{Evaluation Setup}
\subsubsection{Compared Systems}
We evaluate {\sysName} against Maestro\cite{maestro}, the state-of-the-art system for generating benchmarks for KGs. The code of Maestro\cite{maestro} is available. The results reported for Maestro is a result of our running of the system.
\subsubsection{Three Different Real KGs}
To evaluate the system's ability to run with KGs of different domains, We use $3$ KGs: DBpedia, Yago, and DBLP. DBpedia and yago are general knowledge graphs. They contain information about people, places, and movies. DBLP is an academic graph that contains information about scientific publications, authors, and citations. 
\subsubsection{Computing Infrastructure}
We use two different settings for our experiments. In the first setting, We use a Linux machine with $180GB$ RAM and $16$ CPU cores. We use this setting for deploying KGs on virtuoso SPARQL endpoints, running {\sysName} with GPT models, and running Maestro. In the second setting, We use a Linux machine with one Nvidia A100 40GB GPU Card, 32 CPU cores and 64GB RAM. We use this setting for running {\sysName} with openLLMs namely, LLAMA, CodeLLAMA, and Mistral.
\subsubsection{{\sysName} implementation and settings}
{\sysName} is implemented using Python $3.10$. To run {\sysName}, users need to specify the target KG. Our experiments test {\sysName} using two categories of LLMs: \myNum{i} Private models (OpenAI, Google), and \myNum{ii} Open Source LLMs. For SPARQL endpoints, we use Virtuoso $7.2.5.2$, as it is widely adopted as an endpoint for big KGs. We prepare three different Virtuoso endpoints for each of the KGs. The standard, unmodified installation of the Virtuoso engine was run at the endpoints and used in all of our experiments.
\subsubsection{LLMs}




\subsection{Independent Questions}
\input{tables/question_quality}
\begin{figure*}[t]
\centering
   \begin{subfigure}{.3\textwidth}
   	\centering
   	\includegraphics[width=\columnwidth]{figures/maestro_complexity_yago.pdf}
   	\caption{YAGO KG}
   	\label{fig:yago_maestro_complexity}
   \end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dblp.pdf}
	\caption{DBLP KG}
	\label{fig:dblp_maestro_complexity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dbpedia.pdf}
	\caption{DBpedia KG}
	\label{fig:maestro_complexity}
	\end{subfigure}
	\caption{Comparison of the coverage of question types generated by Maestro and {\sysName} for the three KGs.}
	\label{fig:coverage}
\end{figure*}
\begin{figure*}[t]
	\centering
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity.pdf}
		\caption{DBLP KG}
		\label{fig:dblp_diversity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity.pdf}
		\caption{YAGO KG }
		\label{fig:yago_diversity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity.pdf}
		\caption{DBpedia KG}
		\label{fig:dbpedia_diversity}
	\end{subfigure}
	 
	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
	\label{fig:diversity}	
\end{figure*}

\input{tables/maestro_time}
% Conclusion from Maestro Discussion
% \begin{itemize}
%     \item The time performance depends on the number of classes in the KG, not the overall size of the graph
%     \item Having local KG can be faster since remote graphs can impose speed restrictions per user
%     \item He advised me to change the offsets for small graphs such as DBLP to get better inclusion of types (which I am trying)
% \end{itemize}

{\sysName} produces the set of independent questions besides the final generated dialogues. We compare {\sysName} with Maestro on the level of generating independent questions with respect to clarity coverage of types, diversity across node types, and the end-to-end system performance, on a sample of approximately $100$ questions. 

\subsubsection{Quality of Questions}
\begin{figure}[t]
	\begin{verbatim}
		Maestro:
		1. What is the edited by of the Publication "2008"?
		2. Mention the edited by of the Publication "2008"?
		3. The edited by of the Publication "2008"?
		4. Was the Publication "2021" edited by the 
  Creator "651"?
		5. Was the Publication "njap13" edited by the
Creator "651"?"

CoKG:
1. Who has authored 'Cooperative Situation Awareness
in Transportation.'?
2. In what year was 'Cooperative Situation Awareness 
in Transportation.' published?
3. What is the primary Affiliation of Marian Daun?
4. Does Gerhard Kramer have an ORCID?
5. When was 'Natural Language Grounded Multitask 
Navigation' published?
	\end{verbatim}
	\caption{Examples of independent questions generated by Maestro and {\sysName} for DBLP KGs.}
	\label{fig:independent_example}
\end{figure}

Since {\sysName} and Maestro's benchmarks are automatically generated, we need to evaluate the quality of the generated questions to ensure their similarity to human-generated questions. This includes linguistic correctness, i.e. The questions are grammatically correct and well-formed.
To assess the quality we defined the validity of the question by the following criteria: \myNum{i}Grammatically correct, \myNum{ii} Linguistically correct.  We sent a sample of approximately $100$ questions to a group of in-house annotators, with the criteria for valid questions.
Both {\sysName} and Maestro managed to produce a good quality question with {\sysName} providing a better quality as shown in \autoref{fig:independent_example}.
The better quality of {\sysName} for the three KGs is attributed to the entity representation module that empowers the LLM to understand what the entity represents. Maestro deals with the seed entity it chooses as the answer to the question, that's why questions for the same entity are asking about similar facts. On the other hand, {\sysName} asks questions about different facts surrounding the chosen entity.


\subsubsection{Coverage of types}
We evaluate the ability of the {\sysName} and Maestro to challenge the different KGQA systems by generating questions with different types. \autoref{fig:coverage} shows the difference in the distribution of different question words, i.e. different question types, for the two systems on the three KGs. For yago and dblp as shown in \autoref{fig:yago_maestro_complexity} and \autoref{fig:dblp_maestro_complexity}, we can observe Maestro’s bias to boolean questions. While {\sysName} provides a less biased distribution. For DBpedia, we compare the benchmark generated by the two systems with QALD-9 as shown in \autoref{fig:maestro_complexity}. Although the distribution of QALD-9 contains more types than both systems, {\sysName} contains a good variation of question types, despite being automatically generated. Maestro’s bias to boolean questions is still evident, it produces more boolean questions than the average of question answering benchmarks, e.g. QALD-9 contains only $4$ boolean questions from 150 samples, while Maestro generated $30$ is questions from $100$ questions.{\sysName} produces a closer to normal percentage of boolean questions. {\sysName} achieves comparable results on the three KGs, showing its ability to work with different KGs from different domains. Maestro produces some strangely formatted questions, i.e. questions that start with \textit{The} with a high percentage. 


\subsubsection{Diversity}
We evaluate the seed node selection module in {\sysName} and Maestro to ensure that the chosen node types follow a similar distribution to the node types in the KG. \autoref{fig:diversity} shows the distribution of node types in the original KG, compared to the distribution of node types selected by the two systems. We obtain these types through querying the KG endpoint to get the associated type(s), after getting the types of all nodes we calculate the percentage of each type. We only include the non-rare types, i.e. types that exist more than $1\%$ in the KG.
For {\sysName}, the percentage of most types is close to the KG distribution. For some types, you can find a difference in the percentage, as for DBLP KG, some nodes are associated with more than one type, so one seed node in the benchmark contributes to more than one node type. Maestro does not include many seeds from the most representative types in the KG. For DBpedia KG Person represents approximately $17\%$ from the entities in the KG but is unrepresented in the benchmark generated by Maestro.  It is also observable that Maestro produces a high percentage for rare types, e.g. Country, which constitutes $17\%$ of the generated benchmark.


\subsubsection{Systems Time Performance}
This experiment analyzes the time taken by Maestro and {\sysName} to produce benchmarks for different KGs. \autoref{tab:maestro_time} shows that Maestro's time is proportional to the number of different predicates i.e. types existing in the KG.
Maestro needs hours to index the whole KG and save it in a PostgreSQL Database for subsequent access. In the pre-processing step, Maestro visits the whole KG, and extracts all predicates with their associated context, a context is the type of the entities connected by the predicate. Then, they extract the required seed entities from the Database and start the question-generation process. On the other hand, {\sysName} needs minutes to run the end-to-end generation process. This order of magnitude improvement in running time can be attributed to the seed sampling process explained in \autoref{sec:seed}. It eliminates the need to perform any pre-processing step, while the validation of the extracted seeds ensures that the seeds are good enough to create meaningful questions. 


\subsection{Generated Dialogues}
In the following experiments, we evaluate the performance of {\sysName}'s in dialogue generation. Due to the lack of existing systems that automatically creates dialogue benchmarks from knowledge graphs, we evaluate {\sysName}  against the subgraph approach explained in \autoref{sec:subgraph_approach}.
\subsubsection{Quality of Questions}
\begin{figure}[t]
	\begin{verbatim}
		Example YAGO:
		1. What is the birth place of Charlie Chaplin?,
		2. What is his nationality?,
		3. What are his alternate names?,
		4. What awards did he receive?,
		5. When did he die?
		
		Example DBLP:
		1. What is the bibtex Type of 'An Adaptive Hierarchical
		Approach to the Extraction of High Resolution Medial
		Surfaces.'?,
		2. How many creators does it have?,
		3. Is it listed on the Toc Page?,
		4. What is the year of publication?,
		5. In which event was it published in 2012?
	\end{verbatim}
	\caption{Examples of generated questions by {\sysName} for the different KGs.}
	\label{fig:example}
\end{figure}
\input{tables/cost}
\input{tables/answer}

For evaluating the quality of dialogues, we use the validity metrics explained for independent questions in addition to question relevance, which evaluates whether the questions are related to each other and form a coherent dialogue.
\autoref{fig:example} shows an example of the generated dialogues for DBLP and YAGO KGs. 
In addition to the quality criteria for independent questions, we add the following dialogue-based criteria:  \myNum{i} questions are relevant to each other, \myNum{ii} form a dialogue about one specific entity, \myNum{iii} First question explicitly mentions the entity, \myNum{iv} Subsequent questions do not explicitly mention the entity. For points \myNum{i} and \myNum{ii}, we sent a sample of $20$ dialogues (approximately 100 questions) to a group of in-house annotators, with the criteria for valid questions.
For points \myNum{iii} and \myNum{iv}, we relied on the question validator to perform this validation, If the validation fails the entity will be skipped and another entity is re-sampled. We report the number of seed entities skipped due to these validations. We evaluated benchmarks generated from three different KGs: DBLP, YAGO, and DBpedia in \autoref{tab:quality}. The top part of the table represents the number of valid questions as evaluated by the annotators, while the bottom part represents the number of skipped seed nodes as evaluated by the validators. {\sysName} managed to produce a good percentage of generated valid questions, with minimal seed entities skipped, the maximum is $15$ entities in Yago KG.


\subsubsection{Cost Efficiency}

The cost is defined as the number of tokens sent to and returned from the LLM in each end-to-end pipeline. As shown in \autoref{tab:cost}, {\sysName} consistently has lower costs across the different KGs. This shows the effect of using the summarized version of the KG, besides using triple with no answer. In \autoref{tab:cost}, the saved cost for YAGO is significant, {\sysName} saves around 40\% of the number of tokens. There is a cost difference between YAGO and DBLP, although both of them are generated using the same number of dialogues, which can be attributed to the longer DBLP labels e.g. paper titles.

%Another evidence for the superiority of the summarized approach from cost perspective, For large KGs such as DBpedia, the summarized approach will accommodate bigger subgraphs. To get a sample of 20 graphs on DBpedia, the summarized approach had to discard $8$ subgraphs because they did not fit in the LLM context length, while the subgraph approach needed to skip $281$ subgraphs.
 
\subsubsection{Answer Correctness}

This experiment analyzes the ability of each approach to create syntax-correct SPARQL queries that retrieve the correct answer to the dialogue questions. To validate the SPARQL query, we execute the query on the remote endpoint of the KG. and we extract the answer from the subgraph. If the query did not execute then it is a syntax error, if the query executed and returned a different answer than the answer in the subgraph, it is incorrect. Otherwise, it is a correct query.
\autoref{tab:answer} shows the percentage of correct queries across KGs for {\sysName} and the subgraph approach. {\sysName} provides a better percentage in the two tested KGs. Removing the answer from the triples in the input subgraph decreased the LLM confusion. In general, the percentages of {\sysName} and the subgraph approach for YAGO are better than DBLP, this can be attributed to: \myNum{i} YAGO is a general KG i.e. its domain is similar to the data the LLMs were trained on so it can handle this data better, and \myNum{ii} the long labels for the publication names in the DBLP can cause some confusion to the LLM in understanding the input subgraph.

\subsubsection{Time Efficiency}
This experiment analyzes the average time taken by {\sysName} and the subgraph approach to generate one dialogue with its SPARQL queries. The time in both approaches is hugely affected by the response time of the LLM used, which usually resides on a remote server. As shown in \autoref{tab:time}, {\sysName} has a slightly better time to generate the dialogue, this happens due to the shorter prompts generated by our approach because of summarizing the graph and removing any answers.


%\begin{figure*}[t]
%  \centering
%  \begin{subfigure}{.3\textwidth}
%\includegraphics[width=\linewidth]{figures/dblp_diversity.pdf}
%\caption{DBLP KG}
%\label{fig:dblp_diversity}
%\end{subfigure}
%\hfill
% \begin{subfigure}{.3\textwidth}
%  \includegraphics[width=\linewidth]{figures/yago_diversity.pdf}
%\caption{YAGO KG }
%\label{fig:yago_diversity}
%\end{subfigure}
%\hfill
% \begin{subfigure}{.3\textwidth}
%  \includegraphics[width=\linewidth]{figures/dbpedia_diversity.pdf}
%    \caption{DBpedia KG }
%    \label{fig:dbpedia_diversity}
%\end{subfigure}
%
%\caption{Comparison of the distribution of node types sampled by {\sysName} for different KGs on a benchmark of 20 dialogues }
%\label{fig:diversity}
%
%\end{figure*}


%\subsection{Use Case}
%\input{tables/kg_qa}
%One of the motivations of our benchmark generation framework is to showcase the need to focus on generating chatbots for KGs that users can use to explore the KGs they are dealing with. To show this, we tested with a recent KGQA system KGQAn\cite{kgqan} on one of the benchmarks generated by our framework. Since our generated benchmarks contains both the independent questions and the dialogue, we evaluated the system using the two sets of questions. As shown in \autoref{tab:kgqa}, the recall when testing with the set of independent question is higher than the recall when testing on the dialogue, leading to a better F1 score. This reflects the inability of the system to answer the questions in the dialogue format. This behavior is consistent across the two KGs being tested. This shows the need for having a chatbot system that has the ability to engage in dialogues to help users explore different KGs.



% add other models and its citations
\subsection{LLMs}
{\sysName} provides the flexibility to test using different LLMs. We evaluated the ability of Llama-7b, Llama-13b\cite{llama2}, CodeLlama-7b, CodeLlama-13b\cite{codellama}, and Mistral-7b-v0.1\cite{mistral} models to perform the benchmark generation task within the {\sysName} pipeline. We evaluate the benchmarks generated by each model for the two KGS: Yago and DBLP.  We evaluate them on the quality of the generated question, the percentage of correctly generated SPARQL queries, and the number of seed nodes used due to different errors in the LLM output. 


%\input{tables/llm_quality}
The LLMs produce different quality of questions in dialogues. Llama-7b, CodeLlama-7b, and Mistral-7b-v0.1 tend to use the predicate as it is in the questions, while Llama-13b and CodeLlama-13b produce questions that seem to follow a certain template. {\color{red} Add more explanation after further evaluation}


As explained in \autoref{sec:subgraph_approach}, wrong query generation leads to discarding questions within the dialogue. \autoref{tab:llm_query} shows the percentage of correct SPARQL queries generated by each LLM for each Yago and DBLP KGs. Gpt-3.5 produced the best percentage in the two KGs. From the open-source LLMs, CodeLLama-13b has the best performance across openLLMs. CodeLLama-7b and Mistral-7b-v0.1 have comparable performance. Mistral-7b-v0.1 is the only LLM to maintain its percentage across the two KGs, it was not affected by the change in domain or length of the labels. LLama-7b and LLama-13b could not produce any dialogues for DBLP while having very low percentages for YAGO. 


As shown in \autoref{fig:framework}, each LLM-based component is associated with a validator to ensure the correctness of LLM output before moving forward in the pipeline. \autoref{tab:openllm} shows the different errors caught by the validators for different steps in the pipeline. The included errors are those that cause skipping of the current seed entity and replacing it with another one. openLLMs struggle with the first step of the pipeline due to its complexity. We designed an updated version of our pipeline that divides the first module into two tasks: \myNum{i} generating independent questions, and \myNum{ii} choosing the triple associated with each question. As shown in the second part of \autoref{tab:openllm}, the simplified pipeline enabled the LLMs to bypass the first module and move through the rest of the pipeline steps {\color{red} The only LLM benefiting from this is Llama-7b}. The bottleneck module for the considered LLMs is the SPARQL generation module. Some LLMs such as {\color{red} Add examples}, generate queries that use undefined Prefixes, that were not a part of the given triple. To mitigate this issue, we append a set of pre-defined prefixes to the generated query before executing it to test its correctness. Even with this change, only CodeLlama-13b has a reasonable performance for the SPARQL query generation leading to less number of overall skipped entities. 


\subsection{Ablation Analysis}
\input{tables/time}
% \input{tables/question_quality}
In this experiment, we test the effectiveness of the entity representation module, which is responsible for choosing a human-readable representation of the entity to be provided to the LLM within the subgraph.
We repeated the quality of questions and dialogues evaluation process while disabling this module (i.e., using only the last segment of the URI). The third column in \autoref{tab:quality} shows these results. The percentage of valid questions did not drop significantly, due to the effectiveness of the validation process.  On the other hand, the number of skipped nodes significantly increased, especially for YAGO and DBpedia where the number of skipped nodes is $195$ and $88$ respectively. These findings indicate that the entity representation module improved the quality of the generated questions and decreased the number of skipped nodes.



 

==> old_sections/introduction_june10.tex <==
\section{Introduction}
Conversational AI systems, including chatbots (e.g., ChatGPT\footnote{\url{https://openai.com/blog/chatgpt}} and Gemini\footnote{\url{https://gemini.google.com/}}) and virtual assistants (e.g., Alexa and Siri), aim to hold natural conversations with users on a wide range of topics. These conversations provide general information or enable users to complete specific tasks\cite{chatgpt_survey}. Although many users report positive experiences with conversational AI systems, there is a need for a systematic way to evaluate the quality of these interactions. This highlights the importance of dialogue benchmarks that can assess conversational AI systems' ability to understand user requests, leverage the full conversational context, and provide accurate and relevant responses. However, most of the existing dialogue benchmarks focus on information retrieval from documents such as Dream\cite{dream}, and MultiWOZ\cite{multioz}, neglecting the potential of Knowledge Graphs (KGs). KGs incorporate a vast amount of data in many specialized domains (e.g., medical or financial). This specialized data has the potential to significantly improve the performance of general virtual assistants\cite{p_assistant}. Dialogue benchmarks can be used to train chatbots capable of engaging in multi-turn conversations within a specific domain, extending beyond simple question-answering tasks. These benchmarks encourage applications like online tutoring\cite{tutoring} by creating educational exams and the development of educational chatbots\cite{edu_chatbot}. Furthermore, dialogue benchmarks can be used for various KG exploration tasks, such as onboarding new users to existing KGs\cite{AttnIO} and comparing information similarity between different KGs by analyzing the questions generated for each.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/example.pdf}
\caption{An illustration of the steps needed to create a dialogue from an entity belonging to DBpedia KG.}
\label{fig:example1}
\end{figure}

Automating dialogue benchmark generation on KGs presents unique challenges. KGs contain real-world entities interconnected by diverse relationships. Both entities and relationships are represented using Uniform Resource Identifiers (URIs). \autoref{fig:example1} outlines the steps involved in generating a dialogue from a KG, each associated with a specific challenge: \myNum{1} \textbf{Sample Entities}: The first step involves sampling entities from the KG. KGs contain a vast number of entities, making it impractical to incorporate all of them into generated benchmarks. Therefore, selecting a representative sample of entities spanning various important KG node types becomes crucial. \myNum{2} \textbf{Extract Context:} The second step involves extracting subgraphs surrounding the chosen entity. These subgraphs represent the context of the dialogue. \myNum{3} \textbf{Represent Entities:} To generate a question about an entity, we need a human-readable representation for it. Using URIs within natural language questions is impractical, necessitating a more user-friendly representation. \myNum{4} \textbf{Maintain Dialogue Flow:} The generated questions should remain relevant and build upon each other within the dialogue. The primary topic can be explicitly introduced once, with subsequent questions referring to it indirectly. \myNum{5}\textbf{ Generate Answers:} Generating complete benchmarks requires answers for each question. Within the context of KGs, retrieving answers involves utilizing SPARQL queries. This necessitates formulating SPARQL representations corresponding to each question generated. \myNum{6} \textbf{KG Agnostic Design:} The dialogue generation platform should be able to operate on any KG without requiring KG-specific modifications.
\input{tables/background_v2}
Existing dialogue benchmarks on documents, such as CoQA\cite{coqa} and QuAC\cite{quac}, rely on manually generated questions and answers. Single-question benchmarks for KGs face similar limitations. While QALD-9\cite{qald9} utilizes manual question creation, others like LCQuAD\cite{lcquad, lcquad2} and Head-to-Tail\cite{head_to_tail} employ templates. Template-based approaches struggle with arbitrary KGs, requiring redesign of templates for each new KG. Head-to-Tail chooses entities based solely on node popularity, without taking entity types in consideration. CSQA\cite{csqa}  a semi-automatic dialogue benchmark for the Wikidata KG, continues to be labor-intensive and KG-dependent. This is because it requires manually designed templates to identify interconnected predicates within the KG. Maestro\cite{maestro} is an automatic system for single-question benchmark generation on KGs. However, it requires a pre-processing step to extract the required entities from the KG, which can be time-consuming. Furthermore, Maestro does not offer a diverse range of node types, potentially depending on rare types. Furthermore, it utilizes predefined question shapes that might not be present in all KGs which can lead to generating complex questions.  To choose the suitable entity representation in the question, Maestro requires users to provide how to extract this representation. This limits its adaptability to run with arbitrary KG. Both Maestro and other template-based benchmarks, such as LCQuAD, require prior knowledge of the answer to generate questions. This hinders their application for dialogue generation, since the answer is the topic for which we need to generate the question. This way all generated questions will share the same answer. 

To address these limitations, we propose {\sysName}, a novel platform that automatically generates dialogue benchmarks on arbitrary KGs. {\sysName} leverages Large Language Models (LLMs) across its stages. It predicts human-readable entity representations based on their types, resulting in more understandable questions. When selecting dialogue context (entities), {\sysName} considers the distribution of node types within the KG. To maintain a consistent context throughout the dialogue, {\sysName} relies on condensed subgraph shapes. Furthermore, by efficiently encoding the subgraph in a summarized way, {\sysName} can leverage richer subgraphs to generate more comprehensive dialogues. {\sysName} generates queries for each question without requiring prior knowledge of the answer.

We evaluate {\sysName}'s performance on three diverse real-world KGs: DBpedia, Yago, and DBLP. Our experiments demonstrate that {\sysName} successfully generates high-quality questions with clear entities' representation. Moreover, the generated questions exhibit a diverse entity type distribution, including most KG node types. {\sysName} produces a wide variety of question types, enabling it to effectively challenge chatbot systems. Furthermore, {\sysName} demonstrates efficient time performance in end-to-end benchmark generation compared to existing systems. Finally, we explore {\sysName}'s compatibility with different LLMs by evaluating its performance with both commercial models such as OpenAI models and open-source models. This flexibility empowers users to work on various KGs and leverage different LLMs. 
Our key contributions are:
\begin{itemize}
\item Introducing the first platform for automatically generating dialogue benchmarks from KGs based on LLMs; Section 3.
\item Effective and diverse context retrieval method for selecting representative seed nodes with rich subgraphs from the KG with minimal overhead; Section 4.
\item Carefully designed multi-step dialogue generation workflow with automatic assertion-based validation, and adopted the workflow with LLMs of different capabilities; Section 5. 
\item A comprehensive evaluation using three real KGs from different domains, and different LLMs. {\sysName} can work with arbitrary KGs in timely performance regardless of the size of the KG; Section 6. 
\end{itemize}

==> old_sections/introduction_march22.tex <==
\section{Introduction}
Humans' ability to gather information and interact effectively stems from their capacity to engage in conversations. This has driven the development of dialogue benchmarks, aiming to train machines to answer conversational questions.
There has been a rapid rise of large language models (LLMs), from BERT\cite{bert} and T5\cite{T5} to Instruct GPT\cite{instructgpt}, GPT-4\cite{gpt4} and LLAMA-2\cite{llama2}. This advancement has motivated the development of chatbot systems like ChatGPT \footnote{\url{https://openai.com/blog/chatgpt}}. Chatbots offer users a human-like conversational experience. They are capable of handling individual questions, and dialogues. They allow users to ask clarifying follow-up questions for a more satisfying user experience.
While LLMs have positively impacted many Natural Language Processing (NLP) tasks, they come with limitations. One key challenge is that LLMs can only answer questions based on the data they were trained on\cite{graphqa}. Incorporating recent or updated information can be a slow process\cite{chatgpt_survey}. When asked about unknown information, some LLMs might generate incorrect responses or resort to ``hallucination'', providing seemingly reasonable but false or misleading answers\cite{hallucinate}. Some LLMs can indicate their inability to answer a question. Hallucinations can occur due to multiple reasons, e.g. relying on unstructured data \cite{graphqa} and the rare presence of information in the training data \cite{hallucinate}. Other ways of hallucinations can be mitigated by proposing different architectures or algorithms\cite{hallucinate}. Hallucination remains a significant barrier to LLM's usability within systems, That’s why LLM-based systems need to overcome it.
Using knowledge graphs could overcome these limitations. KGs contain the most recent information \cite{chatgpt_survey}\cite{head_to_tail} due to their frequent updates which are valuable for overcoming the lack of information in the LLM's training data especially for the domain-specific and private data. The structured nature of the KGs can decrease the hallucinations introduced by relying on the unstructured data.

Information extraction from LLMs poses another challenge.  Prompting is a technique that instructs LLMs to perform different tasks instead of the time-consuming fine-tuning process. It produces promising results in tasks like entity deduction\cite{entity_deduction} and instruction generation\cite{prompt_engineer}. However, prompt design is challenging, it requires extensive trial and error\cite{prompt_nonexpert}. Minor modifications in the prompts can lead LLMs to generate different outputs, which can be wrong.

Although merging the benefits of LLMs and KGs is promising, it is still under-studied. We explore the potential of merging them to create benchmarks for dialogue systems for KGs. Knowledge graph question answering (KGQA) aims to convert natural language questions into formal queries that can retrieve answers from the knowledge graph. This approach is driven by the vast number of available KGs in various domains, such as DBpedia\cite{dbpedia}, Wikidata\cite{wikidata}, DBLP, and Microsoft Academic. These KGs store a huge amount of factual data. Existing KGQA benchmarks motivated the development of KGQA systems like KGQAn\cite{kgqan} and EDGQA\cite{EDGQA}. These systems focus on answering single questions and are unsuitable for real-world conversational scenarios.
\input{tables/background}
Benchmarks play a crucial role in driving AI research for specific tasks. For KG chatbots, dedicated benchmarks, and systematic evaluation criteria are essential to motivate further exploration. Current benchmarks either cover a limited number of KGs or do not deal with KGs. We categorize these benchmarks into three groups: \myNum{i} Conversational benchmarks on documents such as CoQA\cite{coqa} and QuAC\cite{quac}, which are manually created and do not deal with KGs. \myNum{ii} Benchmarks for KGQA, designed for KGQA tasks like QALD\cite{qald9} and LCQuAD\cite{lcquad, lcquad2}. They do not support conversations and cannot be easily adapted for conversational scenarios as each question targets independent entities or information that cannot be grouped. Recent advancements have led to the creation of semi-automatically generated benchmarks for KGs, such as Head to Tail\cite{head_to_tail} and automatic benchmark generation tools such as Maestro\cite{maestro}. While these approaches require less manual effort compared to fully human-created benchmarks (through the design of rules or templates), they still involve human intervention, limiting scalability. \myNum{iii} Semi-automated conversational benchmarks on KG such as CSQA\cite{csqa}. CSQA is the closest to our work. However, it focuses on specific versions of Wikidata KGs and cannot be automatically adapted to handle arbitrary KGs. Because it requires exploration of all predicates within the KG and subsequent manual steps. Although it is  semi-automated, this approach remains labor-intensive

Conversational chatbots built upon knowledge graphs represent a promising direction. They combine the strengths of LLM-based chatbots(conversational ability) and KGQA systems(fact retrieval) to overcome their shortcomings and deliver a better user experience. These systems have the potential to enhance current chatbots and personal assistants. It also improves upon existing KGQA systems by adding conversational capabilities, making it easier for users to retrieve information from the KG and enhancing overall understanding abilities.

Benchmarks for KG chatbots consist of a set of dialogues.  Each dialogue consists of a list of questions and their corresponding SPARQL query. A dialogue is a multi-turn, one-to-one conversation representing a subgraph within the KG. All questions are answerable from the subgraph, and answering them requires reasoning based on the conversation history. We propose a framework that automatically generates conversational benchmarks for any KG using foundation models. This automatic generation makes it easier to adopt new KGs covering different application domains. Unlike document-based benchmarks where choosing relevant passages is challenging, our approach focuses on selecting representative subgraphs from the given KG. Foundation models eliminate the need for manually creating rules or templates. The approach operates in a sequential, multistep fashion.  The framework first chooses target entities. Then respective subgraphs are extracted based on the chosen entities. Next, independent questions are generated as an intermediate stage. These questions are then used to generate the corresponding SPARQL queries and the final dialogues.

Our contributions can be summarized as follows:
\begin{enumerate}
    \item To our knowledge, this is the first framework for generating conversational benchmarks for KGs.  Our generated benchmarks test the ability of question-answering systems to understand the given question within context (if needed) and retrieve the required data from the KG
    \item Introducing systematic evaluation criteria to assess the performance of KG chatbots. 
\end{enumerate}






==> old_sections/introduction_march27.tex <==
\section{Introduction}
Dialogue systems \cite{unids}\cite{ptod} and chatbots such as ChatGPT \footnote{\url{https://openai.com/blog/chatgpt}}, and Gemini \footnote{\url{https://gemini.google.com/}} are becoming increasingly important. They aim to hold natural conversations with users on various topics. However, existing dialogue benchmarks primarily focus on information retrieval from documents, neglecting the potential of Knowledge Graphs (KGs). Automatically generating dialogue benchmarks on KGs offers promising directions for building personal assistants on specialized KGs \cite{p_assistant} (e.g., for medical staff or data scientists) and training chatbots that can engage in multi-turn conversations within a specific knowledge domain. Such benchmarks extend beyond simple question-answering benchmarks. These benchmarks encourage applications like online tutoring \cite{tutoring} by creating educational exams and developing educational chatbots \cite{edu_chatbot}. Furthermore, they can be used for various KG exploration tasks such as onboarding new users with existing KGs, and comparing information similarity between different KGs by comparing the questions generated on them.

Creating such benchmarks on KGs presents unique challenges. KGs represent real-world entities interconnected by diverse relationships. Both entities and relationships are represented using Uniform Resource Identifiers (URIs). However, using URIs within natural language questions is impractical and user-unfriendly, necessitating a more human-readable entity representation. Additionally, KGs contain millions of facts, making it impossible to incorporate all of them into generated benchmarks. Selecting a representative sample of entities belonging to various important KG types is crucial. Furthermore, extracting relevant subgraphs surrounding each entity is vital, as these subgraphs provide context for the dialogue. Finally, generating high-quality benchmarks requires answers for each question. In the context of KGs, answers can be retrieved using SPARQL queries, necessitating the creation of SPARQL representations for each generated question.

A key challenge lies in ensuring that generated questions are relevant and interconnected within the dialogue. The topic of the dialogue should be explicitly introduced only once, with subsequent questions referring to it implicitly. Another challenge is achieving KG independence, ensuring the framework can operate on any KG without requiring KG-specific modifications.

While several benchmarks and benchmark creation systems currently exist, none address the automatic generation of dialogue benchmarks specifically for KGs. In dialogue benchmarks on documents such as CoQA\cite{coqa} and QuAC\cite{quac}, both questions and answers are manually generated. Single questions benchmark on KGs, are either created manually such as QALD-9\cite{qald9}, or using templates such as LCQuAD\cite{lcquad, lcquad2} and Head-to-Tail\cite{head_to_tail}. Template-based solutions do not work with arbitrary KGs, since templates need to be re-designed when working with new KGs.  Head-to-Tail produces single questions for independent entities that were sampled based on the popularity of the nodes, regardless of their types. CSQA\cite{csqa}, a semi-automatically created dialogue benchmark on Wikidata KG, remains labor-intensive and KG-dependent. As it relies on manually designed templates for interconnected predicates. Although Maestro\cite{maestro} is an automatic single-question benchmark generation system, it requires time-consuming pre-processing to extract the required entities from the KG. It may not provide diverse node types, sometimes relying on rare types. Additionally, Maestro relies on its pre-defined shapes that may not exist in the KG and generates complex questions. To choose the suitable entity representation in the question, the users need to provide how to extract this representation per KG, which limits its running with arbitrary KG. Maestro and other template-based benchmarks e.g. Head-to-Tail and LCQuAD necessitate prior knowledge of the answer before generating questions.

\input{tables/background}

To address these limitations, we propose {\sysName}, a novel platform for automatically generating dialogue benchmarks on KGs, which can work on arbitrary KGs. {\sysName}  leverages Large Language Models (LLMs) in different stages of the platform.  {\sysName}  effectively predicts human-readable entity representations based on their types, leading to more understandable questions. It considers the distribution of node types within the KG when selecting the dialogues’ topics (entities). {\sysName}  relies on condensed subgraph shapes to maintain a single topic throughout the dialogue. Importantly, {\sysName}  generates queries for each question without requiring pre-existing knowledge of the answer.

We evaluate {\sysName} on three distinct real-world KGs: DBpedia, Yago, and DBLP. Our experiments demonstrate that {\sysName} successfully generates high-quality questions with clear entity representations. Additionally, we show a diverse entity distribution, including most KG node types. {\sysName} generates a wide variety of question types that can challenge KG chatbot systems. Finally, {\sysName} displays efficient time performance for end-to-end benchmark generation compared to existing systems. {\sysName} empowers users with the flexibility to work on various KGs and leverage different LLMs. In summary, our contributions include:
\begin{itemize}
\item Introducing the first automatic dialogue benchmark generation framework for KGs.
\item An effective seed node selection and subgraph extraction approach that focuses on extracting nodes and graphs suitable for generating meaningful dialogue.
\item Implementing an automatic entity representation extraction module utilizing LLMs, which significantly improves the quality of generated questions.
\item A comprehensive evaluation using three real-world KGs from diverse domains.
\end{itemize}


==> old_sections/overview_june4.tex <==
 \section{The {\sysName} Platform Overview}
%\section{Benchmark Overview}

% \subsection{Definitions}
A conversational benchmark for KGs is a collection of dialogues, where each dialogue consists of independent and dependent questions and corresponding SPARQL queries.

\begin{definition}[Independent Question]
\label{def:independent}
An independent question $(Q_{In})$ is a question that can be answered directly from the KG without requiring any additional context. All information needed to retrieve the answer is present within the question itself.
\end{definition}

\begin{definition}[Dependent Question]
\label{def:dependent}
A dependent question $(Q_{Dep})$ is a question that cannot be answered solely based on the KG. It requires an associated context $(C)$ to provide the necessary information for retrieving the answer from the KG.
\end{definition}

\begin{definition}[Dialogue]
A Dialogue $D(e) = \{e, Q, SQ\}$ where:
\begin{itemize}
    \item Seed Entity $e$: The topic the dialogue revolves around
    \item Questions $Q$: An ordered list of questions asked during the dialogue, denoted as $Q = [Q_1, Q_2, . . . , Q_n]$ such that The first question $Q_1$ must always be an independent question ($Q_{In}$). Subsequent questions ($Q_i$ where $i > 1$) must be dependent $(Q_{Dep})$, depending on the dialogue flow.
    \item SPARQL Queries ($SQ$): A list of SPARQL queries corresponding to each question in $Q$
\end{itemize}
\end{definition}


\subsection{An Overview of {\sysName}}

This section presents an overview of our fully automated conversational benchmark generation framework for KGs. Our framework requires no human intervention and can operate on any arbitrary KG.
As shown in Figure \ref{fig:framework}, the framework begins by selecting $m$ nodes, where $m$ represents the required number of dialogues. The nodes follow the overall distribution of node types within the KG. 
% Nodes with high connectivity are prioritized, as this facilitates the generation of richer dialogues. 
Based on these chosen seed entities, the corresponding subgraph is extracted from the KG.

Next, the framework employs several foundation model tasks. The independent question generation module takes the extracted subgraph as input and generates a set of independent questions about facts contained within it.  Each generated question is directly associated with the specific triples used to create it. The SPARQL query generation module utilizes a given question and its associated triples to create a SPARQL query that retrieves the answer to the question. A separate validator module ensures the generated query is syntactically correct and successfully retrieves the correct answer. Finally, the list of independent questions is fed to the dialogue generator module. This module processes the questions and transforms them into a dialogue.

The final benchmark dataset consists of three components: conversational questions, independent questions, and corresponding SPARQL queries. The conversational and independent questions inquire about existing KG facts related to the seed entities. The corresponding SPARQL queries, efficiently retrieve the answers from the target KG.

\subsection{Benchmark Characteristics}
Developing effective conversational benchmarks for knowledge graph (KG) chatbots requires consideration of several key characteristics. These characteristics evaluate various aspects of the chatbot's performance.

\subsubsection{Coverage of Different Question Types:} The benchmark should include questions that vary in complexity to test the chatbot's ability to handle different questions. This means assessing the chatbot's understanding of the question and its proficiency in retrieving accurate information from the KG. Question complexity is defined by its linguistic nature. Examples of different categories include count questions, listing questions, and WH questions. Each type requires a distinct approach from the chatbot. For example, listing questions demands returning all relevant answers, while count questions only require the number of answers.

\subsubsection{Grounded Facts:} To evaluate the chatbot's accuracy, the answers to the questions must exist within the target KG. This ensures that the chatbot is leveraging the KG effectively and not generating irrelevant information.

\subsubsection{Diversity of Nodes:} A diverse benchmark assesses the chatbot's flexibility in handling different KG nodes, preventing bias towards specific node types or structures. Ideally, the benchmark would include all nodes in the KG. However, since this is impractical, we need a sampling approach. The sampled nodes should accurately represent the entire graph, including various node types, and simulate their distribution within the original KG. This approach ensures the chatbot's ability to respond effectively to questions about different nodes within the knowledge graph.

\subsubsection{Linguistic and Grammatical Correctness:} Language correctness in the benchmark is vital for ensuring a fair and accurate assessment of KG chatbots. Testing chatbots with incorrect language is not beneficial because it hinders objective evaluation.

By incorporating these essential characteristics, conversational benchmarks for KG chatbots can provide a comprehensive and reliable evaluation of their capabilities. This allows for objective comparisons and facilitates further development in this field.


==> old_sections/related_workMay28.tex <==
\section{Related Work}
\input{tables/llm_query}
% \input{tables/open_llm}
% \input{tables/open_llm_v2}
% \input{tables/open_llm_v3}
% \input{tables/open_llm_v4}
% \input{tables/open_llm_v5}
\input{tables/open_llm_v6}
% \input{tables/open_llm_prompt_updated}
\input{tables/open_llm_may12}

\subsection{Document Based Dialogue Benchmarks}
Among the early efforts in this field are CoQA\cite{coqa} and QuAC\cite{quac} datasets. They are designed for the Machine Reading Comprehension Task (MRC) where answers to the given questions are extracted from a given passage.

CoQA dataset encourages the creation of conversational question-answering systems that perform well across different domains. It is the first large-scale MRC dataset where questions depend on dialogue history. CoQA’s target is to ensure the naturalness of answers\cite{coqa}. It introduces challenges absent in existing MRC datasets, such as coreference resolution and reasoning over conversation history. Questions are categorized as independent or dependent on the dialogue history. The dialogues are multi-turn, each turn consists of question-answer pairs. The answers are free-form, and their evidence is highlighted in the passage. The average conversation length is $15$ turns \cite{coqa}. The benchmark's manual creation involves pairing two workers (questioner and answerer) for each chosen passage, covering seven distinct domains. The final benchmark consists of $8k$ conversations.

QuAC is another example of document-based conversational benchmarks. QuAC is manually constructed through a discussion between two workers about a specific topic. The questioner has limited knowledge, knowing only the topic name and the first paragraph of an article. The answerer has access to the entire article. QuAC's distinction lies in its context-specific questions. The questions are meaningful only within the dialogue scope. They define a dialogue as a multi-turn question-answer pairs. The workers keep discussing until specific conditions are met, e.g., reaching $12$ answered questions. The final benchmark contains $14k$ conversations.



\subsection{Existing KGQA Benchmarks}
The growing interest in knowledge graph question answering systems has led to the development of several benchmark datasets on various KGs such as QALD\cite{qald9}, LCQUAD\cite{lcquad, lcquad2} on DBpedia\cite{dbpedia} KG, DBLP-QuAD \cite{dblpquad} on DBLP KG  and WEBQUESTIONSSP \cite{webquestions} on Freebase KG. These benchmarks offer standardized evaluations for comparing the performance of different question answering systems. Here, we will explore some prominent examples:

QALD is developed from DBpedia version $2016-10$, QALD is a manually generated dataset consisting of $408$ training questions and $150$ testing questions. It was created by compiling and curating previous versions of the dataset. It supports multilingual question answering, being available in $11$ languages.

LCQuAD 1.0 was derived from DBpedia KG version $2016-04$ and contains $4,000$ training questions and $1,000$ testing questions. It was designed to address the limitations of small size and limited complexity found in earlier benchmarks. LCQuAD incorporates questions of varying complexities, including those translatable to a single RDF triple and those translatable to multiple triples. Unlike previous benchmarks, LCQuAD employs a semi-automated generation process. This involves selecting a seed entity and relevant predicate lists from the knowledge graph. Subsequently, a subgraph is generated using nodes within two hops of the seed node. To create SPARQL queries and English questions, template pairs (SPARQL template, normalized natural language question template) are manually designed. Finally, the SPARQL queries and English questions are generated using the subgraph triples and the templates. To guarantee the quality of the questions, two human-dependent steps are performed. The first correct and rephrase questions as needed, and the second performs a final review of the question’s quality.

LCQuAD 2.0 builds upon the first version by expanding the dataset size to $30,000$ question-query pairs and extending its target KGs to include both Wikidata and DBpedia version $2018$. The generation process largely resembles that of LCQuAD 1.0, with the key differences being: \myNum{i} the use of Wikidata entities, \myNum{ii} the creation of SPARQL templates compatible with both Wikidata and DBpedia endpoints, and \myNum{iii} the utilization of Amazon Mechanical Turk for generating the final natural language questions.

DBLP-QuAD\cite{dblpquad} is developed on the DBLP scholarly knowledge graph, It consists of $10,000$ question-answer pairs. It adopts a template-based generation process, involving a manual step for creating templates followed by an automated step for generating questions from those templates. The templates are designed based on an analysis of the DBLP KG's ontology. They consist of SPARQL query templates and their corresponding natural language question templates. To ensure quality, the question template creation process involves two authors, one for initial creation and another for verification. Random nodes are chosen from the KG, and the subgraph within two hops is extracted. Finally, the question-query pairs are automatically generated by filling the template placeholders with the corresponding values from the subgraph.



The Head-to-Tail benchmark, introduced in \cite{head_to_tail}, was designed to evaluate the performance of LLMs on factual information stored in KGs. However, it can also be applied to assess question-answering systems on KGs. The benchmark comprises $18k$ question-answer pairs spanning diverse domains and entities of varying popularity.
The questions within the benchmark are generated using a template-based approach, where each question targets specific attributes of an entity. Templates are manually created for each entity, considering different attributes. For some KGs, the authors initially leveraged LLMs to draft the templates, followed by manual refinement. The answer to each question is the entity's attribute value, representing the object in the relevant triple in the KG. The authors categorized the entities into three groups based on popularity, ensuring an equal number of questions were generated from each group.



==> sections/background-reham.tex <==
\section{Background and Limitations}
\subsection{Dialogue Benchmarks for KGs}
The process of automatically generating conversational benchmarks for Knowledge Graphs (KGs) can be  divided into four main steps: \textit{\myNum{1} Context Extraction:} selects a set of entities representing different types within the target KG. These entities will serve as dialogue topics. Then, extract subgraphs surrounding these entities. These subgraphs must contain sufficient facts to create a conversation. \textit{ \myNum{2} Textual Entity Representation:} In KGs, entities are represented using URIs that lack natural language context and are not user-friendly.  A textual representation of these entities is crucial for generating meaningful questions related to a specific entity. \textit{\myNum{3} Dialogue Generation:} Using the extracted context and entity representations, generate a set of relevant and interconnected conversational questions that ask about facts within the given subgraph. The dialogues can be directly generated, or the process can be divided into two sub-steps: generating individual questions, then connecting them to form a dialogue. \textit{\myNum{4} Answer Generation:} Extracts the answer to each generated question from the KG. The answer can be an entity or a literal value. Since we are dealing with KGs, this step involves generating SPARQL queries.  In addition to explaining these steps, we will discuss the ability of existing systems to work with an arbitrary KG.

There are no existing systems that automatically generate conversational benchmarks for KGs.  CoQA\cite{coqa} and QuAC\cite{quac} are well-known benchmarks for conversational question answering on documents. CSQA\cite{csqa} is a semi-automatically generated conversational benchmark for the Wikidata KG. Head-to-Tail\cite{head_to_tail} utilizes templates to create benchmarks for single questions on KGs. Maestro\cite{maestro} is an automatic framework for generating single-question benchmarks for KGs. \autoref{tab:back} compares these benchmarks and systems.

\textbf{CoQA} and \textbf{QuAC} are manually generated, with slight variations in settings and answer formats. Their manual creation hinders their use with different data sources, like KGs.  Since they focus on documents, context extraction involves selecting passages from the source documents. Entity sampling and representation steps are not applicable because entities are embedded in the extracted passages and exist in a human-readable format.

\textbf{CSQA} supports only the Wikidata KG and utilizes a predicate-centric approach for the benchmark generation. CSQA starts by extracting all $330$ Wikidata predicates with their connected subjects and objects. They are stored as subject-predicate-object triples for further processing. Question generation within CSQA is a manual process that first creates independent questions. Workers formulate questions using the provided subject-predicate-object triples. Questions are formed using either the predicate and subject (with the object as the answer) or vice versa. Then to convert the questions to a conversation, CSQA uses pre-designed templates. In-house annotators design these templates, which consist of connected question-answer pairs sharing a relation or entity. Finally, workers manually modify the generated conversations to introduce complexities, such as coreferences, ellipsis, incompleteness, and contextual dependence. Supporting new KGs with CSQA is labor-intensive. Users need to manually extract predicates, generate independent questions and answers, define connected question-answer pairs, and design templates to transform question sets into dialogues.

\textbf{Head-to-Tail} does not support dialogues, it generates single questions based on templates. It starts its context extraction by employing a popularity based approach for entity selection. Entities are first sorted by popularity and then divided into three categories. However, during sampling, node types are not considered; nodes are randomly chosen from each category. Head-to-Tail focuses on the attributes surrounding the sampled entity. Question generation relies on manually created templates for each attribute surrounding the entity. This approach becomes impractical for KGs with many node types, as users would need to define a vast number of templates for various attribute-node type combinations. Generated questions focus on entity attributes. Grouping them creates a conversation, but it leads to repetitive dialogues for entities of the same type due to the use of templates. Head-to-Tail does not require a separate answer generation step, as the answer to each question is the object of the triple used to create the question template. Although Head-to-Tail considers multiple KGs, supporting a new KG necessitates manually designing a big number of templates to cover all attributes across all node types within that KG.

\textbf{Maestro} performs a pre-processing step before the main process begins. In this stage, Maestro extracts predicates, their labels, connected entity types, and KG examples storing them in a predicate lexicon table. Pre-processing time is proportional to the number of classes in the KG ontology. To extract context, Maestro samples entities belonging to node types existing in the predicate lexicon table. Depending on the desired benchmark size, a subset of this table is chosen, as including all KG nodes within a benchmark is impractical.  However, this subset does not include all important node types. Then, Maestro defines various subgraph shapes around the extracted entities and creates corresponding SPARQL templates. These shapes act as the context surrounding the chosen entity. Some shapes, such as tree and cycle, generate complex questions unsuitable for a conversation. Maestro offers flexibility in entity representation by allowing users to specify the predicate for extracting the appropriate representation. However, this approach assumes a single predicate can be applied to all node types, which isn't always true in KGs.  For instance, different predicates might represent distinct node types, such as \textit{"name"} for \textit{Person} entities and \textit{"title"} for \textit{Publication} entities. Question generation within Maestro is a rule-based process. Each shape has a corresponding natural language template used to generate questions from the subgraph. However, a subsequent transformation step modifies some questions (e.g., converting them to count or boolean questions). This final step exhibits a bias towards boolean questions, leading to a high percentage of such questions within the generated benchmarks. This contrasts with human dialogues, where most questions are open-ended, seeking information or clarification. Questions generated by Maestro cannot be grouped into a dialogue because all questions for a seed entity share the same answer (the entity itself). Maestro works on multiple KGs, however, its support is not user-friendly. Adding support for a new KG necessitates writing three classes totaling around $600$ lines of code, posing a significant challenge for non-technical users.

\subsection{Prompting and Large Language Models}
Large language models (LLMs) have significantly enhanced the performance of various natural language processing (NLP) tasks. However, these models have limitations. LLMs are limited by the data they are trained on\cite{graphqa}. This means they cannot answer questions or engage in conversations about domain-specific information not included in their training data. Additionally, incorporating recent updates can be a slow process\cite{chatgpt_survey}, hindering their ability to stay up-to-date. Another limitation is the context window length, which refers to the amount of text an LLM can process. While recent models like LLaMA3\footnote{\url{https://llama.meta.com/llama3/}} provide extended context window lengths (up to $32k$ tokens), LLMs still face challenges in incorporating recent information and acquiring domain-specific knowledge.

One of the most critical limitations of LLMs is hallucination\cite{hallucinate}. This occurs when LLMs generate outputs that deviate from the given prompt\cite{hallucinate}. LLMs can provide seemingly reasonable but factually incorrect answers\cite{hallucinate}. They can generate completely invented responses for information outside their training data. Hallucination has multiple root causes, including the unstructured nature of the training data \cite{graphqa}, and  rare occurrences of certain information in the training data\cite{hallucinate}. Overcoming hallucinations is crucial for ensuring the reliability and usability of LLM-based systems. Examples of LLM hallucination for dialogue generation from KG includes: (1) ambiguous dialogues: LLM generates a dialogue where the first question does not state the context, e.g. What is his nationality?. (2) Non-existing facts: LLM generates questions that do not map to facts (triples) in the subgraph. (3) wrong SPARQL: LLM generates SPARQL queries that do not correspond to the questions being asked, for example using a predicate not in the triple used for question generation.

Adapting LLMs to new tasks can be achieved through various methods. Fine-tuning involves training only a small portion of the LLM on a domain or task-specific dataset. This technique was common for earlier language models like BERT\cite{bert} and T5\cite{T5}. However, fine-tuning, even for these small models, requires significant computational resources. With the recent surge in LLM size, such as GPT-4\cite{gpt4}, LLAMA\cite{llama}, and PALM\cite{palm}, fine-tuning becomes increasingly expensive due to computational demands. Additionally, it needs to be repeated for each new task or domain. This has led to the emergence of prompting as a more efficient technique\cite{prompt_survey}. Prompting, also known as in-context learning\cite{gpt3}, instructs the LLM to perform a specific task by providing an explanation. This explanation can take different forms. In few-shot learning, users provide both input and output examples for the LLM to learn from. In zero-shot learning, users provide only a prompt, without any examples.

While prompting has become the dominant method for interacting with LLMs, these models remain highly sensitive to the prompts. Minor changes in a prompt can significantly change the output\cite{prompt_change}. Several prompting techniques have been developed to enhance LLM performance. \myNum{1} \textbf{Chain-of-thought (CoT)}\cite{cot}  aims to improve LLM reasoning by guiding the model through the problem-solving process. This technique involves including intermediate reasoning steps within the prompt itself.  \myNum{2} \textbf{Zero-shot CoT}\cite{zeroshot_cot} offers a variant of CoT that doesn't require step-by-step examples. Instead, \textit{Let’s think step-by-step} sentence is appended to the end of the prompt. It employs a two-prompt approach: the first prompt tasks the LLM with extracting the reasoning, while the second prompt provides both the question and the extracted reasoning for the LLM to solve the task. \myNum{3} \textbf{Least-to-most prompting}\cite{least_to_most} tackles tasks requiring generalization, where the task is more complex than the examples provided in the prompt. This process involves two steps: first, it prompts the LLM to break down the task into simpler subtasks. Then, the LLM is instructed to solve these subtasks sequentially until the desired output is achieved. Although this technique outperforms CoT for certain tasks like math reasoning\cite{least_to_most}, it can be more expensive and prone to error propagation in tasks like text-to-SQL\cite{text_sql_cot}. This highlights the ongoing exploration to identify the most effective prompting technique for different tasks. \myNum{4} \textbf{Automatic prompting engineering}\cite{APE} seeks to reduce human effort and the need for extensive prompt testing. This approach automatically generates and selects prompts\cite{APE}. Given a sample of input and output, an LLM generates various instructions. Each instruction is evaluated on a subset of the data and assigned a score. This process iterates until convergence based on the generated scores. 

While these prompting techniques achieve significant success, they are not ideally suited for dialogue generation from KGs. Unlike the well-defined reasoning steps found in math problems, for instance, the KG dialogue generation reasoning is not as clear. Additionally, these techniques are limited to single outputs, hindering their ability to generate the complex output required for KG dialogue tasks which consist of the dialogue and SPARQL queries generating the answers. Therefore, there is a need for a cost-effective prompting technique that overcomes hallucinations and produces complex outputs.


\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/Architecture - 2 - labeled.pdf}
\caption{{\sysName}’s architecture includes two main phases: A) Context Extraction: all node types from the KG are extracted with a predicate for each node type to retrieve the textual representation of nodes  of this type. Then seed entities and their surrounding subgraph are extracted to represent the context of the dialogue, B) Dialogue Generation: The generation process is divided into three LLM-based steps, generating independent questions and associating them to triples used in their generation, utilizing question and triple to generate SPARQL queries, and transforming the independent questions into a dialogue.}
\label{fig:framework}
\end{figure*}











==> sections/benchmark_generation.tex <==
% \section{The Benchmark Generation}
% \section{The {\sysName} Platform}
\section{{\sysName} Platform}

% This section explains how the various modules of the platform interact to generate the final benchmarks using the provided KG and the number of dialogues $m$. 





==> sections/context_extraction-reham.tex <==
\section{Dialogue Context Extraction as Subgraphs}

{\sysName} aims to extract a representative set of entities that comprehensively cover different concepts of the KG. Subgraphs surrounding these entities are then extracted to capture the dialogue context, which will be used in subsequent steps to generate dialogues. The subgraph of a given seed entity is defined as follows:

\begin{definition}
% [Subgraph $SG$]
\label{def:subgraph}
Given a $KG$ containing a set of vertices $V$, and a set of relations $R$. Let $e$ be the target seed entity. The subgraph $SG(e) = \{T\}$ is a set of triples, where $T = \langle s, p, o \rangle$, such that $s= e$ or $o = e$.\shorten      
\end{definition}



A typical brute-force solution involves initially extracting all entities from the KG in a preprocessing step. A subset of these entities is then chosen based on specific criteria, such as the entity's degree (number of incoming and outgoing predicates) or the types of surrounding nodes. Subgraphs are subsequently extracted for each selected entity. This brute-force approach suffers from significant limitations in terms of time and space complexity. Retrieving all entities is computationally expensive, and storing them for later sampling incurs a linear space complexity relative to the number of entities, which can be in the billions, making this solution impractical for large KGs.\shorten

To efficiently extract context for dialogue generation, our approach leverages node type information within the KG through a three-step process: \myNum{i} relevant node type selection, \myNum{ii} textual entity representation, and \myNum{iii} seed node and subgraph extraction. 
The first step focuses on identifying relevant node types within the KG. These node types represent the different concepts, e.g., people, locations represented in the KG. 
Subsequent steps leverage the node type information to extract entities’ textual representation and sample a representative set of entities for subgraph extraction and dialogue generation. This approach works efficiently with large KGs. It eliminates the need for the expensive pre-processing that traverses the whole graph and stores the entities.

% \subsection{Node Types Selection}
\subsection{Identifying Representative Node Types}
\label{sec:seed}

In a KG, real-world entities are classified into types based on their shared characteristics. These characteristics include properties that describe the entities, and relationships that represent how entities interact. Within a KG, there are multiple types. Our dialogue generation process begins by identifying representative node types. For each node type, we then identify suitable seed entities.\shorten

We can categorize these types into two groups: domain-specific and metadata types. Domain-specific types reflect the core information and entities within a KG. They are the most important for dialogue generation on the KG. Examples include \url{https://dblp.org/rdf/schema#Publication} in the DBLP academic graph. Metadata types do not represent entities, they describe properties of the data within the KG such as \url{http://www.w3.org/2002/07/owl#DatatypeProperty}, as well as RDF engine-specific types like \url{http://www.openlinksw.com/schemas/virtrdf#array-of-string}. Because metadata types do not represent core KG entities, they are less useful for generating dialogues. Within domain-specific types, there are additional considerations for dialogue generation. Rare types are highly specific types with a very low percentage of entities within the KG, indicating they are not the main focus, so the priority to include them for dialogue generation is low. Examples include \url{http://schema.org/Reservoir} in Yago KG, which represent only 0.020\% of the KG's entities, respectively. Shadowed types are parent types whose entities mostly belong to a single child type.  For instance in DBLP KG, \url{https://dblp.org/rdf/schema#Creator} is a parent of \url{https://dblp.org/rdf/schema#Person}, and over 99\% of Creator entities belong to Person type. Including both parent and child types in dialogue generation reduces efficiency and leads to redundant types.\shorten
% Commented Examples
% \url{https://dblp.org/rdf/schema#Person}, \url{http://www.w3.org/2002/07/owl#TransitiveProperty},  and \url{http://schema.org/ShoppingCenter} ( 0.022\%)

This module identifies the most relevant node types to the domain of the KG. We first retrieve all node types. Then, we exclude metadata and other irrelevant types. 
We aim to identify types that facilitate generating meaningful dialogues about concepts and information relevant to the KG's specific domain (e.g., medicine, law). This approach improves time complexity compared to the brute-force solution because the number of node types in a KG is generally much smaller than the total number of nodes. Then, we create the distribution of the entities to sample from each type.

Algorithm \autoref{alg:node_selection} details the process for selecting node types and determining the number of entities to sample from each type. Each entity corresponds to a single generated dialogue.  The algorithm takes five inputs: \myNum{1} KG SPARQL endpoint for accessing the KG, \myNum{2} the required number of dialogues to generate, \myNum{3} domain prefixes for identifying relevant KG types, \myNum{4} a rare type threshold to mark types with low entity counts, and \myNum{5} a shadowed parent threshold to identify redundant types. Line 1 retrieves domain-specific types. It utilizes the provided endpoint and domain prefixes to retrieve all KG types along with their associated entity counts, creating a comprehensive list. The list is sorted by descending entity count. Then, the list is filtered to exclude irrelevant metadata and non-domain-specific types. By default, we utilize the KG's main ontology types, which represent its core information. Users can specify additional types or prefixes for inclusion. We use entity counts in the filtered list to calculate the coverage percentage of each type.

\input{algorithms/node_type_selection}
Line 2 removes rare types whose percentage is lower than the user-specified threshold. Line 3 handles shadowed types. For each type, if its direct parent type exists in the filtered list, 
we calculate the percentage of entities belonging to the child type relative to the parent type. If this percentage exceeds the user-defined threshold, the parent type is excluded. These removals cause the type percentages to no longer sum to $100\%$. Therefore, we recalculate the percentages for the remaining included types only. Finally, leveraging these adjusted percentages and the number of entities, Line 4 determines the number of entities to sample from each type. This ensures the sampled entities reflect a distribution similar to the overall KG entity distribution.\shorten

\textbf{Complexity:} Algorithm 1 has a time complexity of $O(q_{cost}+\tau)$, where $\tau$ represents the number of node types and $q_{cost}$ denotes the cost of executing the SPARQL query to retrieve types and their entity counts. Retrieving all node types ($q_{cost}$) and iterating through them ($\tau$) for filtering and calculations dominates the overall complexity. $q_{cost}$ varies depending on the used RDF engine, as it relies on the engine’s implementation and built-in indices. This approach offers a significant improvement over a brute-force solution that would require iterating through all KG nodes.

% Let $\tau$ be the number of node types returned, and $q_{cost}$ denotes the cost of executing the query to retrieve types and their counts. $q_{cost}$ varies across RDF engines since it depends on the presence of the indices and built-in functions, especially an index between node types and entity counts. Line 1's execution cost is O($q_{cost}$ + $\tau$). Because we first execute the query to retrieve all KG types ($q_{cost}$) and then iterate through the returned list ($\tau$) to filter and calculate percentages. Lines 2-4 involve iterating through the type list ($\tau$), resulting in an individual cost of O($\tau$) for each line. Thus, the overall time complexity of Algorithm \autoref{alg:node_selection} is $O(q_{cost}+\tau)$.

\subsection{Textual Entity representation}
\label{sec:entity_rep}
The textual representation significantly impacts how humans and LLMs understand the entity and their ability to generate questions. KGs represent entities using URIs, which are unsuitable for natural language questions. Therefore, we need a method to convert these URIs into a text to use in the generated questions.
One approach is to encode the entity using the final URI segment. This method assumes the human-readability of the final segment (e.g., \url{http://dbpedia.org/resource/The_Future_of_Freedom_Conference}). However, this does not generalize. In many URIs, the final segment contains IDs (e.g., \url{https://dblp.org/pid/00/10071}) or character-number combinations (e.g., \url{https://dblp.org/rec/conf/valuetools/Coppa14}). These formats hinder LLMs' ability to understand the entity's meaning, leading to ambiguous or low-quality questions.

URIs are insufficient for generating textual descriptions of entities. A more effective approach involves leveraging the context surrounding the entity. This context includes predicates outgoing from the entity, and connections to other nodes and literals. Each entity is connected to various predicates, some offer good textual representations. However, identifying a single predicate for diverse KGs or even for different node types within a single KG is challenging. Because entities of different node types are connected to their labels using different predicates (e.g., "name" for Person entities and "title" for Publication entities). Therefore, we need a mapping between node types and the most suitable predicates in the KG that retrieves the appropriate textual representation for entities. Users with domain expertise can define such mappings manually. While this may be feasible for smaller KGs with a few node types, it becomes impractical for large KGs like DBpedia or Yago, which contain hundreds or thousands of node types. This necessitates the development of an automatic approach for identifying the predicate that can be used to retrieve the label for each node type within a KG. For the remainder of this paper, we will refer to this predicate as the \textit{entity label}.\shorten

We propose a novel LLM-based approach for automatically extracting the entity label ($p_l$) for each node type within a KG. For each node type ($t$), we first sample a random entity ($e$) belonging to that type from the KG. We then extract all outgoing predicates ($P_{list}$) connected to this sampled entity ($e$). To ensure the extracted representation is a string suitable for use within questions, we filter the extracted predicate list ($P_{list}$) to keep only predicates connecting the entity ($e$) to string literals. This filtering process focuses solely on the type of node connected to the entity ($e$), regardless of the length of the literal. Because the length of labels for different entities within the same node type can vary significantly. For example, consider Place node type in the Yago KG: one entity has the label "\textit{Administrative Department of Science, Technology, and Innovation}" while another has the label "\textit{Admaston}." We defer any specific conditions on the label to the entity-level processing stage.


\begin{equation}
    \label{eq:entity}
    p_l = f(t, P_{list}, I)
\end{equation} 

% \begin{lstlisting}[language=Python, caption=Choosing representative predicate for type prompt, escapechar=@, label=label_predicate]
% # Instruction:
% Given the specified node type and its
% associated predicates, choose a suitable
% predicate to be used to extract labels for
% this type.

% # Input:
% node type:
% predicates: 

% # Response:
% \end{lstlisting}

Instruction $I$ utilizes zero-shot prompting to instruct the LLM to select the most representative predicate from the filtered list ($P_{list}$). The chosen predicate then becomes the entity label for the node type ($t$). This approach generates human-readable entity representations for all node types, regardless of the information encoded in the URIs. Additionally, it eliminates the need for technical knowledge to manually create the mapping between node types and entity labels. This improves the quality of questions asked and enhances the overall system usability.


\input{algorithms/entiy_subgraph_extraction}

\subsection{Seed Nodes and Subgraph Extraction}
This module efficiently extracts seed entities and their corresponding subgraphs from a KG. The extracted subgraph is the context for generating a dialogue. It utilizes the distribution of entity counts per node type and the entity labels for each type. To ensure smooth LLM processing, extracted entities and subgraphs meet specific criteria. Entities must have short textual labels to avoid overwhelming LLMs, and to enable them to focus on core subgraph information. For instance, in the DBLP KG, the label "\textit{Algorithmic Number Theory, First International Symposium, ANTS-I, Ithaca, NY, USA, May 6-9, 1994, Proceedings}" includes extra details such as date and location, which can distract the LLM from focusing on the subgraph information. Entities with labels that satisfy the criteria of being less than a predefined length threshold are designated as valid entities. Second, the subgraph must fit in the LLM's context length. Additionally, the subgraph should contain a sufficient number of unique predicates because they connect entities to diverse facts, providing a strong foundation for generating multiple distinct questions within a dialogue (e.g. a dialogue needs to have a minimum of three questions). Subgraphs satisfying these constraints are marked as valid subgraphs. This approach offers an advantage over the brute-force solution by eliminating the need for storing KG entities. Instead, it retrieves only the required number of entities and their corresponding subgraphs directly on the fly from the KG endpoint without traversing the entire graph, resulting in a more efficient process. Our technique prioritizes efficiency and guarantees a sufficient number of unique predicates to generate conversations, it may not necessarily select entities surrounded by the highest number of unique predicates, which might be achievable with the brute-force approach.\shorten

% \footnote{\url{https://dblp.org/rec/conf/ants/1994.html}} 



Algorithm \autoref{alg:seed_subgraph_extraction} outlines the extraction process for a specific node type. This process iterates until the desired number of entity-subgraph pairs for that type are extracted. We repeat this process for each node type. In line 3, a SPARQL query retrieves an entity of the current node type ($t$) along with its label using the entity label ($p_l$). To optimize this step, and minimize query overhead, we batch-retrieve entities from the endpoint using the input batch size and process them individually. A new SPARQL query is executed only if the entire batch is exhausted before reaching the required number of pairs ($n$).  Lines 4-6 ensure the extracted entity's label length is suitable for LLM processing. Labels exceeding the maximum label length ($label_{max}$) are skipped. For entities with suitable labels, lines 7-8 calculate the graph size and the number of unique predicates surrounding the entity within a specified hop limit ($h$). We use count queries to leverage the RDF engine's built-in indices for faster response times. Line 9 verifies that the graph size and number of unique predicates satisfy LLM processing constraints and are sufficient to generate diverse questions in the dialogue.



When the LLM's requirements are met, subgraph extraction proceeds. Line 13 extracts the subgraph surrounding the seed entity based on a pre-defined shape, the number of hops to traverse outward from the entity, and the predicate direction (e.g. outgoing only, incoming only  or both directions). The extracted subgraph encompasses all entities and literals linked to the seed entity within these parameters. Line 14 filters out triples from the extracted subgraph. First, triples containing the entity label are excluded, as the answer to any question using it would be the label itself. Additionally, triples with predicates not related to the KG domain, such as \url{http://www.w3.org/1999/02/22-rdf-syntax-ns#type} are removed. These lack domain-specific information and wouldn't contribute to questions related to useful information in the subgraph.

Furthermore, triples containing very long string literals as objects are excluded. These increase the graph size and potentially confuse the LLM by leading to questions about the object's content rather than questions related to the entity. Examples include predicates like \url{http://dbpedia.org/ontology/abstract}, which describes entities in the DBpedia KG. The abstract value for an entity like \url{http://dbpedia.org/resource/University_of_Tulsa} is too lengthy and could lead the LLM to hallucinate. Similarly, the \url{http://dbpedia.org/ontology/thumbnail} predicate connects entities to image URLs, not relevant for human-like dialogues.
Line 15 validates the filtered subgraph, ensuring it still contains sufficient information (number of triples) to enable dialogue generation. If the subgraph is marked as valid, the subgraph is added to the final list of entity-subgraph pairs. Otherwise, the algorithm moves on to process the next entity. The algorithm outputs a list of these valid entity-subgraph pairs for each node type.



\textbf{Complexity:} Algorithm \autoref{alg:seed_subgraph_extraction} has a time complexity of $O(\tau * (q2_{cost} + K))$, where $\tau$ represents the number of selected node types in Algorithm \autoref{alg:node_selection}, $q2_{cost}$ denotes the cost of extracting the subgraph within the specified hop limit and direction, and K signifies the number of triples within the extracted subgraph. $q2_{cost}$ varies depending on the used RDF engine, as it relies on the engine’s implementation and built-in indices. This approach achieves significant efficiency compared to the brute-force solution by reducing the number of iterations ($\tau \lll V$, where $V$ is the total number of entities) and avoiding entity storage by working on the fly, resulting in constant space complexity ($O(1)$).



==> sections/dialgoue_answer_generation-reahm.tex <==
% \section{Dialogue and Answer Generation}
\section{Our Multi-stage Dialogue Generation}

This section aims to automatically generate dialogue benchmarks by creating dialogues from subgraphs of seed entities and their entity labels. Our objective is to generate human-quality benchmarks. Each subgraph will be used to generate one dialogue.\shorten
% This section is organized as follows, \autoref{sec:workflow} explains the details of the three stages, \autoref{sec:validation} explains our assertion-based validations and how it works, and \autoref{sec:serialize} explains our subgraph serialization process to be used as the LLM input.\shorten

\subsection{Our LLM-based Platform}
\label{sec:llmObjective}
Our platform leverages LLMs for dialogue generation due to their exceptional understanding and text generation capabilities. 
% Unlike rule-based or template-based approaches, LLMs can generate different question types without the need for manual rule creation or template design. These methods require creating new rules or templates for each question type, increasing the human effort required for the design and limiting scalability for large KGs. Additionally, the process is time-consuming. They also result in similar questions that follow the predefined rules or templates, failing to effectively challenge systems.
To facilitate dialogue generation across arbitrary KGs, we opted for a prompting based solution. 
% Prompting is preferable to fine-tuning because fine-tuning is less time-efficient and necessitates a unique dataset for each new KG.
The brute force approach prompts the LLM with the subgraph and asks to generate dialogues using the information in the subgraph. This requires designing only one prompt, which is cost-effective and helps generate questions of different types. However, the complexity of the task restricts it to highly capable LLMs. Additionally, using zero-shot for this complex task can lead the LLM to hallucinate by generating duplicates, or unclear questions. Adding examples to the prompts using few-shot learning mitigates this issue. However, the generated dialogues become repetitive and limited by the patterns and question types in the examples. This necessitates carefully designing and selecting examples that cover various question types. Moreover, answer generation is challenging since we need to provide subgraphs with the full URIs to generate an answer linked to the KG, significantly increasing cost. If we used subgraphs with more cost-effective textual representations, the generated answers are the labels of the entity.\shorten
% Linking these labels to entities from the KG is hard since different entities can have the same label.
% For example \url{http://dbpedia.org/resource/Category:Celine_Dion}, and \url{http://dbpedia.org/resource/Celine_Dion} have the same label, \textit{Celine Dion}.\shorten

To address these limitations, we propose a multi-stage approach with assertion-based validations. This approach serializes the subgraph and leverages the LLM's text generation capabilities to generate dialogues across three stages: \myNum{1} Independent Question Generation, that generates questions asking about different facts in the KG. \myNum{2} SPARQL Query Generation which translates questions into SPARQL queries to extract answers from the KG, and \myNum{3} Dialogue Generation which transforms the independent questions into a dialogue.  This breakdown allows for better control over the process by validating the intermediate results and guiding the LLM toward high-quality dialogue generation. While the multi-stage approach may have a slightly higher cost due to executing multiple prompts, it overcomes the limitations of the single-step approach. Dividing the dialogue generation process into three less complex tasks enables {\sysName} to work with LLMs of different capabilities. Additionally, it eliminates the need for adding examples in the prompts. This provides the LLM with more flexibility to generate different question types (which may not exist in the examples) and overcome the repetitive dialogues. This approach also overcomes answer generation problems as it uses the textual representation in the input subgraphs for less costly prompts while providing queries that extract the answer directly from the KG. Our platform validation modules address the LLMs’ context length by efficiently serializing the subgraph. It also overcomes hallucination by preventing error propagation by ensuring only valid outputs at each stage progress to the next stage.

\subsection{Multi-stages Generation Workflow}
\label{sec:workflow}
This module describes our multi-stage workflow that utilizes LLMs to generate dialogues leveraging seed entities and their corresponding subgraphs. We iterate over all entity-subgraph pairs to construct the final benchmark. First, the subgraph $SG$ is serialized to a string containing the list of triples in $SG$ because LLMs require textual input~\cite{structure_serialize}. All prompts used in the different stages in our workflow uses zero-shot prompting, i.e. we do not provide examples with the prompt provided to the LLM.

\subsubsection{Independent Question Generation}
Our workflow begins by generating a set of independent questions. Given an entity $e$, its corresponding serialized subgraph $SG_{ser}$, and the number of questions per dialogue $n_d$, we prompt the LLM to automatically generate a list $Q'$, of $n_d$ independent questions. All  questions in  $Q'$ must be answerable by the subgraph, $SG_{ser}$. Also, question generated must span different question types. Moreover, answering any question in  $Q'$ doesn't require context or knowledge from other questions in the list.\shorten
\begin{equation}
\label{eq: q_gen}
    Q' = f(SG_{ser}, n_d, I)    
\end{equation}
% \begin{lstlisting}[language=Python, caption=Generating independent questions prompt, escapechar=@, label=lst:question_prompt]
% # Instruction:
% Generate a list of  questions based on the
% given entity and its subgraph. The subgraph
% is represented as a list of triples. Each
% question must ask about a fact from the 
% triples in the subgraph and must fall into
% one of the following categories: list, count
% , boolean, wh (open-ended), or date-related 
% questions. Each question must include the
% entity. Each question must be answerable
% solely from the information in the provided 
% subgraph without explicitly mentioning it.

% # Input:
% Entity:
% Subgraph:
% number of questions: 

% # Response:
% \end{lstlisting}

\subsubsection{SPARQL Query Generation}
The second stage is generating SPARQL queries for each independent question in $Q'$. Providing the LLM with the question alone is insufficient to generate a correct SPARQL query. Without knowledge of the underlying structure (i.e., the subgraph), the LLM might introduce incorrect prefixes or create predicates not existing in the subgraph based on its interpretation of the question. To generate correct queries, the LLM needs the relevant context from the KG. One approach is to inject the entire KG ontology into the LLM prompt. However, this is computationally expensive and burdens the LLM with unnecessary information about irrelevant parts of the KG, i.e. parts that the question does not ask about. A more efficient approach leverages our knowledge of the subgraph used to generate the questions. We inject only this subgraph into the prompt. However, even the subgraph might contain facts not directly related to the question since each question is generated from a subset of the subgraph, potentially confusing the LLM. Therefore, we opted to provide the LLM with the minimal information necessary: the exact triples used to generate each question. To achieve this, we extended the independent question generation module to return these triples with each question. This modification necessitates revising \autoref{eq: q_gen} to return the triples:
\begin{equation}
\label{eq:ssg_gen}
    Q', T_q = f(SG_{ser}, n_d, I)
\end{equation}

% \begin{lstlisting}[language=Python, caption=Generating Independent Questions Prompt with Triples, escapechar=@, label=lst:question_triples_prompt]
% # Instruction:
% {Question Generation Prompt}
% For each question, choose the triples from
% the input subgraph which was used to
% generate the question. Return both the
% question and the exact triple from the
% subgraph that it was based on.
% # Input:
% Entity:
% Subgraph:
% number of questions: 

% # Response:
% \end{lstlisting}

We leverage LLMs to generate SPARQL queries that answers the question from the KG given the question-triple pairs. The LLM relies solely on the question and its associated triples. This module output $SQ$ a list of SPARQL queries corresponding to the independent question list $Q’$. This approach generates syntactically correct SPARQL queries without relying on the KG ontology.

\begin{equation}
    \label{eq:sparql}
    SQ = f(Q', T_q, I) 
\end{equation}

% \begin{lstlisting}[language=Python, caption=Generating SPARQL query from Question and Triples, escapechar=@, label=lst:sparql_prompt]
% # Instruction:
% Given a question and set of triples used to
% generate this question. Create the SPARQL
% query representing the question. Do not
% include the answer in the query.
% # Input:
% Question:
% Triples:

% # Response:
% \end{lstlisting}

\subsubsection{Dialogue Generation}
The final stage of our workflow transforms the set of independent questions $Q'$ into a dialogue. This transformation must preserve the correspondence between each question and the corresponding SPARQL query. The first question remains independent, as it serves as a clear starting point of the conversation that requires no prior context. Subsequent questions depend on the answers or context provided by earlier questions. These specifications mirror the natural flow of human conversation, where initial questions are independent, and later questions build upon the established context.\shorten

Our four-step approach transforms independent questions into dialogues by: \myNum{i} identifying the common entity shared across all questions, \myNum{ii} predicting the appropriate pronoun to replace the entity, \myNum{iii} substituting the entity with the chosen pronoun in each question, and \myNum{iv} ensuring the modified questions are grammatically and linguistically correct. We leverage the LLM's understanding and linguistic capabilities by creating prompt $I$ that incorporates a clear explanation of these steps.

Successful dialogue generation requires the LLM to correctly execute each step, since they are sequentially dependent. While providing all details to the LLM is a promising direction, the complexity of the task incurs some limitations. In some instances, the LLM identifies the target entity per individual question, rather than one target entity for the entire dialogue. This leads to incorrect and different target entities per question, resulting in disconnected questions within the dialogues. For example, given questions "\textit{What is the primary affiliation of Anne Condon?}" and "\textit{What is the nationality of Anne Condon?}". The LLM incorrectly assigns "\textit{primary affiliation of Anne Condon}" and "\textit{nationality of Anne Condon}" as target entities, respectively. While, to produce a valid dialogue, the LLM must identify “\textit{Anne Condon}” as a common entity. To address this we update the LLM prompt with additional information to reduce the number of sequential steps, thereby decreasing the complexity of the task.
% To address this, we propose two solutions: \myNum{i} Using Few-Shot Learning to guide the LLM through the process instead of zero-shot, and \myNum{ii} Updating the LLM prompt with additional information to reduce the number of sequential steps, thereby decreasing the complexity of the task.

% In the few-shot based solution, we provide examples to guide the LLM through the pronoun identification and substitution steps. To produce the best performance, we divided the process into two steps, with each step having its corresponding examples. In step one, we identify the target entity and predict the pronoun given the whole dialogue. In step two, we utilize the predicted pronoun and substitute it in the questions. This method prevents identifying incorrect target entities but can generate linguistically incorrect questions, such as "\textit{What is the nationality of him?}" instead of "\textit{What is his nationality?}". Additionally, it suffers from two drawbacks: \myNum{i} The example selection process is tedious. We need to create a comprehensive set of examples for all pronouns and their forms for step one, and all possible ways to substitute them in step two, and \myNum{ii} splitting the prompt into two and including examples reduces the cost-efficiency.\shorten

% Our second and more effective, solution utilizes a single prompt. 
We utilize our knowledge of the target entity (our extracted seed entity) as additional input. The LLM predicts the appropriate pronoun based on its understanding and knowledge, then replaces the seed entity with the predicted pronoun and makes necessary adjustments to ensure grammatically and linguistically correct questions. This method offers improved dialogue quality at a lower cost compared to the few shot approach. Therefore, we chose it for generating dialogues in the final benchmark.\shorten

\begin{equation}
    \label{eq:dialogue}
    D = f(Q', e, I)
\end{equation}
% \begin{lstlisting}[language=Python, caption=Generating SPARQL query from Question and Triples, escapechar=@, label=lst:dialogue_prompt]
% # Instruction:
% Given an entity and a set of questions
% focused on this entity, choose the
% appropriate pronoun that refers to it.
% Replace the entity with its pronoun in the
% questions and return the modified questions. 
% Ensure that the modified questions do not 
% contain the original entity and that the 
% pronoun used in the modified questions is
% contextually appropriate and grammatically
% correct.

% # Input:
% Questions:
% Seed Entity:

% # Response:
% \end{lstlisting}


\subsection{Assertion-based validation}
\label{sec:validation}
To ensure a stable workflow, we need to mitigate LLM's potential hallucinations by We integrating a validator module into each workflow stage. the validator verifies the compliance of LLM's outputs with the instructions. If the output is deemed invalid, we implement a retry mechanism with a maximum of three attempts. During each attempt, the same prompt and inputs are sent to the LLM. If we do not obtain valid output after three trials, the current seed entity is skipped, and we sample a new entity of the same node type. Our validation approach relies on assertions to ensure that the LLM's output satisfies specific constraints.

\subsubsection{Question validator} 
This module validates both questions and triples. We need to ensure that questions are independent, i.e. they explicitly mention the entity. This implies that the entity was not replaced by pronouns or general concepts that make the question context-dependent. For triples, we ensure that they exist within the provided subgraph. This guarantees the correctness of triples used for subsequent query generation, preventing the LLM from being confused by inaccurate information.

\subsubsection{Query validator} 
Validation of generated queries ensures they are syntactically correct for execution and they retrieve results matching the subgraph information. Only query lists with at least three correct queries progress to the next step.\shorten

% The validation of generated queries involves multiple aspects. First, queries must be syntactically correct to ensure proper execution. Second, the retrieved results (i.e., answers to the questions) should match the information existing in the subgraph. To qualify as valid, the query list must contain at least three correct queries, as this is the minimum user-adjustable threshold to have a dialogue. Only this subset of valid queries and their corresponding questions progress to the next step.

\subsubsection{Dialogue validator}
To validate dialogues, we assess the independence of the opening question, as it initiates the conversation. For the second-to-last question, we ensure context dependence, meaning questions must not explicitly mention the target entity. Additionally, we verify that questions contain multiple words, as some LLMs return single words like pronouns \textit{his?} instead of a full question. These responses are marked as invalid.

% \subsection{Prompts Creation}
% \label{sec:prompts}
% LLMs' capabilities impact their performance on various tasks. Powerful models such as GPT-3\cite{gpt3} and GPT-4\cite{gpt4} excel in handling tasks with different complexities. Open-source models such as Llama\cite{llama, llama2} and Mistral\cite{mistral}, which perform well on many tasks, can struggle with complex tasks. To make our platform work with a wider range of LLMs regardless of their ability, we analyzed the complexity of each stage in our workflow to specify which stage is a potential bottleneck for less capable LLMs. All stages require generating structured outputs, but they differ in complexity. The first stage requires understanding the input subgraph, generating questions, and linking each question to the triples used in its generation. The output here is complex since it consists of multiple question-triple pairs. The second stage takes a question and its associated triples as input and returns a SPARQL query that answers the question. We consider this task as a simple task because the given triples are the building blocks of the SPARQL query. The last stage takes the questions as input and returns the dialogue. The output is the list of dialogue questions, which is less complex than stage one. From the previous analysis, we can conclude that the first stage (independent question generation with triples) has the most complex input to understand (subgraph), and output to generate. Therefore, we designed a simplified version of our workflow, that simplifies the independent question, and triples generation. We refer to this as the simplified workflow, and the original workflow from \autoref{sec:workflow} as the complex workflow.

% In the simplified workflow, we divide the first stage into two steps: independent question generation and question-triple binding. In the first step, we utilize the prompt in \autoref{lst:question_prompt}, to generate a list of questions. In the second step, we process each question individually. We provide the LLM with the question and the subgraph, prompting it to identify the subgraph triples that contributed to the question's generation. The detailed prompt is shown in \autoref{lst:triple_prompt}. To ensure consistency with the complex workflow's validation, we only consider the set of triples valid if the binding process succeeded for all questions, i.e. each question in the input list is associated with a valid triple from the subgraph. Although this approach has the potential to increase the cost due to the additional prompts sent to the LLM, it enables our platform to work with different LLMs.

% \begin{lstlisting}[language=Python, caption=Binding Triple to Question Prompt, escapechar=@, label=lst:triple_prompt]
% # Instruction:
% Given a question and a list of triples, your
% task is to choose the specific triples 
% within this list that were used to form the 
% question. Each triple comprises a subject, a
% predicate, and an object, denoting a
% relationship between entities. You must
% choose triples from the given triple list.,

% # Input:
% Subgraph:
% Question:

% # Response:
% \end{lstlisting}

\subsection{Subgraph Serialization}
\label{sec:serialize}

\input{algorithms/summarize_subgraph}
Serialization involves designing encoding methods for nodes and predicates within the subgraph's triples. We utilize the textual representation extracted using the entity label  $p_l$ (explained in \autoref{sec:entity_rep}) for node encoding. Predicate encoding utilizes the final segment of their URIs. This approach relies on the fact that not all KGs have label properties associated with predicates, and most KGs employ human-readable URIs (e.g., \url{https://dblp.org/rdf/schema#authoredBy} from DBLP and \url{http://schema.org/birthPlace} from Yago). In these examples, the encoded predicates would be \textit{authored By} and \textit{birth place}, respectively. This encoding removes unnecessary namespace information, allowing the LLM to focus on the meaning of nodes and predicates. The final serialized subgraph string is a list of triples, where each node and predicate is encoded using its respective technique.\shorten


\begin{definition}[Summarized Subgraph $SSG$]
\label{def:sum_subgraph}
Given a subgraph $SG(e) = \{T\}$, A summarized subgraph $SSG = \{T' ; T' \in SG \}$. For triple $T \in SG$, the corresponding $T' = \langle v_i, p, '' \rangle$, if $v_j = e$ or  $T' = \langle '', p, v_j \rangle$, if $v_i = e$. Each predicate $p$ exists only once in $SSG$
\end{definition}

We evaluated two serialization alternatives. The subgraph serialization incorporates the complete list of triples, including subject, predicate, and object. The summarized serialization, includes only specific parts of the triples. This helps the LLM to focus on question and query generation. Our summarization approach is motivated by the observation that subgraphs contain numerous predicates, some of which appear only once, while others repeat. Repeated predicates offers valuable information during graph exploration, but they are less beneficial for question generation. For example, consider a person entity who authored multiple publications. The subgraph might contain multiple triples like $\langle$Author, authored, PublicationName$\rangle$. We can generate questions like \textit{What did the author publish?} or \textit{How many papers did he author?} by only using one triple. Since the object (PublicationName), if the entity is the subject, is not included in the generated question since it is the answer.\shorten

\begin{figure}[t]
\begin{verbatim}
PREFIX rdfs: <https://dblp.org/rdf/schema>
select ?numberOfCreators 
where { <https://dblp.org/rec/conf/ichi/AgrawalSSG13>
    rdfs:numberOfCreators ?numberOfCreators. 
Filter(?numberOfCreators = 2) }
\end{verbatim}
\vspace*{-2ex}
\caption{A SPARQL query with Filter clause that ensures that the answer is equal to the specific value in the triple.\shorten}
\label{fig:wrong_example}
\end{figure}

Algorithm \autoref{alg:summarize} explains the summarization. Line $1$ extracts all unique predicates from the subgraph $SG$ to ensure complete fact inclusion. Each unique predicate represents a fact connected to the seed entity. Line $2$ groups the triples within the subgraph by predicate. This means all triples in a group share the same predicate. In lines $4-7$ for each (predicate, triple list) pair, the first triple is chosen as the group representative. Then we modify the triple based on the seed entity’s position within the triple. If the seed entity is the subject, the object is removed and vice versa. Then we add the modified triple to the summarized subgraph $SSG$. We provide the LLM with $SG_{ser}$, the string containing the list of modified triples from $SSG$.\shorten

The subgraph serialization suffers from several limitations: \myNum{1} popular entities are surrounded by many predicates cause LLM context length overflow, \myNum{2} processing long subgraphs leads to a high execution cost, and \myNum{3} Including the answer in the triples (if the seed entity is the subject) leads to generating overly strict or incorrect SPARQL queries in some cases as shown in \autoref{fig:wrong_example}. The summarized serialization addresses these issues by using  modified triples instead of  full triples. This reduces the size of the input subgraph. This allows bigger subgraphs to fit in the LLM's context length. It also decreases the cost 
% due to smaller serialized subgraphs, 
and improves token efficiency. Additionally, removing the answer enables the LLM to focus on aligning the seed entity and predicate to generate a correct SPARQL query. Therefore, the summarized serialization effectively reduces the generation of incorrect queries.\shorten


Despite the improvements in  the percentage of correct SPARQL queries while using summarized  serialization, LLM's limitations still sometimes generate incorrect queries. Examples include count questions and compound predicates. Some count questions have answers as literals in the KG, e.g., $\langle$Publication, numberOfCreators, 3$\rangle$. Others require the Count() function to get the answer, such as $\langle$Author, authored, Publication$\rangle$. LLMs struggle to differentiate between these cases, leading to incorrect query generation. Compound predicates are predicates that can be linguistically broken down, e.g "\textit{publishedInSeries}" becomes  "\textit{publishedIn}" and "\textit{series title}". The LLM generates queries using these divided forms, even if they do not exist in the KG. These errors are identified and discarded by the query validator.\shorten

% \input{algorithms/approach}
% \input{algorithms/generate_dialogue}











==> sections/discussion-old.tex <==
{\color{blue}
% \section{Discussion: Limitations, future work, and use case}
\section{Limitations, Future Work, and Use Case}
\noindent \textbf{Use case:}
To demonstrate {\sysName}'s benchmark quality, we compared its dialogues to the human-generated conversational benchmark ConvQuestions\cite{convquestions}. ConvQuestions was created using Amazon Mechanical Turk. Each set of 5 dialogues required 3 hours and cost 25 Euros\cite{convquestions}. Therefore, generating the entire benchmark costs thousands of dollars. We analyzed ConvQuestions to compare its question coverage with {\sysName}'s\footnote{Figure added to supplementary materials due to space constraints.}. We found that ConvQuestions exhibits a bias to \emph{What} questions and does not contain commands. {\sysName} produced a similar distribution, indicating alignment with human-generated conversations. For the experiments, we randomly selected $20$ entities from the ConvQuestions dataset, covering all five types. We used this list of entities to generate {\sysName} benchmarks.

In the first experiment, we used {\sysName} to generate three benchmarks with three of our top-performing LLMs from \autoref{tab:openllm}: Gpt-4o, Multi-LLM-1, and CodeLlama-13b. We used LLMs to compare dialogues for the same entity from both datasets. We instructed the LLM to identify the set of dialogues with better quality considering fluency, clarity, and variety in the questions factors. 
% The prompt for better rephrasing: Consider factors such as fluency , clarity , and variety in the questions . Based on these criteria , determine which set has better overall quality .
To prevent bias towards the models, we employed Gemini to evaluate the dialogues quality. To prevent bias to the position of the dialogue in the prompt, we provided each pair of dialogues to the LLM twice in different orders \cite{llm_judge}. If Gemini's evaluation of the same entity differed, it is considered a tie (indicating its inability to distinguish between dialogue quality). As shown in \autoref{tab:usecase}, Gemini identified a tie in $70\%$ of dialogues when using Gpt-4o and $63\%$ with Multi-LLM1. The lower tie percentage $(25\%)$ for CodeLLama-13b can be attributed to its relatively less power compared to the other two LLMs. These results demonstrate that {\sysName}-generated dialogues are comparable in quality to human-created questions. For cases where the evaluator chose ConvQuestions, {\sysName} still showed a good quality of dialogues.  The evaluator must select one dialogue as superior, even if both have high quality.

In the second experiment, we manually compared dialogues from ConvQuestions and {\sysName} to determine the similarity rate, defined as the percentage of questions that asked about the same facts with minor variations. Our analysis yielded a $25\%$ similarity rate. Given the average of $36$ unique predicates surrounding the entities and the five-question dialogues, this percentage demonstrates {\sysName}'s ability to efficiently generate human-like questions.\highlightedReply{}{R1.O4, R3.O2}\shorten


% To demonstrate the quality of the benchmarks generated by {\sysName}, we compared its dialogues to the human-generated conversational benchmark, ConvQuestions\cite{convquestions}. ConvQuestions was created using Amazon Mechanical Turk, with each set of 5 dialogues requiring 3 hours and costing 25 Euros. This means generating the entire benchmark cost thousands of dollars. We analyzed ConvQuestions to compare its question coverage with {\sysName}'s\footnote{Figure added to supplementary materials due to space constraints.}. We found that ConvQuestions exhibits a bias towards \emph{What} questions, and does not contain commands. {\sysName} provides a similar distribution, showing that its output aligns well with human-generated conversations.

% We randomly selected $20$ entities from the ConvQuestions dataset and sent them to {\sysName} to generate benchmarks. We used Gpt-4o model for generation due to its superior success rate as shown in \autoref{tab:openllm}. In the first experiment, we manually compared dialogues from ConvQuestions and {\sysName} to calculate the similarity rate, defined as the percentage of questions asking about the same facts with minor variations. Our analysis yielded a $25\%$ similarity rate. Given the average of $36$ unique predicates surrounding the entities and the five-question dialogues, this percentage demonstrates {\sysName}'s ability to efficiently generate human-like questions.

% For the second experiment, we used LLMs to compare dialogues for the same entity from both datasets. We instructed the LLM to identify the set of dialogues with a better quality. To ensure fairness, we used Gemini to evaluate the dialogues. To prevent bias to the position of the dialogue, we provided each pair of dialogues to the LLM twice in different orders \cite{llm_judge}. If the LLM produced different results for the same entity, it is considered a tie (indicating LLM’s inability to distinguish between dialogue quality). As shown in \autoref{tab:usecase}, Gemini identified a tie in $70\%$ of the dialogues, suggesting that {\sysName}-generated dialogues are comparable  in quality to human-created questions.\shorten
\input{tables/usecase}
% \input{tables/usecase_run2}
% \input{tables/usecase_run3}

\noindent \textbf{Limitations and Future work:}
{\sysName} aims to ensure the correctness of generated dialogues while being cost-efficient. To achieve this, it discards entities if hallucinations are detected during the generation process. However, users may be interested in exploring specific entities and may not want them skipped, even if it incurs additional costs. To address this, instead of discarding entities with hallucinated output, {\sysName} can be extended with a correction module that fixes erroneous output, allowing the generation pipeline to continue as expected. As shown in \autoref{tab:openllm}, hallucinations can occur at various stages of the pipeline. The correction module would require different approaches to handle these different forms of hallucination, potentially employing rule-based or model-based techniques. For instance, in the question and triple generation step, one error might involve returning a triple that is not part of the subgraph. In such cases, the correction module could either retrieve the closest triple from the subgraph or use a model to select the correct triple from the subgraph based on the given question. Another example of an error is generating a context-dependent question as the first question in the dialogue, or returning any of the second-to-last questions as an independent question. For these scenarios, a model-based solution can be adopted to utilize the entity and incorrect question to generate the correct questions according to their appropriate positions within the dialogue. Parsing errors can occur at any stage of the pipeline. If the error is minor, the correction module can fix the returned JSON. Otherwise, it can re-generate it using existing information in the output.\shorten

Additionally, most existing knowledge graph question answering systems(KGQA), such as KGQAn\cite{kgqan}, EDGQA\cite{EDGQA}, and NSQA\cite{nsqa}, do not support answering dialogue questions. {\sysName} aims to encourage developing robust conversational KGQA systems. One way to achieve this is to extend current KGQA systems with a dialogue-supporting module. \highlightedReply{}{R3.O1}

% \colorbox{blue!30}{R1.O2}


% {\sysName}, while effective in addressing certain LLM limitations like hallucinations and handling complex tasks with structured output, is still constrained by others. For example, its context length limitations can restrict the inclusion of popular head entities with large subgraphs. Additionally, {\sysName} currently generates only questions that are directly answerable from the information in the KG.  To ensure the correctness of the generated dialogues, {\sysName} discards entities if any hallucination is detected during the generation process. While this approach helps maintain dialogue quality, it may result in skipping entities that users are interested in exploring.\shorten

% \noindent \textbf{Future work:} 
% Extending {\sysName} to generate unanswerable questions from the KG will pose a significant challenge to conversational KGQA systems. These questions require systems to determine if the information needed to answer exists in the KG before attempting retrieval. Additionally, instead of discarding entities with hallucinated output, {\sysName} can be extended with a correction module. This module would attempt to fix the generated text, allowing the generation pipeline to continue as expected. This would decrease the error rate of the generation process. With the lack of existing conversational KGQA systems.  {\sysName} aims to motivate the development of robust conversational KGQA systems that can effectively handle a wide range of question types and entities.\shorten


}

==> sections/evaluation-essam1.tex <==
\section{Evaluation}

% \subsection{Benchmark Characteristics}
% For conversational benchmarks to effectively challenge systems, they must possess several key characteristics. Firstly, they should cover different question types, such as listing and WH questions, to evaluate a chatbot's ability to handle varying complexities. Secondly, the answers must be grounded in the target dataset to ensure answerability. Thirdly, benchmarks should include various entities of diverse types to test the chatbot's flexibility in dealing with miscellaneous dialogue contexts. Hence, there is a need to detect the distribution of node types within the KG. Finally, linguistic and grammatical correctness in the benchmark's questions is essential for a fair and accurate assessment, as errors in language can hinder objective evaluation.

\subsection{Evaluation Setup}

\subsubsection{Compared Systems}
We evaluate {\sysName} against Maestro \cite{maestro}, the state-of-the-art system for generating standalone and self-contained questions from KGs. It does not support dialogues. We used Maestro's code\footnote{\url{https://github.com/aorogat/Maestro}} and consulted the authors to reproduce Maestro's results on DBpedia. We extended it to work with Yago and DBLP, which required about 600 lines of code per KG\footnote{We thank the authors for reviewing our code and results for Maestro.}.\shorten

\subsubsection{Utilized LLMs}
We evaluated {\sysName} using various LLMs categorized into:
\myNum{I} Commercial LLMs: GPT-3.5-turbo \cite{radford2018improving}\cite{instructgpt}, GPT-4 \cite{gpt4}, GPT-4o \cite{gpt4o}, Gemini-1-pro \cite{geminiteam2024gemini1}, Gemini-1.5-pro \cite{geminiteam2024gemini15}. These models are accessed via API requests.
\myNum{II} Open Source LLMs: LLAMA-2-13B \cite{llama2}, LLAMA-3-8B \cite{llama3modelcard}, LLAMA-3-8B-instruct \cite{llama3modelcard}, CodeLLAMA-7B \cite{codellama}, CodeLLAMA-13B \cite{codellama}, Mistral-7B-v0.1 \cite{mistral}, Mistral-v0.1-instruct \cite{mistral}, Mistral-7B-v0.2 \cite{mistral}, Mistral-v0.2-instruct \cite{mistral}. These models are hosted on our server.

% We evaluated {\sysName} using different LLMs of different sizes. They can be divided into two categories: \myNum{i} Closed access models: GPT-3.5-turbo\cite{radford2018improving}\cite{instructgpt}, GPT-4\cite{gpt4}, GPT-4o\cite{gpt4o}, Gemini-1-pro\cite{geminiteam2024gemini1}, Gemini-1.5-pro\cite{geminiteam2024gemini15}, and \myNum{ii} Open source LLMs: LLAMA-2-13B \cite{llama2}, LLAMA-3-8B \cite{llama3modelcard}, LLAMA-3-8B-instruct \cite{llama3modelcard}, CodeLLAMA-7B \cite{codellama}, CodeLLAMA-13B \cite{codellama}, Mistral-7B-v0.1 \cite{mistral}, Mistral-v0.1-instruct \cite{mistral}, Mistral-7B-v0.2 \cite{mistral}, Mistral-v0.2-instruct \cite{mistral}. The closed access models are used via sending requests to their APIs. Open source LLMs are used via sending requests to our server hosting these LLMs.

\subsubsection{Three Different Real KGs}
To evaluate the system's ability to run with KGs of different domains, We use three KGs: DBpedia, Yago, and DBLP. DBpedia and yago are general knowledge graphs. They contain information about people, places, and movies, … etc. DBLP is an academic graph that contains information about scientific publications, authors, and citations. 

\subsubsection{Computing Infrastructure}
We use two different setups for our experiments: \myNum{I} A Linux machine with 180GB RAM and 16 CPU cores, used for deploying KGs on Virtuoso SPARQL endpoints, running {\sysName} with closed access models (via APIs), and running Maestro. \myNum{II} A Linux machine with one Nvidia A100 40GB GPU, 32 CPU cores, and 64GB RAM, used for hosting open-source LLMs and running {\sysName} with them.

% We use two different settings for our experiments. In the first setting, We use a Linux machine with $180GB$ RAM and $16$ CPU cores. We use this setting for deploying KGs on virtuoso SPARQL endpoints, running {\sysName} with closed access models i.e. models accessed using APIs, and running Maestro. In the second setting, We use a Linux machine with one Nvidia A100 40GB GPU Card, 32 CPU cores and 64GB RAM. We use this setting to host Open source LLMs, and running {\sysName} with them.\shorten

\subsubsection{{\sysName} Implementation and Configuration}
{\sysName} is implemented using Python 3.10, the Lang chain library v0.1.4, and the OpenLLM library v0.4.44 \cite{Pham_OpenLLM_Operating_LLMs_2023} to host open-source LLMs. For SPARQL endpoints, we use Virtuoso v7.2.5.2, widely adopted for large KGs, preparing three separate Virtuoso endpoints for each KG. A standard, unmodified Virtuoso installation was used in all experiments. For node type selection, we apply a 1\% rare types threshold and a 99\% shadowed parent threshold. For entity and subgraph extraction, we use an entity batch size of 10,000, a hop count of 1, and both outgoing and incoming predicate directions.
%
{\sysName} is a configurable benchmark generation framework, allowing users to generate tailored benchmarks with different settings. Users can specify parameters such as: (i) the KG endpoint URL, (ii) the number of dialogues, (iii) the maximum number of questions per dialogue, and (iv) the LLM to use per module.

% \subsubsection{{\sysName} Implementation, Settings, and Configuration}
% {\sysName} is implemented using Python $3.10$, Lang chain library v$0.1.4$, and OpenLLM library v$0.4.44$ \cite{Pham_OpenLLM_Operating_LLMs_2023} to host the open source LLMs. For SPARQL endpoints, we use Virtuoso v$7.2.5.2$, as it is widely adopted as an endpoint for big KGs. We prepare three different Virtuoso endpoints, one for each of the KGs. The standard, unmodified installation of the Virtuoso engine was used in all of our experiments. For node type selection, we use $1\%$ rare types' threshold, and $99\%$ shadowed parent threshold. For entity and subgraph extraction, we use entity batch size of $10,000$, number of hops is equal to $1$, and outgoing and incoming predicate direction. 

% \subsubsection{{\sysName} Configuration}
% {\sysName}  is a configurable benchmark generation framework. It empowers users to generate benchmarks tailored to their specific needs using different settings. Users can create benchmarks containing the required number of questions and targeting various KGs with minimal configuration. To initiate the benchmark generation, users specify the following key parameters: \myNum{i} the KG endpoint URL, \myNum{ii} the number of dialogues, \myNum{iii}  the maximum number of questions per dialogue, and \myNum{iv}  the LLM to use per module.



% \subsection{Benchmark Quality}
 \subsection{Question Quality and Time Efficiency}
% We evaluated {\sysName}'s ability to generate human-like questions. \autoref{fig:independent_example} shows examples of the generated questions. The textual entity representation plays a crucial role. Disabling this module and relying on the URI's last segment significantly impacts question quality and clarity, as shown in \autoref{fig:independent_example}. This results in a significant increase in question validation errors, indicating the absence of the entity representation in the generated questions. This demonstrates the importance of a meaningful entity representation to the LLM to comprehend the entity and generate questions. Disabling the module resulted in a significant increase in question validation errors, from $1$ to $109$ for DBLP KG, from $1$ to $51$ for Yago KG, and from $0$ to $16$ for DBpedia KG. This highlights the effectiveness of textual representations, as a reduction in the number of errors suggests improved LLM understanding and question quality.

\subsubsection{Human-Like Generated Questions}
We compared the independent questions generated by {\sysName} and Maestro to determine which system produces more human-like questions. \autoref{fig:independent_example} illustrates examples generated by the two systems. All Maestro’s questions for the same seed entity have the same answer, the entity itself. This leads to similar questions asking about the same facts with different rephrasing.
In contrast, {\sysName} asks questions about various facts surrounding the chosen entity. This diversity in facts included in questions suggests {\sysName}'s superior performance. The same pattern persists for the other KGs: Yago and DBpedia. This improvement is attributed to the rich subgraphs with multiple facts used for question generation, and the entity representation module, which empowers the LLM to understand the entity's meaning and rely on its capabilities instead of rule-based approach followed by Maestro.

\begin{figure}[t]
\vspace*{-2ex}
\small
	\begin{verbatim}
Maestro:
1. Who authored the Publication "baraki19"?
2. The authored by of the Publication "baraki19"?
3. Is the Person "8766" the authored by of
the  Publication "baraki19"?
4. What authored by the Person "11171"?
5. Who is the authored by of the Publication "daun18"?

Chatty-Gen using predicate label:
1. Who is the author of Cooperative Situation
Awareness in Transportation?
2. In which year was Cooperative Situation 
Awareness in Transportation published?
3. What is the primary affiliation of Jiaxin Pan?
4. Is Jiaxin Pan associated with any other affiliation?
5. In which journal was 'Trust-Region Methods
on Riemannian Manifolds.' published?
\end{verbatim}
 \vspace*{-3ex}
	\caption{Examples of questions generated by Maestro and {\sysName} from the DBLP KG. {\sysName} predicts textual representations for entities, which helps LLMs generate human-like questions.}
	\label{fig:independent_example}
 \vspace*{-1ex}
\end{figure}

\begin{figure*}[t]
\vspace*{-2ex}
\centering
   \begin{subfigure}{.3\textwidth}
   	\centering
   	\includegraphics[width=\columnwidth]{figures/maestro_complexity_yago.pdf}
   	\caption{YAGO KG}
   	\label{fig:yago_maestro_complexity}
   \end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dblp.pdf}
	\caption{DBLP KG}
	\label{fig:dblp_maestro_complexity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dbpedia.pdf}
	\caption{DBpedia KG}
	\label{fig:maestro_complexity}
	\end{subfigure}
 \vspace*{-3ex}
	\caption{Comparison of the coverage of question types generated by Maestro and {\sysName} for the three KGs.}
	\label{fig:coverage}
 \vspace*{-1ex}
\end{figure*}

\begin{figure*}[t]
% \vspace*{-2ex}
	\centering
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity2.pdf}
		\caption{DBLP KG}
		\label{fig:dblp_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity2.pdf}
		\caption{YAGO KG }
		\label{fig:yago_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity2.pdf}
		\caption{DBpedia KG}
		\label{fig:dbpedia_diversity2}
	\end{subfigure}
	 \vspace*{-3ex}
	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
	\label{fig:diversity2}	
 \vspace*{-2ex}
\end{figure*}

\subsubsection{Diversity of Question Types}
We evaluated {\sysName} and Maestro with respect to the question types covered in their generated benchmarks. \autoref{fig:coverage} illustrates the distribution of question types (question words) for both systems on the three KGs: DBLP, Yago, and DBpedia. We group questions that does not start with a question word into categories. Examples include Yes/No questions (We refer to it as Boolean) starting with \textit{is, did, …, etc.}, and questions starting with nouns (we refer to it as Noun) such as \textit{through, the, by, ..., etc.} As shown in Figures \ref{fig:yago_maestro_complexity} and \ref{fig:dblp_maestro_complexity}, Maestro has a bias towards boolean questions for YAGO and DBLP, whereas {\sysName} produces a less biased distribution. For DBpedia, we compared the benchmark question types generated by the two systems with the human generated QALD-9 dataset (\autoref{fig:maestro_complexity}). While QALD-9 offers a wider variety of question types than either system, {\sysName} still demonstrates a good variation, despite being automatically generated. Notably, Maestro's bias towards boolean questions persists, generating a higher percentage of boolean questions compared to the average in question answering benchmarks. For example, QALD-9 contains only $3\%$ boolean questions, while Maestro generates $34\%$. In contrast, {\sysName} produces a more typical percentage of boolean questions. {\sysName}’s consistency across the three KGs suggests its ability to work with different KGs from various domains. {\sysName} effectively generates high-quality dialogues that mimic human conversations. 
% \autoref{fig:example} shows examples of the generated dialogues for DBLP and YAGO KGs. The questions within the dialogue are relevant and form a coherent discussion about various facts related to one entity.\shorten





% \begin{figure}[t]
% 	\begin{verbatim}
% 		Example YAGO:
% 		1. What is the birth place of Charlie Chaplin?,
% 		2. What is his nationality?,
% 		3. What are his alternate names?,
% 		4. What awards did he receive?,
% 		5. When did he die?
		
% 		Example DBLP:
% 		1. What is the bibtex Type of 'An Adaptive Hierarchical
% 		Approach to the Extraction of High Resolution Medial
% 		Surfaces.'?,
% 		2. How many creators does it have?,
% 		3. Is it listed on the Toc Page?,
% 		4. What is the year of publication?,
% 		5. In which event was it published in 2012?
% 	\end{verbatim}
% 	\caption{Examples of generated questions by {\sysName} for the different KGs.}
% 	\label{fig:example}
% \end{figure}

% yago - gpt-4 example
% dblp - gpt-4 example

% \begin{figure}[t]
% \small
% 	\begin{verbatim}
% Example YAGO:
% 1. Where was Arthur Stuart-Menteth Hutchinson born?
% 2. What alternate names are known for him?
% 3. What was the occupation of him?
% 4. When did he die?
% 5. Where did he pass away?

% Example DBLP:
% 1. What type of work is 'Systems of Logic Based on -
% -Ordinals.' classified as in Bibtex?
% 2. Who authored it?
% 3. What is the DOI of it?",
% 4. In which year was it published?
% 5. How many creators were involved in it?
% 	\end{verbatim}
%  \vspace*{-3ex}
% 	\caption{Examples of generated questions by {\sysName} for the different KGs.}
% 	\label{fig:example}
%  \vspace*{-2ex}
% \end{figure}


\subsubsection{Coverage of Main KG Node Types}
We evaluate the seed node selection module in {\sysName} and Maestro to ensure the chosen node types reflect the node type distribution in the KG. \autoref{fig:diversity2} illustrates how the KG node type distribution compare to {\sysName} and Maestro. We obtain node types by querying the KG endpoint for each chosen entity and calculating the percentage of each type. For {\sysName}, most types closely match the KG distribution. However, some differences exist because some nodes have multiple types, so a single seed contributes to multiple types. On the other hand, Maestro does not include many seeds from the most representative types in the KG. For instance, the Person type, constituting $18\%$of DBpedia KG entities, is absent from Maestro's benchmark. Maestro generates a high percentage of rare types, like Social Person ($26\%$ of its benchmark). To simplify the figure, we excluded KG types with less than $5\%$ 

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity.pdf}
% 		\caption{DBLP KG}
% 		\label{fig:dblp_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity.pdf}
% 		\caption{YAGO KG }
% 		\label{fig:yago_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity.pdf}
% 		\caption{DBpedia KG}
% 		\label{fig:dbpedia_diversity}
% 	\end{subfigure}
	 
% 	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
% 	\label{fig:diversity}	
% \end{figure*}


\subsubsection{Time Performance in Question Generation}
This experiment analyzes the time taken by Maestro and {\sysName} to produce benchmarks of $100$ questions for different KGs, \autoref{tab:maestro_time} shows the time taken in hours by both systems. Maestro first needs to traverse the whole KG. It extracts all predicates with their context, a context defined as (predicate, subject\_type, object\_type).  All contexts are saved in PostgreSQL Database for subsequent access. Then, the required number of seed entities is retrieved from the Database and the benchmark generation process starts. In \autoref{tab:maestro_time}, we show the number of predicates processed by Maestro per KG, for DBLP and YAGO we included all predicates, while for DBpedia we stopped at $18,211$ out of $994,592$ predicates for memory limitations, but the whole process needs days to finish. Maestro time is dominated by this preprocessing, and it is proportional to the number of predicates. {\sysName} uses the information in the entire KG on the fly, and needs minutes to run the end-to-end generation process, regardless of the size of the target KG. This order of magnitude improvement in running time can be attributed to the seed sampling process explained in \autoref{sec:seed}. It eliminates the need to perform any pre-processing step, while the validation of the extracted seeds ensures that the seeds are good enough to create meaningful questions.

\input{tables/maestro_timev2}

\input{tables/open_llm_june23_v2}

\subsection{Consistent Performance with Diverse LLMs}

This experiment demonstrates how our multi-stage approach optimizes Retrieval Augmented Generation (RAG) systems for complex tasks like dialogue generation from KGs, enhancing performance, especially for less powerful and open-source models. We focus on open-source models as they are more cost-effective for long-term projects and eliminate the need to send private data to external APIs. To illustrate the performance improvements, we compared our multi-stage approach to a one-stage approach (providing the LLM with a subgraph and prompting it to generate dialogue questions with corresponding SPARQL queries) using various LLMs and two KGs: YAGO and DBLP.


\subsubsection{Open-Source vs. Commercial LLMs}

We tested representative samples of commercial and open-source LLMs. \autoref{tab:openllm} summarizes the LLMs' performance on both approaches across different domains. We measured dialogues generated successfully (\texttt{Dialogues-S}), success rate, validation errors (\texttt{Questions-E}, \texttt{Triples-E}, \texttt{Dialogue-E}), parsing errors (\texttt{Parsing-E}), time, and total tokens. Each LLM was tasked with generating benchmarks of 20 dialogues, each with up to 5 questions. We set a limit of 500 seed entities for the multi-stage approach and 1000 for the one-stage approach.
%
For open-source LLMs, our multi-stage approach significantly improves the success rate compared to a single prompt approach. Only one model (\texttt{LLAMA-3-8b-inst}) successfully generated all dialogues using the single prompt approach, while all models succeeded with the multi-stage approach.
%
For commercial LLMs, despite requiring only a single prompt compared to three in the multi-stage approach, the multi-stage method achieves significantly higher success rates. For example, \texttt{GPT-4o} achieved success rates of 100\% and 95\% for YAGO and DBLP, respectively, using the multi-stage approach, compared to 38\% and 8\% using the single-prompt approach. This approach also leads to lower costs and time due to processing fewer nodes and not needing to restart due to hallucinations.\shorten

\subsubsection{Multi-Stage with Multiple LLMs (Multi-LLMs)}

We tested two variations of {\sysName} with Multi-LLMs, combining the best-performing open-source and commercial models from each stage:
\myNum{1} \texttt{Multi-LLM-1}: Uses \texttt{LLAMA-3-instruct (8B)} for question-triple and dialogue generation, and \texttt{CodeLLAMA (13B)} for SPARQL queries (open-source only).
\myNum{2} \texttt{Multi-LLM-2}: Uses \texttt{GPT-4} for question-triple generation, \texttt{LLAMA-3-instruct (8B)} for dialogue generation, and \texttt{CodeLLAMA (13B)} for SPARQL queries (uses \texttt{GPT-4} for one stage).
%
Both Multi-LLM variations achieve performance comparable to commercial models. \texttt{Multi-LLM-1} uses only open-source models, while \texttt{Multi-LLM-2} uses \texttt{GPT-4} for only one stage, demonstrating the cost-effectiveness of this approach.

In conclusion, our multi-stage approach in {\sysName} effectively improves the performance of open-source and commercial LLMs in dialogue benchmark generation tasks. \texttt{\sysName} offers a more efficient and cost-effective solution by dividing complex tasks into sub-tasks and leveraging the strengths of different models. The flexibility to use different models in different stages allows for customization and improved success rates across a broader range of LLMs.\shorten

% This experiment shows how our multi-stage approach for optimizing Retrieval Augmented Generation (RAG) systems for complex tasks such as dialogue generation from KGs helps models perform better, especially for less powerful and open source models. We focus on working with open source models since they make LLM solutions more affordable, especially for organizations’ long term projects which will cost a lot if it relied on commercial models. Also, from a security perspective, this will eliminate the need to send private data to external APIs. To show the improvement in performance, we compare our multi-stage approach to the one-stage approach (Providing the LLM with a subgraph and prompting it to generate dialogue questions with its corresponding SPARQL queries) using multiple LLMs of different sizes and two KGs of different domains: YAGO and DBLP. We tested it with commercial models (GPT-3.5, GPT-4, GPT-4o, Gemini-Pro-1, Gemini-Pro-1.5) and open-source models (LLAMA-2 (13B), LLAMA-3 (8B), LLAMA-3-instruct (8B), CodeLLAMA (7B/13B), Mistral-v0.1 (7B)). 

% \autoref{tab:openllm} summarizes the performance of the LLMs on both multi-stage and one-stage approaches for different domains. Dialogues-S is the number of successfully generated dialogues. Success rate is the proportion of successful dialogue generation attempts. A higher success rate reflects the LLM's ability to generate Dialogues-S while skipping few or no seed entities. Questions-E, Triples-E, and Dialogue-E are the number of validation errors skipped for question, triples, and dialogue generation, respectively. Parsing-E is the number of cases where LLMs fail to return a correctly structured response. Time is the total time taken by {\sysName} to generate the benchmark in minutes. Number of tokens is the total token count sent to and returned from the LLMs in millions to generate the benchmarks.  For this experiment, we asked the LLM to generate benchmarks of $20$ dialogues, each containing a maximum of $5$ questions. To ensure a finite generation, we set a limit of 500 seed entities for multi-stage and $1000$ for one-stage. If the limit is reached before generating the $20$ dialogues, we stop the process.

% As shown in \autoref{tab:openllm}, the overall success rate for all open source LLMs using the multi-stage approach is better than the one-stage approach. This shows that dividing the complex dialogue generation task to simpler tasks (question-triple, SPARQL, dialogue generation) enables the LLMs to successfully generate the required outputs. Additionally, for most LLMs, the number of validation errors caught in each stage is less than the number of errors generated at the one-stage. Even if LLMs passed all validation checks and successfully generated dialogues, converting the generated text into a structured format proves challenging for some models. This is why dividing the tasks into simpler tasks that simplify the output led to a decrease in the number of parsing errors in the multi-stage approach. Across open source models, only the LLAMA-3-8b-inst model succeeds in generating $20$ dialogues using the single-stage approach, while all models were successful with the multi-stage approach. The performance trends for both DBLP and YAGO graphs are similar, with DBLP being the more challenging dataset for most LLMs. This can be concluded from the lower success rates in DBLP. This can be attributed to two factors: the similarity of YAGO data (general knowledge) to the LLMs' training data unlike DBLP (academic, domain-specific). And, the long titles of papers and conferences in DBLP likely make it harder for LLMs to understand entity semantics.

% The commercial models show a similar pattern to the open source models, where the multi-stage approach helps these models achieve better success rate with less or comparable validation errors. For example, GPT- 4o’s success rate for single-stage for YAGO KG and DBLP KG are $38\%$ and $8\%$, while for multi-stage it is $100\%$ and $95\%$. For these models, the multi-stage approach offers additional advantages of lower cost and time compared to the one-stage approach. Despite requiring only one prompt compared to three in the multi-stage approach, the multi-stage method achieves a significantly higher success rate. This leads to processing fewer nodes, leading to lower cost and time for benchmark generation.

% To improve the overall performance of the dialogue generation task using the open source models and decrease the cost of using commercial models. We combined the best performing model from each stage (i.e. models with lower validation error in this stage) to leverage these models' ability to achieve a better overall performance. We tested {\sysName} using two variations of Multi-LLMs where we use different models in each stage of the process. Multi-LLM-1 uses LLAMA-3-instruct (8B) for Question-triple and Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. Multi-LLM-2 uses GPT-4 for Question-triple Generation, LLAMA-3-instruct (8B) for Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. These two variations achieve comparable performance to commercial models. Multi-LLM-1 uses only open source models, and Multi-LLM2 uses GPT-4 for only one stage which decrease the cost. This flexibility to use different models in different stages allows LLM-based systems like {\sysName} to generate more complex outputs while achieving better performance and success rate at a lower cost.

\subsection{Summarization}
In the following experiments, We evaluate the effect of subgraph summarization on the cost (number of tokens), time to complete benchmark generation, and percentage of correct SPARQL queries generated by LLMs.

\input{tables/subgraph_vs_summarized}

\subsubsection{Cost Efficiency}
The cost is defined as the number of tokens sent to and returned from the LLM in each end-to-end pipeline. To evaluate the cost of the two approaches, we report the average, minimum, maximum, and total number of tokens needed to generate benchmarks of 20 dialogues ( $\approx$ 100 questions) As shown in \autoref{tab:comp}, {\sysName} consistently has lower costs across the different KGs. This demonstrates the efficiency of summarizing the subgraph. There is a cost difference between YAGO and DBLP, although both are generated using the same number of dialogues. This can be attributed to the longer DBLP labels, e.g. paper titles.

\subsubsection{Answer Correctness}
We evaluate the subgraph and summarized approaches with respect to generating syntactically correct SPARQL queries that retrieve the answer to the questions. We validate the queries by executing them against the remote KG endpoint, and only correct question-query pairs exist in the benchmark. If a query fails to execute, it's considered a syntax error. If it executes but returns a different answer than the one stored in the subgraph, it's marked as incorrect. Otherwise, it's considered correct. \autoref{tab:comp} shows the percentage of correct queries generated by {\sysName}  and the subgraph approach across the three KGs. {\sysName}  outperforms the subgraph approach in all KGs. This improvement arises from removing the answer when creating the summarized subgraph, which reduced LLMs confusion. In general, both {\sysName}  and the subgraph approach perform better on YAGO compared to DBLP. This can be attributed to two factors: \myNum{i} YAGO's domain (general knowledge) is more similar to the data the LLMs were trained on, and \myNum{ii} the long labels for publication names in DBLP can confuse the LLM during processing the subgraph.

\subsubsection{Time Efficiency}
We compare the average time taken by {\sysName} and the subgraph approach to generate one dialogue with its SPARQL queries. This time is divided into processing time of the LLM and network latency if the LLM resides on a remote server.  \autoref{tab:comp} shows that both approaches needs comparable time to generate dialogues, as the network latency dominates the time.


==> sections/evaluation-reham.tex <==
\section{Evaluation}
\subsection{{\sysName} Configuration}
{\sysName}  is a configurable benchmark generation framework. It empowers users to generate benchmarks tailored to their specific needs using different settings. Users can create benchmarks containing the required number of questions and targeting various KGs with minimal configuration. To initiate the benchmark generation, users specify the following key parameters: \myNum{i} the KG endpoint URL, \myNum{ii} the number of dialogues, \myNum{iii}  the maximum number of questions per dialogue, and \myNum{iv}  the LLM to use per module
% , and \myNum{v} the workflow type (complex or simplified).

\subsection{Benchmark Characteristics}
For conversational benchmarks to effectively challenge systems, they must possess several key characteristics. Firstly, they should cover different question types, such as listing and WH questions, to evaluate a chatbot's ability to handle varying complexities. Secondly, the answers must be grounded in the target dataset to ensure answerability. Thirdly, benchmarks should include various entities of diverse types to test the chatbot's flexibility in dealing with miscellaneous dialogue contexts. Hence, there is a need to detect the distribution of node types within the KG. Finally, linguistic and grammatical correctness in the benchmark's questions is essential for a fair and accurate assessment, as errors in language can hinder objective evaluation.

\subsection{Evaluation Setup}
\subsubsection{Compared Systems}
We evaluate {\sysName} against Maestro \cite{maestro}, the state-of-the-art system for generating benchmarks for KGs. The code of Maestro\cite{maestro} is available. The results reported for Maestro are a result of our running of the system.
\subsubsection{Three Different Real KGs}
To evaluate the system's ability to run with KGs of different domains, We use three KGs: DBpedia, Yago, and DBLP. DBpedia and yago are general knowledge graphs. They contain information about people, places, and movies, … etc. DBLP is an academic graph that contains information about scientific publications, authors, and citations. 
\subsubsection{Computing Infrastructure}
We use two different settings for our experiments. In the first setting, We use a Linux machine with $180GB$ RAM and $16$ CPU cores. We use this setting for deploying KGs on virtuoso SPARQL endpoints, running {\sysName} with closed access models i.e. models accessed using APIs, and running Maestro. In the second setting, We use a Linux machine with one Nvidia A100 40GB GPU Card, 32 CPU cores and 64GB RAM. We use this setting to host Open source LLMs, and running {\sysName} with them.
\subsubsection{{\sysName} implementation and settings}
{\sysName} is implemented using Python $3.10$, Lang chain library v$0.1.4$, and OpenLLM library v$0.4.44$ \cite{Pham_OpenLLM_Operating_LLMs_2023} to host the open source LLMs. For SPARQL endpoints, we use Virtuoso v$7.2.5.2$, as it is widely adopted as an endpoint for big KGs. We prepare three different Virtuoso endpoints, one for each of the KGs. The standard, unmodified installation of the Virtuoso engine was used in all of our experiments. For node type selection, we use $1\%$ rare types' threshold, and $99\%$ shadowed parent threshold. For entity and subgraph extraction, we use entity batch size of $10,000$, number of hops is equal to $1$, and outgoing and incoming predicate direction. 
\subsubsection{LLMs}
We evaluated {\sysName} using different LLMs of different sizes. They can be divided into two categories: \myNum{i} Closed access models: GPT-3.5-turbo\cite{radford2018improving}\cite{instructgpt}, GPT-4\cite{gpt4}, GPT-4o\cite{gpt4o}, Gemini-1-pro\cite{geminiteam2024gemini1}, Gemini-1.5-pro\cite{geminiteam2024gemini15}, and \myNum{ii} Open source LLMs: LLAMA-2-7B \cite{llama2}, LLAMA-2-13B \cite{llama2}, LLAMA-3-8B \cite{llama3modelcard}, LLAMA-3-8B-instruct \cite{llama3modelcard}, CodeLLAMA-7B \cite{codellama}, CodeLLAMA-13B \cite{codellama}, Mistral-7B-v0.1 \cite{mistral}, Mistral-v0.1-instruct \cite{mistral}, Mistral-7B-v0.2 \cite{mistral}, Mistral-v0.2-instruct \cite{mistral}. The closed access models are used via sending requests to their APIs. Open source LLMs are used via sending requests to our server hosting these LLMs.

\subsection{Benchmark Quality}
We evaluated {\sysName}'s ability to generate human-like questions. \autoref{fig:independent_example} shows examples of the generated questions. The textual entity representation plays a crucial role. Disabling this module and relying on the URI's last segment significantly impacts question quality and clarity, as shown in \autoref{fig:independent_example}. This results in a significant increase in question validation errors, indicating the absence of the entity representation in the generated questions. This demonstrates the importance of a meaningful entity representation to the LLM to comprehend the entity and generate questions. Disabling the module resulted in a significant increase in question validation errors, from $1$ to $109$ for DBLP KG, from $1$ to $51$ for Yago KG, and from $0$ to $16$ for DBpedia KG. This highlights the effectiveness of textual representations, as a reduction in the number of errors suggests improved LLM understanding and question quality.

We compared the independent questions generated by {\sysName} and Maestro to determine which system produces more human-like questions. \autoref{fig:independent_example} illustrates examples generated by the two systems. All Maestro’s questions for the same seed entity have the same answer, the entity itself. This leads to similar questions asking about the same facts with different rephrasing.
In contrast, {\sysName} asks questions about various facts surrounding the chosen entity. This diversity in facts included in questions suggests {\sysName}'s superior performance. The same pattern persists for the other KGs: Yago and DBpedia. This improvement is attributed to the rich subgraphs with multiple facts used for question generation, and the entity representation module, which empowers the LLM to understand the entity's meaning and rely on its capabilities instead of rule-based approach followed by Maestro.

\begin{figure}[t]
\vspace*{-2ex}
\small
	\begin{verbatim}
Maestro:
1. Who authored the Publication "baraki19"?
2. The authored by of the Publication "baraki19"?
3. Is the Person "8766" the authored by of
the  Publication "baraki19"?
4. What authored by the Person "11171"?
5. Who is the authored by of the Publication "daun18"?

Chatty-Gen using predicate label:
1. Who is the author of Cooperative Situation
Awareness in Transportation?
2. In which year was Cooperative Situation 
Awareness in Transportation published?
3. What is the primary affiliation of Jiaxin Pan?
4. Is Jiaxin Pan associated with any other affiliation?
5. In which journal was 'Trust-Region Methods
on Riemannian Manifolds.' published?

Chatty-Gen without predicate label
1. What is the bibtex Type of item Adler12?
2. Who is the author of Adler12?
3. When was the Phdthesis 'Bailer20' published?
4. Which school accepted the thesis in publication
Beck15?
5. In which year was publication Beck15 published?
	\end{verbatim}
 \vspace*{-3ex}
	\caption{Examples of questions generated by Maestro and {\sysName} with and without using labels for DBLP KG.}
	\label{fig:independent_example}
 \vspace*{-1ex}
\end{figure}

We evaluated {\sysName} and Maestro with respect to the question types covered in their generated benchmarks. \autoref{fig:coverage} illustrates the distribution of question types (question words) for both systems on the three KGs: DBLP, Yago, and DBpedia. We group questions that does not start with a question word into categories. Examples include Yes/No questions (We refer to it as Boolean) starting with \textit{is, did, …, etc.}, and questions starting with nouns (we refer to it as Noun) such as \textit{through, the, by, ..., etc.} As shown in Figures \ref{fig:yago_maestro_complexity} and \ref{fig:dblp_maestro_complexity}, Maestro has a bias towards boolean questions for YAGO and DBLP, whereas {\sysName} produces a less biased distribution. For DBpedia, we compared the benchmark question types generated by the two systems with the human generated QALD-9 dataset (\autoref{fig:maestro_complexity}). While QALD-9 offers a wider variety of question types than either system, {\sysName} still demonstrates a good variation, despite being automatically generated. Notably, Maestro's bias towards boolean questions persists, generating a higher percentage of boolean questions compared to the average in question answering benchmarks. For example, QALD-9 contains only $3\%$ boolean questions, while Maestro generates $34\%$. In contrast, {\sysName} produces a more typical percentage of boolean questions. {\sysName}’s consistency across the three KGs suggests its ability to work with different KGs from various domains. {\sysName} effectively generates high-quality dialogues that mimic human conversations. \autoref{fig:example} shows examples of the generated dialogues for DBLP and YAGO KGs. The questions within the dialogue are relevant and form a coherent discussion about various facts related to one entity.\shorten

\begin{figure*}[t]
\vspace*{-2ex}
\centering
   \begin{subfigure}{.3\textwidth}
   	\centering
   	\includegraphics[width=\columnwidth]{figures/maestro_complexity_yago.pdf}
   	\caption{YAGO KG}
   	\label{fig:yago_maestro_complexity}
   \end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dblp.pdf}
	\caption{DBLP KG}
	\label{fig:dblp_maestro_complexity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dbpedia.pdf}
	\caption{DBpedia KG}
	\label{fig:maestro_complexity}
	\end{subfigure}
 \vspace*{-3ex}
	\caption{Comparison of the coverage of question types generated by Maestro and {\sysName} for the three KGs.}
	\label{fig:coverage}
 \vspace*{-1ex}
\end{figure*}



% \begin{figure}[t]
% 	\begin{verbatim}
% 		Example YAGO:
% 		1. What is the birth place of Charlie Chaplin?,
% 		2. What is his nationality?,
% 		3. What are his alternate names?,
% 		4. What awards did he receive?,
% 		5. When did he die?
		
% 		Example DBLP:
% 		1. What is the bibtex Type of 'An Adaptive Hierarchical
% 		Approach to the Extraction of High Resolution Medial
% 		Surfaces.'?,
% 		2. How many creators does it have?,
% 		3. Is it listed on the Toc Page?,
% 		4. What is the year of publication?,
% 		5. In which event was it published in 2012?
% 	\end{verbatim}
% 	\caption{Examples of generated questions by {\sysName} for the different KGs.}
% 	\label{fig:example}
% \end{figure}

% yago - gpt-4 example
% dblp - gpt-4 example

\begin{figure}[t]
\small
	\begin{verbatim}
Example YAGO:
1. Where was Arthur Stuart-Menteth Hutchinson born?
2. What alternate names are known for him?
3. What was the occupation of him?
4. When did he die?
5. Where did he pass away?

Example DBLP:
1. What type of work is 'Systems of Logic Based on -
-Ordinals.' classified as in Bibtex?
2. Who authored it?
3. What is the DOI of it?",
4. In which year was it published?
5. How many creators were involved in it?
	\end{verbatim}
 \vspace*{-3ex}
	\caption{Examples of generated questions by {\sysName} for the different KGs.}
	\label{fig:example}
 \vspace*{-2ex}
\end{figure}


\subsection{Node type Distribution}
We evaluate the seed node selection module in {\sysName} and Maestro to ensure the chosen node types reflect the node type distribution in the KG. \autoref{fig:diversity2} illustrates how the KG node type distribution compare to {\sysName} and Maestro. We obtain node types by querying the KG endpoint for each chosen entity and calculating the percentage of each type. For {\sysName}, most types closely match the KG distribution. However, some differences exist because some nodes have multiple types, so a single seed contributes to multiple types. On the other hand, Maestro does not include many seeds from the most representative types in the KG. For instance, the Person type, constituting $18\%$of DBpedia KG entities, is absent from Maestro's benchmark. Maestro generates a high percentage of rare types, like Social Person ($26\%$ of its benchmark). To simplify the figure, we excluded KG types with less than $5\%$ 

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity.pdf}
% 		\caption{DBLP KG}
% 		\label{fig:dblp_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity.pdf}
% 		\caption{YAGO KG }
% 		\label{fig:yago_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity.pdf}
% 		\caption{DBpedia KG}
% 		\label{fig:dbpedia_diversity}
% 	\end{subfigure}
	 
% 	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
% 	\label{fig:diversity}	
% \end{figure*}

\begin{figure*}[t]
\vspace*{-2ex}
	\centering
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity2.pdf}
		\caption{DBLP KG}
		\label{fig:dblp_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity2.pdf}
		\caption{YAGO KG }
		\label{fig:yago_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity2.pdf}
		\caption{DBpedia KG}
		\label{fig:dbpedia_diversity2}
	\end{subfigure}
	 \vspace*{-3ex}
	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
	\label{fig:diversity2}	
 \vspace*{-2ex}
\end{figure*}

\subsection{Systems Time Performance}
\input{tables/maestro_timev2}
This experiment analyzes the time taken by Maestro and {\sysName} to produce benchmarks of $100$ questions for different KGs, \autoref{tab:maestro_time} shows the time taken in hours by both systems. Maestro first needs to traverse the whole KG. It extracts all predicates with their context, a context defined as (predicate, subject\_type, object\_type).  All contexts are saved in PostgreSQL Database for subsequent access. Then, the required number of seed entities is retrieved from the Database and the benchmark generation process starts. In \autoref{tab:maestro_time}, we show the number of predicates processed by Maestro per KG, for DBLP and YAGO we included all predicates, while for DBpedia we stopped at $18,211$ out of $994,592$ predicates for memory limitations, but the whole process needs days to finish. Maestro time is dominated by this preprocessing, and it is proportional to the number of predicates. {\sysName} uses the information in the entire KG on the fly, and needs minutes to run the end-to-end generation process, regardless of the size of the target KG. This order of magnitude improvement in running time can be attributed to the seed sampling process explained in \autoref{sec:seed}. It eliminates the need to perform any pre-processing step, while the validation of the extracted seeds ensures that the seeds are good enough to create meaningful questions.

\subsection{Summarization}
In the following experiments, We evaluate the effect of subgraph summarization on the cost (number of tokens), time to complete benchmark generation, and percentage of correct SPARQL queries generated by LLMs.
\input{tables/subgraph_vs_summarized}

\subsubsection{Cost Efficiency}
The cost is defined as the number of tokens sent to and returned from the LLM in each end-to-end pipeline. To evaluate the cost of the two approaches, we report the average, minimum, maximum, and total number of tokens needed to generate benchmarks of 20 dialogues ( $\approx$ 100 questions) As shown in \autoref{tab:comp}, {\sysName} consistently has lower costs across the different KGs. This demonstrates the efficiency of summarizing the subgraph. There is a cost difference between YAGO and DBLP, although both are generated using the same number of dialogues. This can be attributed to the longer DBLP labels, e.g. paper titles.

\subsubsection{Answer Correctness}
We evaluate the subgraph and summarized approaches with respect to generating syntactically correct SPARQL queries that retrieve the answer to the questions. We validate the queries by executing them against the remote KG endpoint, and only correct question-query pairs exist in the benchmark. If a query fails to execute, it's considered a syntax error. If it executes but returns a different answer than the one stored in the subgraph, it's marked as incorrect. Otherwise, it's considered correct. \autoref{tab:comp} shows the percentage of correct queries generated by {\sysName}  and the subgraph approach across the three KGs. {\sysName}  outperforms the subgraph approach in all KGs. This improvement arises from removing the answer when creating the summarized subgraph, which reduced LLMs confusion. In general, both {\sysName}  and the subgraph approach perform better on YAGO compared to DBLP. This can be attributed to two factors: \myNum{i} YAGO's domain (general knowledge) is more similar to the data the LLMs were trained on, and \myNum{ii} the long labels for publication names in DBLP can confuse the LLM during processing the subgraph.

\subsubsection{Time Efficiency}
We compare the average time taken by {\sysName} and the subgraph approach to generate one dialogue with its SPARQL queries. This time is divided into processing time of the LLM and network latency if the LLM resides on a remote server.  \autoref{tab:comp} shows that both approaches needs comparable time to generate dialogues, as the network latency dominates the time.

\subsection{LLMs}
This experiment shows how our multi-stage approach for optimizing Retrieval Augmented Generation (RAG) systems for complex tasks such as dialogue generation from KGs helps models perform better, especially for less powerful and open source models. We focus on working with open source models since they make LLM solutions more affordable, especially for organizations’ long term projects which will cost a lot if it relied on commercial models. Also, from a security perspective, this will eliminate the need to send private data to external APIs. To show the improvement in performance, we compare our multi-stage approach to the one-stage approach (Providing the LLM with a subgraph and prompting it to generate dialogue questions with its corresponding SPARQL queries) using multiple LLMs of different sizes and two KGs of different domains: YAGO and DBLP. We tested it with commercial models (GPT-3.5, GPT-4, GPT-4o, Gemini-Pro-1, Gemini-Pro-1.5) and open-source models (LLAMA-2 (13B), LLAMA-3 (8B), LLAMA-3-instruct (8B), CodeLLAMA (7B/13B), Mistral-v0.1 (7B)). 

\autoref{tab:openllm} summarizes the performance of the LLMs on both multi-stage and one-stage approaches for different domains. Dialogues-S is the number of successfully generated dialogues. Success rate is the proportion of successful dialogue generation attempts. A higher success rate reflects the LLM's ability to generate Dialogues-S while skipping few or no seed entities. Questions-E, Triples-E, and Dialogue-E are the number of validation errors skipped for question, triples, and dialogue generation, respectively. Parsing-E is the number of cases where LLMs fail to return a correctly structured response. Time is the total time taken by {\sysName} to generate the benchmark in minutes. Number of tokens is the total token count sent to and returned from the LLMs in millions to generate the benchmarks.  For this experiment, we asked the LLM to generate benchmarks of $20$ dialogues, each containing a maximum of $5$ questions. To ensure a finite generation, we set a limit of 500 seed entities for multi-stage and $1000$ for one-stage. If the limit is reached before generating the $20$ dialogues, we stop the process.

As shown in \autoref{tab:openllm}, the overall success rate for all open source LLMs using the multi-stage approach is better than the one-stage approach. This shows that dividing the complex dialogue generation task to simpler tasks (question-triple, SPARQL, dialogue generation) enables the LLMs to successfully generate the required outputs. Additionally, for most LLMs, the number of validation errors caught in each stage is less than the number of errors generated at the one-stage. Even if LLMs passed all validation checks and successfully generated dialogues, converting the generated text into a structured format proves challenging for some models. This is why dividing the tasks into simpler tasks that simplify the output led to a decrease in the number of parsing errors in the multi-stage approach. Across open source models, only the LLAMA-3-8b-inst model succeeds in generating $20$ dialogues using the single-stage approach, while all models were successful with the multi-stage approach. The performance trends for both DBLP and YAGO graphs are similar, with DBLP being the more challenging dataset for most LLMs. This can be concluded from the lower success rates in DBLP. This can be attributed to two factors: the similarity of YAGO data (general knowledge) to the LLMs' training data unlike DBLP (academic, domain-specific). And, the long titles of papers and conferences in DBLP likely make it harder for LLMs to understand entity semantics.

The commercial models show a similar pattern to the open source models, where the multi-stage approach helps these models achieve better success rate with less or comparable validation errors. For example, GPT- 4o’s success rate for single-stage for YAGO KG and DBLP KG are $38\%$ and $8\%$, while for multi-stage it is $100\%$ and $95\%$. For these models, the multi-stage approach offers additional advantages of lower cost and time compared to the one-stage approach. Despite requiring only one prompt compared to three in the multi-stage approach, the multi-stage method achieves a significantly higher success rate. This leads to processing fewer nodes, leading to lower cost and time for benchmark generation.

To improve the overall performance of the dialogue generation task using the open source models and decrease the cost of using commercial models. We combined the best performing model from each stage (i.e. models with lower validation error in this stage) to leverage these models' ability to achieve a better overall performance. We tested {\sysName} using two variations of Multi-LLMs where we use different models in each stage of the process. Multi-LLM-1 uses LLAMA-3-instruct (8B) for Question-triple and Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. Multi-LLM-2 uses GPT-4 for Question-triple Generation, LLAMA-3-instruct (8B) for Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. These two variations achieve comparable performance to commercial models. Multi-LLM-1 uses only open source models, and Multi-LLM2 uses GPT-4 for only one stage which decrease the cost. This flexibility to use different models in different stages allows LLM-based systems like {\sysName} to generate more complex outputs while achieving better performance and success rate at a lower cost.


==> sections/evaluation-simplified.tex <==
\section{Evaluation}
\subsection{{\sysName} Configuration}
{\sysName}  is a configurable benchmark generation framework. It empowers users to generate benchmarks tailored to their specific needs using different settings. Users can create benchmarks containing the required number of questions and targeting various KGs with minimal configuration. To initiate the benchmark generation, users specify the following key parameters: \myNum{i} the KG endpoint URL, \myNum{ii} the number of dialogues, \myNum{iii}  the maximum number of questions per dialogue, \myNum{iv}  the LLM to use per module, and \myNum{v} the workflow type (complex or simplified).

\subsection{Evaluation Setup}
\subsubsection{Compared Systems}
We evaluate {\sysName} against Maestro \cite{maestro}, the state-of-the-art system for generating benchmarks for KGs. The code of Maestro\cite{maestro} is available. The results reported for Maestro are a result of our running of the system.
\subsubsection{Three Different Real KGs}
To evaluate the system's ability to run with KGs of different domains, We use three KGs: DBpedia, Yago, and DBLP. DBpedia and yago are general knowledge graphs. They contain information about people, places, and movies, … etc. DBLP is an academic graph that contains information about scientific publications, authors, and citations. 
\subsubsection{Computing Infrastructure}
We use two different settings for our experiments. In the first setting, We use a Linux machine with $180GB$ RAM and $16$ CPU cores. We use this setting for deploying KGs on virtuoso SPARQL endpoints, running {\sysName} with closed access models i.e. models accessed using APIs, and running Maestro. In the second setting, We use a Linux machine with one Nvidia A100 40GB GPU Card, 32 CPU cores and 64GB RAM. We use this setting to host Open source LLMs, and running {\sysName} with them.
\subsubsection{{\sysName} implementation and settings}
{\sysName} is implemented using Python $3.10$, Lang chain library v$0.1.4$, and OpenLLM library v$0.4.44$ \cite{Pham_OpenLLM_Operating_LLMs_2023} to host the open source LLMs. For SPARQL endpoints, we use Virtuoso v$7.2.5.2$, as it is widely adopted as an endpoint for big KGs. We prepare three different Virtuoso endpoints, one for each of the KGs. The standard, unmodified installation of the Virtuoso engine was used in all of our experiments. For node type selection, we use $1\%$ rare types' threshold, and $99\%$ shadowed parent threshold. For entity and subgraph extraction, we use entity batch size of $10,000$, number of hops is equal to $1$, and outgoing and incoming predicate direction. 
\subsubsection{LLMs}
We evaluated {\sysName} using different LLMs of different sizes. They can be divided into two categories: \myNum{i} Closed access models: GPT-3.5-turbo\cite{radford2018improving}\cite{instructgpt}, GPT-4\cite{openai2024gpt4}, GPT-4o\cite{gpt4o}, Gemini-1-pro\cite{geminiteam2024gemini1}, Gemini-1.5-pro\cite{geminiteam2024gemini15}, and \myNum{ii} Open source LLMs: LLAMA-2-7B \cite{llama2}, LLAMA-2-13B \cite{llama2}, LLAMA-3-8B \cite{llama3modelcard}, LLAMA-3-8B-instruct \cite{llama3modelcard}, CodeLLAMA-7B \cite{codellama}, CodeLLAMA-13B \cite{codellama}, Mistral-7B-v0.1 \cite{mistral}, Mistral-v0.1-instruct \cite{mistral}, Mistral-7B-v0.2 \cite{mistral}, Mistral-v0.2-instruct \cite{mistral}. The closed access models are used via sending requests to their APIs. Open source LLMs are used via sending requests to our server hosting these LLMs.

\subsection{Benchmark Quality}
We evaluated {\sysName}'s ability to generate human-like questions. \autoref{fig:independent_example} shows examples of the generated questions. The textual entity representation plays a crucial role in this ability. Disabling this module and relying on the URI's last segment significantly impacts question quality and clarity, as shown in \autoref{fig:independent_example}. This results in a significant increase in question validation errors, indicating the absence of the entity representation in the generated questions. This demonstrates the importance of a meaningful entity representation to the LLM to comprehend the entity and generate questions. Disabling the module resulted in a significant increase in question validation errors, from $1$ to $109$ for DBLP KG and from $1$ to $51$ for Yago KG. This highlights the effectiveness of textual representations, as a reduction in the number of errors suggests improved LLM understanding and question quality.

We compared the independent questions generated by {\sysName} and Maestro to determine which system produces more human-like questions. \autoref{fig:independent_example} illustrates examples generated by the two systems. All Maestro’s questions for the same seed entity have the same answer, the entity itself. This leads to similar questions asking about the same facts with different rephrasing.
In contrast, {\sysName} asks questions about various facts surrounding the chosen entity. This diversity in facts included in questions suggests {\sysName}'s superior performance. The same pattern persists for the other KGs: Yago and DBpedia. This improvement is attributed to the rich subgraphs with multiple facts used for question generation, and the entity representation module, which empowers the LLM to understand the entity's meaning and rely on its capabilities instead of rule-based approach followed by Maestro.

\begin{figure}[t]
	\begin{verbatim}
Maestro:
1. Who authored the Publication "baraki19"?
2. The authored by of the Publication "baraki19"?
3. Is the Person "8766" the authored by of
the  Publication "baraki19"?
4. What authored by the Person "11171"?
5. Who is the authored by of the Publication "daun18"?

Chatty-Gen using predicate label:
1. Who is the author of Cooperative Situation
Awareness in Transportation?
2. In which year was Cooperative Situation 
Awareness in Transportation published?
3. What is the primary affiliation of Jiaxin Pan?
4. Is Jiaxin Pan associated with any other affiliation?
5. In which journal was 'Trust-Region Methods
on Riemannian Manifolds.' published?

Chatty-Gen without predicate label
1. What is the bibtex Type of item Adler12?
2. Who is the author of Adler12?
3. When was the Phdthesis 'Bailer20' published?
4. Which school accepted the thesis in publication
Beck15?
5. In which year was publication Beck15 published?
	\end{verbatim}
	\caption{Examples of independent questions generated by Maestro and {\sysName} with and without using labels for DBLP KG.}
	\label{fig:independent_example}
\end{figure}

We evaluated {\sysName} and Maestro with respect to the question types covered in their generated benchmarks. \autoref{fig:coverage} illustrates the distribution of question types (question words) for both systems on the three KGs: DBLP, Yago, and DBpedia. We group questions that does not start with a question word into categories. Examples include Yes/No questions (We refer to it as Boolean) starting with \textit{is, did, …, etc.}, and questions starting with nouns (we refer to it as Noun) such as \textit{through, the, by, ..., etc.} As shown in Figures \ref{fig:yago_maestro_complexity} and \ref{fig:dblp_maestro_complexity}, Maestro has a bias towards boolean questions for YAGO and DBLP, whereas {\sysName} produces a less biased distribution. For DBpedia, we compared the benchmark question types generated by the two systems with the human generated QALD-9 dataset (\autoref{fig:maestro_complexity}). While QALD-9 offers a wider variety of question types than either system, {\sysName} still demonstrates a good variation, despite being automatically generated. Notably, Maestro's bias towards boolean questions persists, generating a higher percentage of boolean questions compared to the average in question answering benchmarks. For example, QALD-9 contains only $3\%$ boolean questions, while Maestro generates $34\%$. In contrast, {\sysName} produces a more typical percentage of boolean questions. {\sysName}’s consistency across the three KGs suggests its ability to work with different KGs from various domains.

\begin{figure*}[t]
\centering
   \begin{subfigure}{.3\textwidth}
   	\centering
   	\includegraphics[width=\columnwidth]{figures/maestro_complexity_yago.pdf}
   	\caption{YAGO KG}
   	\label{fig:yago_maestro_complexity}
   \end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dblp.pdf}
	\caption{DBLP KG}
	\label{fig:dblp_maestro_complexity}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
	\centering
	\includegraphics[width=\columnwidth]{figures/maestro_complexity_dbpedia.pdf}
	\caption{DBpedia KG}
	\label{fig:maestro_complexity}
	\end{subfigure}
	\caption{Comparison of the coverage of question types generated by Maestro and {\sysName} for the three KGs.}
	\label{fig:coverage}
\end{figure*}

{\sysName} effectively generates high-quality dialogues that mimic human conversations. \autoref{fig:example} shows examples of the generated dialogues for DBLP and YAGO KGs. The questions within the dialogue are relevant and form a coherent discussion about various facts related to one entity.\shorten

% \begin{figure}[t]
% 	\begin{verbatim}
% 		Example YAGO:
% 		1. What is the birth place of Charlie Chaplin?,
% 		2. What is his nationality?,
% 		3. What are his alternate names?,
% 		4. What awards did he receive?,
% 		5. When did he die?
		
% 		Example DBLP:
% 		1. What is the bibtex Type of 'An Adaptive Hierarchical
% 		Approach to the Extraction of High Resolution Medial
% 		Surfaces.'?,
% 		2. How many creators does it have?,
% 		3. Is it listed on the Toc Page?,
% 		4. What is the year of publication?,
% 		5. In which event was it published in 2012?
% 	\end{verbatim}
% 	\caption{Examples of generated questions by {\sysName} for the different KGs.}
% 	\label{fig:example}
% \end{figure}

% yago - gpt-4 example
% dblp - gpt-4 example
\begin{figure}[t]
	\begin{verbatim}
Example YAGO:
1. Where was Arthur Stuart-Menteth Hutchinson born?
2. What alternate names are known for him?
3. What was the occupation of him?
4. When did he die?
5. Where did he pass away?

Example DBLP:
1. What type of work is 'Systems of Logic Based on -
-Ordinals.' classified as in Bibtex?
2. Who authored it?
3. What is the DOI of it?",
4. In which year was it published?
5. How many creators were involved in it?
	\end{verbatim}
	\caption{Examples of generated questions by {\sysName} for the different KGs.}
	\label{fig:example}
\end{figure}


\subsection{Node type Distribution}
We evaluate the seed node selection module in {\sysName} and Maestro to ensure the chosen node types reflect the node type distribution in the KG. \autoref{fig:diversity2} illustrates how the KG node type distribution compare to {\sysName} and Maestro. We obtain node types by querying the KG endpoint for each chosen entity and calculating the percentage of each type. We only include non-rare types(i.e., types exceeding $1\%$ in the KG). For {\sysName}, most types closely match the KG distribution. However, some differences exist because some nodes have multiple types, so a single seed contributes to multiple types. On the other hand, Maestro does not include many seeds from the most representative types in the KG. For instance, the Person type, constituting $18\%$of DBpedia KG entities, is absent from Maestro's benchmark. Maestro generates a high percentage of rare types, like Social Person ($26\%$ of its benchmark). To simplify the figure, we excluded types existing in the KG less than $5\%$ 

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity.pdf}
% 		\caption{DBLP KG}
% 		\label{fig:dblp_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity.pdf}
% 		\caption{YAGO KG }
% 		\label{fig:yago_diversity}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{.3\textwidth}
% 		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity.pdf}
% 		\caption{DBpedia KG}
% 		\label{fig:dbpedia_diversity}
% 	\end{subfigure}
	 
% 	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
% 	\label{fig:diversity}	
% \end{figure*}

\begin{figure*}[t]
	\centering
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dblp__maestro_diversity2.pdf}
		\caption{DBLP KG}
		\label{fig:dblp_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/yago__maestro_diversity2.pdf}
		\caption{YAGO KG }
		\label{fig:yago_diversity2}
	\end{subfigure}
	\hfill
	\begin{subfigure}{.3\textwidth}
		\includegraphics[width=\columnwidth]{figures/dbpedia__maestro_diversity2.pdf}
		\caption{DBpedia KG}
		\label{fig:dbpedia_diversity2}
	\end{subfigure}
	 
	\caption{Comparison of the distribution of the node types used in the KG, the node types sampled by {\sysName} and the node types of the seed entities chosen by Maestro}
	\label{fig:diversity2}	
\end{figure*}

\subsection{Systems Time Performance}
\input{tables/maestro_timev2}
This experiment analyzes the time taken by Maestro and {\sysName} to produce benchmarks of $100$ questions for different KGs, \autoref{tab:maestro_time} shows the time taken in hours by both systems. Maestro first needs to traverse the whole KG. It extracts all predicates with their context, a context defined as (predicate, subject\_type, object\_type).  All contexts are saved in PostgreSQL Database for subsequent access. Then, the required number of seed entities is retrieved from the Database and the benchmark generation process starts. In \autoref{tab:maestro_time}, we show the number of predicates processed by Maestro per KG, for DBLP and YAGO we included all predicates, while for DBpedia we stopped at $18,211$ out of $994,592$ predicates for memory limitations, but the whole process needs days to finish. Maestro time is dominated by this preprocessing, and it is proportional to the number of predicates. {\sysName} uses the information in the entire KG on the fly, and needs minutes to run the end-to-end generation process, regardless of the size of the target KG. This order of magnitude improvement in running time can be attributed to the seed sampling process explained in \autoref{sec:seed}. It eliminates the need to perform any pre-processing step, while the validation of the extracted seeds ensures that the seeds are good enough to create meaningful questions.

\subsection{Summarization}
In the following experiments, We evaluate the effect of subgraph summarization on the cost (number of tokens), time to complete benchmark generation, and percentage of correct SPARQL queries generated by LLMs.
\input{tables/subgraph_vs_summarized}

\subsubsection{Cost Efficiency}
The cost is defined as the number of tokens sent to and returned from the LLM in each end-to-end pipeline. To evaluate the cost of the two approaches, we report the average, minimum, maximum, and total number of tokens needed to generate benchmarks of 20 dialogues ( $\approx$ 100 questions) As shown in \autoref{tab:comp}, {\sysName} consistently has lower costs across the different KGs. This demonstrates the efficiency of summarizing the subgraph. There is a cost difference between YAGO and DBLP, although both are generated using the same number of dialogues. This can be attributed to the longer DBLP labels, e.g. paper titles.

\subsubsection{Answer Correctness}
We evaluate the subgraph and summarized approaches with respect to generating syntactically correct SPARQL queries that retrieve the answer to the questions. We validate the queries by executing them against the remote KG endpoint, and only correct question-query pairs exist in the benchmark. If a query fails to execute, it's considered a syntax error. If it executes but returns a different answer than the one stored in the subgraph, it's marked as incorrect. Otherwise, it's considered correct. \autoref{tab:comp} shows the percentage of correct queries generated by {\sysName}  and the subgraph approach across the three KGs. {\sysName}  outperforms the subgraph approach in all KGs. This improvement arises from removing the answer when creating the summarized subgraph, which reduced LLMs confusion. In general, both {\sysName}  and the subgraph approach perform better on YAGO compared to DBLP. This can be attributed to two factors: \myNum{i} YAGO's domain (general knowledge) is more similar to the data the LLMs were trained on, and \myNum{ii} the long labels for publication names in DBLP can confuse the LLM during processing the subgraph.

\subsubsection{Time Efficiency}
We compare the average time taken by {\sysName} and the subgraph approach to generate one dialogue with its SPARQL queries. This time is divided into processing time of the LLM and network latency if the LLM resides on a remote server.  \autoref{tab:comp} shows that both approaches needs comparable time to generate dialogues, as the network latency dominates the time.

\subsection{LLMs}
% Paragraph 1: how to read the table 
% Paragraph 2: Overview of the dimensions we explored
% Paragraph 3: Fixing LLM, Changing domain
% Paragraph 4: Fixing LLM, chaning complexity
% Paragraoh 5: Fixing domain, getting the highest performing models. 
% The size, the instruct

% our goal for these section is to explain the results with following highlevel dimensions
% one dimension - from yago to dblp 
% second dimension - granularity/complexity of instruction task- affect or not
% third dimension - size of the model + model variation
% so we will have 3 para one for each dimension in mind - with citation in each for effect of that dimension results in differnet performance, with overview para at the beginning of it as intro to our approach towards understanding of the table. 
% a para to explain what is each column and how to read each row. considering the seed is not equal to question error plus triple error plus parsing error. 
% and after these we will have patterns related paragraph
% ##TODO: unify the model names across paper by referring the publication

% {\sysName} provides the flexibility to generate benchmarks using different LLMs. We evaluated the ability of Llama-7b, Llama-13b\cite{llama2}, CodeLlama-7b, CodeLlama-13b\cite{codellama}, and Mistral-7b-v0.1\cite{mistral} models to perform the benchmark generation task within the {\sysName} pipeline. We generated the benchmarks to evaluate each model for the two KGS: Yago and DBLP. We evaluate them on the quality of the generated questions, the percentage of correctly generated SPARQL queries, and the number of seed nodes used to successfully generate given number of dialogues, skipping a node due to different errors in the LLM output. 

% % From ... it is known as performance of large language models is influenced by various factors, in the context of our evaluation it can be broadly categorized into following three groups. 1. LLM's capabilities, 2. Domain of 

% The LLMs produce different quality of questions in dialogues. Llama-7b, CodeLlama-7b, and Mistral-7b-v0.1 tend to use the predicate as it is in the questions, while Llama-13b and CodeLlama-13b produce questions that seem to follow a certain template. {\color{red} Add more explanation after further evaluation}


% As explained in \autoref{sec:subgraph_approach}, wrong query generation leads to discarding questions within the dialogue. \autoref{tab:llm_query} shows the percentage of correct SPARQL queries generated by each LLM for each Yago and DBLP KGs. Gpt-3.5 produced the best percentage in the two KGs. From the open-source LLMs, CodeLLama-13b has the best performance across openLLMs. CodeLLama-7b and Mistral-7b-v0.1 have comparable performance. Mistral-7b-v0.1 is the only LLM to maintain its percentage across the two KGs, it was not affected by the change in domain or length of the labels. LLama-7b and LLama-13b could not produce any dialogues for DBLP while having very low percentages for YAGO. 


% As shown in \autoref{fig:framework}, each LLM-based component is associated with a validator to ensure the correctness of LLM output before moving forward in the pipeline. \autoref{tab:openllm} shows the different errors caught by the validators for different steps in the pipeline. The included errors are those that cause skipping of the current seed entity and replacing it with another one. openLLMs struggle with the first step of the pipeline due to its complexity. We designed an updated version of our pipeline that divides the first module into two tasks: \myNum{i} generating independent questions, and \myNum{ii} choosing the triple associated with each question. As shown in the second part of \autoref{tab:openllm}, the simplified pipeline enabled the LLMs to bypass the first module and move through the rest of the pipeline steps {\color{red} The only LLM benefiting from this is Llama-7b}. The bottleneck module for the considered LLMs is the SPARQL generation module. Some LLMs such as {\color{red} Add examples}, generate queries that use undefined Prefixes, that were not a part of the given triple. To mitigate this issue, we append a set of pre-defined prefixes to the generated query before executing it to test its correctness. Even with this change, only CodeLlama-13b has a reasonable performance for the SPARQL query generation leading to less number of overall skipped entities. 




% intro
We evaluated {\sysName}'s ability to work with multiple LLMs of different sizes. We tested it with closed-access models (GPT-3.5, GPT-4, GPT-4o, Gemini-Pro-1) and open-source models (LLAMA-2 (7B/13B), LLAMA-3 (8B), LLAMA-3-instruct (8B), CodeLLAMA (7B/13B), Mistral-v0.1 (7B)). We analyzed the performance of the models to identify the best performing models. Then we tested {\sysName} with two variation of using different LLMs for each stage. Our first variation is using  LLAMA-3-instruct (8B) for Question-triple and Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. The second variation is using GPT-4 for Question-triple Generation, LLAMA-3-instruct (8B) for Dialogue Generation, and CodeLLAMA(13b) for SPARQL queries generation. To assess performance, we generated benchmarks consisting of $20$ dialogues, each containing a maximum of $5$ questions. We evaluated with two KGs of different domains: YAGO and DBLP. To ensure a finite evaluation process, we set a limit of $500$ seed entities. If this limit was reached before generating the $20$ dialogues, we stop the process.

% how to read the table
\autoref{tab:openllm} shows the results of this experiment, Num\_seeds is the total number of seeds used to successfully generate the $20$ dialogues. Dialogues-S is the number of successfully generated dialogues, since some models reaches the limit of $500$ before generating all $20$ dialogues. Questions-E and Triples-E are the number of validation errors skipped for the question and triples generation, respectively. Parsing-E identifies the cases where LLMs failed to return a correctly structured response. Time is the total time taken by {\sysName} to generate the benchmark in minutes. Number of tokens is the sum total number of tokens sent to and returned from the LLMs in millions to generate the benchmarks.  The table shows the performance of each LLM across domains (YAGO and DBLP), and across complex (\autoref{sec:workflow}) and simplified (\autoref{sec:prompts}) pipelines.

\autoref{tab:openllm} shows that GPT-3.5, GPT-4, and GPT-4o are not affected by changes in domain or task complexity. For Gemini-Pro-1 and open-source LLMs, performance is impacted by change of domain, with most models performing better on YAGO KG. This is due to similarity between YAGO data (general knowledge) to the LLMs’ training data, unlike DBLP (academic, domain-specific data). DBLP also contains long titles of papers and conferences (longer than average entity length in YAGO) which can confuse LLMs and reduce performance. These models are also affected by pipeline complexity change, they perform better with the complex pipeline which requires fewer prompts. This is likely because of the higher number of prompts, which increases the probability of LLM hallucinations. The complex pipeline requires $7$ prompts ($1$ question and triples, $5$ SPARQL, and $1$ dialogue) while the simplified requires $12$ prompt ($1$ question, $5$ triples, $5$ SPARQL, and $1$ dialogue). The simplification has the potential to improve the performance of LLMs, but it is preferred in single prompt solutions where a task can be broken down to minimal number of subtasks.  Overall, the top performing LLMs across both KGs are GPT-3.5, GPT-4, GPT-4o, CodeLLama (13b), and Gemini-Pro-1. These models require less than 100 seed entities to process before generating 20 dialogues. Using variations of LLMs for different stages can achieve comparable performance to the top performing models at a lower cost. For example, Multi-LLM-2 variation leverages the code generation ability of CodeLLama's (13b) for SPARQL queries and the natural language capabilities of LLAMA-3 instruct (8B) for dialogue generation, requiring GPT-4 only for the complex question-triples generation task.


% % changing the complexity | second statement is wrong as it just reduces question error with trend
% The Simplified approach doesn't help already very good and very bad performing models, for example CodeLLAMA-13b and LLAMA-2-7b respectively. It only helps only average performing models to limit the question and triple validation errors by their independent generation. With simplified approach, the question json errors always decreases or stays the same for almost all the models, with CodeLLAMA-7b having the biggest decrease for DBLP KG. <some words about triple errors>

% % changing the model's variation (size and type)
% Our evaluation shows that while keeping the same approach and a domain, by changing the model's size or variation the performance of it degrades or increases by a lot. LLAMA-3-8b-inst is instruction fine-tuned variation of LLAMA-3-8b, and it always performs better than LLAMA-3-8b, except in simplified approach and DBLP KG, where it struggles to parse the triples and performs very badly. But with CodeLLAMA-7b and CodeLLAMA-13b models which are pretrained for code infilling and long context fine-tuning, from LLAMA-2, performs best among all the open source models just by changing the size from 7b to 13b.


% % multi-llm-paragraph
% {\sysName} provides the flexibility to generate benchmarks using different LLMs for every stage of the pipeline. Our multi-llm experiments shows that with the use of multiple opensource models, compatible with associated stages, leads to best and comparable performace with very big private api based LLMs. With combination of using llama-3-8b-inst for question-triple geneation and dialogue generation, and codellama-13b for sparql query generation leads to best performance. 


 

==> sections/introduction-reham.tex <==
\section{Introduction}
Conversational AI systems, including chatbots (e.g., ChatGPT\cite{chatgpt} and Gemini\cite{gemini} and virtual assistants (e.g., Alexa and Siri), aim to hold natural conversations with users on a wide range of topics. These conversations provide general information or enable users to complete specific tasks\cite{chatgpt_survey}. Although many users report positive experiences with conversational AI systems, there is a need for a systematic way to evaluate the quality of these interactions. This highlights the importance of dialogue benchmarks that can assess conversational AI systems' ability to understand user requests, leverage the full conversational context, and provide accurate and relevant responses. However, most of the existing dialogue benchmarks focus on information retrieval from documents, such as Dream\cite{dream}, and MultiWOZ\cite{multioz}, neglecting the potential of Knowledge Graphs (KGs). 

KGs incorporate a vast amount of data in many specialized domains (e.g., medical or financial). This specialized data has the potential to significantly improve the performance of general virtual assistants\cite{p_assistant}. Dialogue benchmarks can be used to train chatbots capable of engaging in multi-turn conversations \cite{dialogue_training} within a specific domain, extending beyond simple question-answering tasks. These benchmarks encourage applications like online tutoring\cite{tutoring} by creating educational exams and the development of educational chatbots\cite{edu_chatbot}. Furthermore, dialogue benchmarks can be used for various KG exploration tasks, such as onboarding new users to existing KGs\cite{AttnIO}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/example.pdf}
\caption{An illustration of the steps needed to create a dialogue from an entity belonging to DBpedia KG.}
\label{fig:example1}
\end{figure}

Automating dialogue benchmark generation on KGs presents unique challenges. KGs contain real-world entities interconnected by diverse relationships. Both entities and relationships are represented using Uniform Resource Identifiers (URIs). \autoref{fig:example1} outlines the steps involved in generating a dialogue from the DBpedia KG using an example: \myNum{1} \textbf{Sample Entities:} The first step involves sampling entities from the KG. The huge number of entities in KGs makes including them all in benchmarks impractical. Therefore, selecting a representative sample of entities spanning the important KG node types becomes crucial. Our example shows a node from Person type \myNum{2} \textbf{Extract Context:} The second step involves extracting subgraphs surrounding the chosen entity. These subgraphs represent the context of the dialogue. (3) \textbf{Extract Textual Entities Representation:} To generate a question about an entity, we need a human-readable representation for it. Using URIs (e.g. \url{http://dbpedia.org/resource/Celine_Dion}) within natural language questions is impractical, necessitating a more user-friendly representation (e.g. Celine Dion) as shown in \autoref{fig:example1}. \myNum{4} \textbf{Maintain Dialogue Flow:} The generated questions should remain relevant and build upon each other within the dialogue. The primary entity can be explicitly introduced once, with subsequent questions referring to it indirectly. In our example, the entity is mentioned clearly in the first questions while subsequent questions refer to it using \textit{“she”} or \textit{“her”} \myNum{5} \textbf{Generate Answers:} Generating complete benchmarks requires answers for each question. Within the context of KGs, retrieving answers involves utilizing SPARQL queries. This necessitates formulating SPARQL representations corresponding to each question generated. \myNum{6} \textbf{KG Agnostic Design:} The dialogue generation platform should be able to operate on any KG without requiring KG-specific modifications. 

\input{tables/background_v2}

Existing dialogue benchmarks on documents, such as CoQA\cite{coqa} and QuAC\cite{quac}, rely on manually generated questions and answers. CSQA\cite{csqa}  a semi-automatic dialogue benchmark for the Wikidata KG, continues to be labor-intensive and KG-dependent. It requires manually designed templates to identify interconnected predicates within the KG. Single-question benchmarks for KGs \cite{qald9, lcquad, lcquad2, head_to_tail} face similar limitations. QALD-9\cite{qald9} is manually created, others like LCQuAD\cite{lcquad, lcquad2} and Head-to-Tail\cite{head_to_tail} use templates. Template-based approaches struggle with arbitrary KGs, requiring redesign of templates for each new KG. Head-to-Tail chooses entities based solely on node popularity, without taking entity types in consideration. Maestro\cite{maestro} is an automatic system for single-question benchmark generation on KGs. However, it requires a pre-processing step, proportional to the number of unique predicates in the KG, to extract the required entities. Maestro sample entities spanning a limited set of entity types, making the benchmark less comprehensive. Additionally, Maestro relies on pre-defined question shapes that does not exist in all KGs. This results in generating complex questions that make it difficult for both users and systems to generate comprehensive answers given the context. To choose the suitable textual entity representation in the question, Maestro requires users to provide how to extract this representation. This limits its adaptability to run with arbitrary KG. Both Maestro and template-based benchmarks require prior knowledge of the answer (entity) to generate questions. This hinders their application for dialogue generation, since all generated questions for an entity will share the same answer.

To address these limitations, we propose {\sysName}, a novel platform that automatically generates dialogue benchmarks on arbitrary KGs. {\sysName} leverages Large Language Models (LLMs) across its stages. {\sysName} dynamically select entities considering the distribution of node types within the KG, allowing it to work with arbitrary KGs. It automatically predicts textual representation of entities, resulting in human-friendly questions. To maintain context and generate simple questions suitable for dialogues, {\sysName} relies on condensed subgraph shapes. Furthermore, by efficiently encoding the subgraph in a summarized way, {\sysName} leverages richer subgraphs to generate comprehensive dialogues. {\sysName} generates queries for each question without requiring prior knowledge of the answer. {\sysName} divides the benchmark generation process into multi stages to simplify the task and make it compatible with a wide range of LLMs regardless of their capabilities. To overcome the hallucination potential of LLMs, {\sysName} uses assertion based validation modules. These modules ensure the correctness of the LLM output by verifying it against pre-defined constraints.

We evaluate {\sysName}'s performance on three diverse real-world KGs: DBpedia, Yago, and DBLP. Our experiments demonstrate that using textual entity representation improves the quality of the generated questions. Moreover, the generated questions exhibit a diverse entity type distribution, including all KG node types that exceed a user defined percentage. {\sysName} produces a wide variety of question types, enabling it to effectively challenge chatbot systems. Furthermore, {\sysName} demonstrates efficient time performance in end-to-end benchmark generation compared to Maestro (state-of-the-art system), especially for large KGs such as DBpedia which shows a time improvement of 99\% (from $30$ hours to $10$ minutes). Finally, we explore {\sysName}'s compatibility with different LLMs by evaluating its performance with both commercial models such as Gpt-4o\cite{gpt4o}, and Gemini-pro-1.5\cite{geminiteam2024gemini15} and open-source models such as Llama-3\cite{llama3modelcard}, and CodeLLama\cite{codellama}. This flexibility empowers users to work on various KGs and leverage different LLMs. 
Our key contributions are:
\begin{itemize}
\item Introducing the first platform for automatically generating dialogue benchmarks from KGs based on LLMs; Section 3.
\item Effective and diverse context retrieval method for selecting representative seed nodes with rich subgraphs from the KG with minimal overhead; Section 4.
\item Carefully designed multi-step dialogue generation workflow with automatic assertion-based validation, and adopted the workflow with LLMs of different capabilities; Section 5. 
\item A comprehensive evaluation using three real KGs from different domains, and different LLMs. {\sysName} can work with arbitrary KGs in timely performance regardless of the size of the KG; Section 6. 
\end{itemize}

==> sections/overview-old.tex <==
 \section{The {\sysName} Platform Overview}
This section provides an overview of the key characteristics of conversational benchmarks for KGs, and how {\sysName} utilizes LLMs and KGs to automatically generate these benchmarks. The benchmarks consist of dialogues, where each dialogue includes questions with their corresponding SPARQL queries to retrieve the answers to these questions.

\begin{definition}[Independent Question]
\label{def:independent}
An independent question $(Q_{In})$ is a question that can be answered directly from the KG without requiring any additional context. All information needed to retrieve the answer is present within the question itself.
\end{definition}

\begin{definition}[Dependent Question]
\label{def:dependent}
A dependent question $(Q_{Dep})$ is a question that cannot be answered solely based on the KG. It requires an associated context $(C)$ to provide the necessary information for retrieving the answer from the KG.
\end{definition}

\begin{definition}[Dialogue]
A Dialogue $D(e) = \{e, Q, SQ\}$ where:
\begin{itemize}
    \item Seed Entity $e$: The seed entity the dialogue asks about.
    \item Questions $Q$: An ordered list of questions asked during the dialogue, denoted as $Q = [Q_1, Q_2, . . . , Q_n]$. $Q_1$ must be an independent question. Subsequent questions ($Q_i$ where $i > 1$) must be dependent on the dialogue flow.
    \item SPARQL Queries ($SQ$): A list of SPARQL queries corresponding to each question in $Q$.
\end{itemize}
\end{definition}

\subsection{Benchmark Characteristics}
For conversational benchmarks to effectively challenge systems, the following characteristics are essential. 

\subsubsection{Coverage of Different Question Types:} 
The benchmark should include questions that vary in complexity to comprehensively evaluate the chatbot’s ability to answer different questions. This allows evaluating the chatbot's understanding of the question and its proficiency in retrieving accurate information from the KG. Question complexity can be defined by  question types. Examples of different types include count questions, listing questions, and WH questions. Each type requires a distinct approach from the chatbot to answer. For example, listing questions demand returning all relevant answers, while count questions only require the number of answers. 

\subsubsection{Grounded Facts:}
For the benchmark to effectively evaluate chatbots’ accuracy, answers to questions must exist in the target KG. This ensures that the chatbot is leveraging the KG and not generating answers based on its training data or irrelevant information.\shorten

\subsubsection{Diversity of Nodes:} 
A diverse benchmark assess chatbots' flexibility to deal with KG nodes of different types and surrounding structures. Although an ideal benchmark would encompass all KG nodes, this is impractical for KGs containing thousands of types. This necessitates a sampling approach that ensures the chosen sample accurately reflects the distribution of node types within the KG. Thus, the benchmark effectively tests chatbots' ability to answer questions about diverse nodes within the KG.

\subsubsection{Linguistic and Grammatical Correctness:} 
Language correctness within the benchmark’s questions is vital for ensuring a fair and accurate assessment of KG chatbots. Testing with incorrect language hinders objective evaluation.

\subsection{{\sysName} Overview }
{\sysName} follows the four steps for automatically generating conversational benchmarks: context extraction, entity representation, dialogue generation and answer generation as shown in \autoref{fig:framework}. In contrast to existing systems that rely on rules or templates to generate questions, {\sysName} leverages LLMs by providing them with the necessary inputs to successfully generate dialogue. Additionally, the lack of manual effort and pre-processing steps in the process enables {\sysName} to work with arbitrary KGs. 

\textbf{Context Extraction and Entity Representation.} 
{\sysName} uses a node-type-based approach for context extraction, eliminating the pre-processing step, and improving efficiency. It starts by selecting node types from the given KG at runtime. It maintains the distribution of node types within the KG. {\sysName} then leverages LLMs to extract a predicate for each node type, since different node types are represented by different predicates. This predicate is used to extract the textual representation of the KG entities belonging to this type, making it easier for LLMs to process the extracted context. For each node type, {\sysName} selects nodes belonging to that type with their textual representation, at runtime by querying the KG through its SPARQL endpoint. {\sysName} uses the extracted entities to retrieve the surrounding subgraphs, which represent the context for question generation within a dialogue. 

\textbf{Dialogue and Answer Generation.} To generate the dialogue, {\sysName} utilizes the extracted subgraph and textual representation, and leverages LLMs in a multi-stage pipeline. Since LLMs are prone to hallucinations, each subsequent step includes a validator module to ensure the correctness of the generated output. Correctness is defined based on the previously explained benchmark characteristics and LLM limitations. The subgraph is fed to the summarization module, which keeps only information that can help LLM achieve the required task and eliminates any possible confusions. This summarized subgraph is then fed to the independent question generation module, which also utilizes the LLM to generate a set of independent questions about different facts within the summarized subgraph. Each question is linked back to the specific triple in the subgraph from which it was generated. Next, the questions along with their corresponding triples are provided to the answer generation module. This module generates a SPARQL query for each question, which retrieves the answer to the question from the KG. Finally, the dialogue generation module transforms the set of independent questions into a dialogue while keeping the first question independent since it is the dialogue starting point. 

The final benchmark dataset consists of three components: dialogue, independent questions, and corresponding SPARQL queries. The conversational and independent questions inquire about existing KG facts related to the seed entities. The SPARQL queries, retrieve the answers from the target KG.

==> sections/related_work-reham.tex <==
\section{Related Work}
\subsection{Benchmarking}
There is a growing effort in developing benchmarks for different AI tasks. Our task involves creating dialogue benchmarks on KG. To address that, we need to consider two aspects: dialogue nature of questions and KG related information. Among the early efforts for document based conversational benchmarks are the manually created CoQA\cite{coqa} and QuAC\cite{quac} datasets. System answering the question on these datasets leverages the dialogue history to correctly answer them. There has been a growing interest in generating single questions and dialogue benchmarks on KG, some datasets are manually generated while others are template based.  Single questions datasets on KGs include QALD\cite{qald9}, LCQUAD\cite{lcquad, lcquad2} on DBpedia\cite{dbpedia} KG, DBLP-QuAD \cite{dblpquad} on DBLP KG  and WEBQUESTIONSSP \cite{webquestions} on Freebase KG. QALD is a multilingual manually generated dataset on DBpedia KG version $2016-10$. LCQuAD 1.0\cite{lcquad} is a semi-automated template-based generated dataset on DBpedia  KG version $2016-04$. it contains questions of different complexities. LCQuAD 2.0 builds upon LCQuAD 1.0 by expanding the dataset size to $30,000$ question-query pairs and extending its target KGs to include both Wikidata and DBpedia version $2018$. They have a final step of utilizing  Amazon Mechanical Turk to generate the final questions. DBLP-QuAD\cite{dblpquad} is developed on the DBLP scholarly knowledge graph, It consists of $10,000$ question-answer pairs.  It adopts a template-based generation process, involving a manual step for creating templates based on DBLP KG ontology followed by an automated step for generating questions from those templates. Head-to-Tail benchmark \cite{head_to_tail} is a recent template-based generated benchmark. The benchmark comprises $18k$ question-answer pairs spanning diverse domains and entities of varying popularity. Each question targets specific attributes of an entity. Maestro \cite{maestro} is an automatic rule-based single-question benchmark generation framework for KGs that leverages rules and templates to generate questions given chosen seed entities and subgraphs from the target KG. CSQA \cite{csqa} is an early benchmark generated on Wikidata KG. It is a semi-automated labor-intensive benchmark, which requires a manual KG exploration step, manual template creation, and template-based generation of questions.
 
\subsection{Large Language Models}
Recently, there has been a surge in the development of large language models (LLMs) from early models like Bert\cite{bert} and T5\cite{T5} to powerful recent models like GPT-3\cite{gpt3}, GPT-4\cite{gpt4}, Llama\cite{llama, llama2}, PALM\cite{palm}, and Claude\cite{claude}. Approaches relying on LLMs significantly improved the performance of many NLP tasks in various domains. Using smaller early models on new tasks or domains required fine-tuning the models with task or domain-related datasets, which can be time-consuming and costly. Recent powerful models eliminates the need to perform fine-tuning by using prompting or in-context learning \cite{prompt_survey} which needs less time and cost than fine-tuning. In prompting, users specify the desired task for the LLM in natural language. The prompt can include input-output examples (few-shot learning) or no examples (zero-shot learning). Given prompting's potential to improve LLM performance at lower costs, various prompting techniques have been explored, such as Chain of Thought\cite{cot} and least-to-most prompting \cite{least_to_most}. 

Prompting is now used to achieve state-of-the-art performance in tasks like Text-to-SQL \cite{dinsql, text_sql_cot} and code generation \cite{codegeneration, codegeneration2}. Generally, closed-access commercial models like GPT-4 tend to achieve better results across different tasks. However, they can be costly for tasks involving frequent or lengthy prompts. This has led to a growing focus on improving the performance of open-source models like LLama and Mistral\cite{maestro} to achieve comparable performance to closed-access models in some tasks such as dialogue state tracking \cite{DST}.





==> tables/answer.tex <==
% refer data at /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/subgraph
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/dbpedia/original for dbpedia
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/gpt3.5_triple_update for yago and dblp - chatty-gen

\begin{table*}[t]
  \caption{Comparison between {\sysName} and the subgraph approach in terms of the number of correctly generated SPARQL queries for a benchmark of 20 dialogues}
  \label{tab:answer}
  \begin{tabular}{ccccccc}
    \toprule
       & \multicolumn{2}{c}{\textbf{DBLP}} & \multicolumn{2}{c}{\textbf{YAGO}} & \multicolumn{2}{c}{\textbf{DBpedia}}\\
     \midrule
        & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} \\
    \midrule
    \textbf{Correct} & 68 & 90 & 73 & 86 & 79 & 94\\
    \textbf{Incorrect} & 14 & 6 & 9 & 5 & 18 & 5\\
    \midrule
    \textbf{Correct \%} & 82.9\% & 93.8\% & 89.0\% & 94.5\% & 81.4\% & 94.9\%\\
  \bottomrule
\end{tabular}
\end{table*}



% % old table % %

% \begin{table*}[t]
%   \caption{Comparison between {\sysName} and the subgraph approach in terms of the number of correctly generated SPARQL queries for a benchmark of 20 dialogues}
%   \label{tab:answer}
%   \begin{tabular}{ccccccc}
%     \toprule
%        & \multicolumn{2}{c}{\textbf{DBLP}} & \multicolumn{2}{c}{\textbf{YAGO}} & \multicolumn{2}{c}{\textbf{DBpedia}}\\
%      \midrule
%         & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} \\
%     \midrule
%     \textbf{Correct} & 94 & 86 & 97 & 97& 89 & 93\\
%     \textbf{Incorrect} & 6 & 14 & 3 & 1 & 16 & 12\\
%     \midrule
%     \textbf{Correct \%} & 94.0\% & 86.0\% & 97.0\% & 98.9\% & 84.8\% & 88.6\%\\
%   \bottomrule
% \end{tabular}
% \end{table*}

==> tables/background.tex <==
\begin{table*}[t]
  \caption{A Comparative Analysis Between conversational and KG-based benchmarks}
  \label{tab:back}
  \begin{tabular}{cccc}
    \toprule
    \textbf{Benchmark} & \textbf{Answer Source} & \textbf{Benchmark Creation} & \textbf{Conversational}\\
    \midrule
    \textbf{CoQA\cite{coqa}} & Documents & Manual & \checkmark\\
    \textbf{QuAC\cite{quac}} & Documents & Manual & \checkmark\\
    \textbf{CSQA\cite{csqa}} & KG & Semi-Automated & \checkmark \\
    \textbf{Maestro\cite{maestro}} & KG & Automatic & x \\
    \textbf{Head-to-Tail\cite{head_to_tail}} & KG & Semi-Automatic &x \\
    \midrule
    \textbf{{\sysName}} & KG & Automatic & \checkmark \\
  \bottomrule
\end{tabular}
\end{table*}

==> tables/cost.tex <==
% refer data at /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/subgraph/*
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/dbpedia/original for dbpedia
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/gpt3.5_triple_update for yago and dblp - chatty-gen

\begin{table*}[t]
  \caption{Cost comparison between the subgraph and summarized approaches in terms of the number of tokens for a benchmark of 20 dialogues}
  \label{tab:cost}
  \begin{tabular}{ccccccc}
    \toprule
       & \multicolumn{2}{c}{\textbf{DBLP}} & \multicolumn{2}{c}{\textbf{YAGO}} & \multicolumn{2}{c}{\textbf{DBpedia}} \\
     \midrule
        & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} \\
    \midrule
    \textbf{Average} & 3090.9 & 2733.7 & 3153.8 & 2304.4 & 3438.15 & 2517.65 \\
    \textbf{Minimum} & 1779 & 1910 & 1675 & 1362 & 1868 & 1808\\
    \textbf{Maximum} & 5970 & 7104 & 9247 & 3397 & 10198 & 4179 \\
    \textbf{Total} & 61818 & 54674 & 63076 & 46088 & 68763 & 50353\\
  \bottomrule
\end{tabular}
\end{table*}



%% old table %%

% \begin{table*}[t]
%   \caption{Cost comparison between the subgraph and summarized approaches in terms of the number of tokens for a benchmark of 20 dialogues}
%   \label{tab:cost}
%   \begin{tabular}{ccccccc}
%     \toprule
%        & \multicolumn{2}{c}{\textbf{DBLP}} & \multicolumn{2}{c}{\textbf{YAGO}} & \multicolumn{2}{c}{\textbf{DBpedia}} \\
%      \midrule
%         & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} \\
%     \midrule
%     \textbf{Average} & 2897.1 & 2258.7 & 3897.8 & 1895.55 & 4693.2& 3778.7 \\
%     \textbf{Minimum} & 2215 & 1959 & 2561 & 1365 & 2001 & 1925\\
%     \textbf{Maximum} & 7076 & 2568 & 5920 & 2059 &8098&5073 \\
%     \textbf{Total} & 57942 & 45174 & 77956 & 37911 &98557 & 79352\\
%   \bottomrule
% \end{tabular}
% \end{table*}

==> tables/kg_qa.tex <==
\begin{table*}[t]
  \caption{Testing the generated benchmarks with 20 dialogues using KGQA system KGQAn}
  \label{tab:kgqa}
    \begin{tabular}{cccccccccc}
    \toprule
       &  \multicolumn{3}{c}{\textbf{DBLP}} & \multicolumn{3}{c}{\textbf{YAGO}} & \multicolumn{3}{c}{\textbf{DBpedia}} \\
     \midrule
        & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
    \midrule
    \textbf{Questions} & 90.94 & 19.77& 40.58 & 40.58 & 57.73 & 47.66 & 50.96 & 33.33& 40.30\\
    \textbf{Dialogue} & 93.02 & 4.65 & 8.86  & 81.11 & 13.40 & 23.00 & 85.49 & 8.60 &  15.63\\
    % \midrule
    %  \textbf{Questions-NoFil} & & & & 61.28 & 60.00 & 60.63 & 19.87 & 59.57 & 29.80 \\
    % \textbf{Dialogue-NoFil} & & & & 78.17 & 38.00 & 51.14 & 82.08 & 23.40 & 36.42\\
  \bottomrule
\end{tabular}
\end{table*}
% DBLP-KG Latest values: Dialogue: 93.18 & 30.68 & 46.16, Questions: 85.38 & 32.95 & 47.55
% YAGO latest values: Questions: 40.49 & 59.18 & 48.08, Dialogue: 80.25 & 24.49 & 37.53

==> tables/kg_statistics.tex <==
\begin{table}[t]
  \caption{KG Statistics: The number of entities, and triples in Millions, The number of unique predicates and the total size in GB of each KG.\highlightedReply{}{R1.O3.4, R3.O3, C8}}
  \label{tab:stats}
  \begin{tabular}{ccccc}
    \toprule
    \textbf{Stat} & \textbf{Yago} & \textbf{DBLP} & \textbf{DBPedia} &\textbf{MAG} \\
    \midrule
    \textbf{\# Entities(M)} & 12 &18&14&586\\
    \textbf{\# Triples(M)} &207&263&350&13,705\\
    \textbf{\# Predicates} & 259&167&60,736&178\\
    \textbf{Size(GB)} &27&13&29&637\\
    
  \bottomrule
\end{tabular}
\end{table}
% YAGO: Unique Predicates:  259, Num Entities:  12,598,108, Num Triples:  207029212
% DBPedia: Unique Predicates:  60736, Num Entities:  14,397,265, Num Triples:  350,677,804
% DBLP: Unique Predicates:  167 , Number of Entities:  18,306,226 , Number of Triples:  263,195,019
% MAG: Unique Predicates:  178 , Number of Entities:  568,309,304 , Number of Triples:  13705,145,395


==> tables/llm_detail.tex <==
\begin{table}[t]
\footnotesize
\caption{Characteristics of used LLMs}
\label{tab:llm_details}
\begin{tabular}{c|c}
    \toprule
    \textbf{} & \textbf{Models}  \\
    \midrule
    \textbf{Private} & \textbf{gpt-4o, gpt-4, gpt-3.5} \\
    \textbf{} & \textbf{gemini-1-pro, gemini-1.5-pro} \\
    \midrule
    \textbf{Open Source} & \textbf{LLAMA-2-13B, LLAMA-3-8B, CodeLLAMA-7B, CodeLLAMA-13B} \\
    \textbf{} & \textbf{Mistral-7B-v0.1, Mistral-7B-v0.2} \\
    \midrule
\end{tabular}
\end{table}


==> tables/llm_error.tex <==
\begin{table}[t]
  \caption{Comparison Between the number of seed nodes skipped due to different errors while using Llama and Gpt3.5 on Yago KG.}
  \label{tab:error}
  \begin{tabular}{ccc}
    \toprule
    \textbf{Error Type} & \textbf{Gpt-3.5} & \textbf{Llama} \\
    \midrule
    \textbf{Context Length} & 0 & 0 \\
    \textbf{Question Validation} & 0 & 10  \\
    \textbf{Triples Validation} & 0 & 67 \\
    \textbf{Dialogue Validation} & 0 & 1 \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/llm_quality.tex <==
\begin{table}[t]
  \caption{Comparison Between the quality of questions generated by Llama and Gpt-3.5 in a benchmark of $5$ dialogues on YAGO KG.}
  \label{tab:llm_quality}
  \begin{tabular}{ccc}
    \toprule
    \textbf{} & \textbf{Gpt-3.5} & \textbf{Llama} \\
    \midrule
    \textbf{Valid} & 21 & 11 \\
    \textbf{InValid} & 0 &  4 \\
    \textbf{Percentage(\%)} & 100 & 73.3 \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/llm_query.tex <==
\begin{table}[t]
  \caption{Percentage of correct SPARQL queries generated by the different LLMs for DBLP and YAGO KGs.}
  \label{tab:llm_query}
  \begin{tabular}{ccc}
    \toprule
    \textbf{LLM} & \textbf{YAGO} & \textbf{DBLP} \\
    \midrule
	 \textbf{LLAMA-7b} & 37.50 & - \\
	 \textbf{LLAMA-13b} & 50.00 & -  \\
	 \textbf{Mistral-7b-v0.1} & 63 & 64.44 \\
	 \textbf{CodeLLAMA-7b} & 64.60 & 57.14 \\
	  \textbf{CodeLLAMA-13b} & 90 & 77 \\
	  \textbf{GPT-3.5} & 100 & 89.90 \\
       \textbf{GPT-4} &  94 & 83.00 \\
  \bottomrule
\end{tabular}
\end{table}

==> tables/maestro_time.tex <==
\begin{table*}[t]
  \caption{End to end time performance comparison between {\sysName} and Maestro}
  \label{tab:maestro_time}
  \begin{tabular}{ccccc}
    \toprule
    \textbf{KG} & \textbf{Maestro} & \textbf{Number of types} & \textbf{Number of questions} & \textbf{{\sysName}} \\
    \midrule
    \textbf{DBpedia-R} & 13.5 hours & 33939 & 3408 & 7 mins \\
    \textbf{YAGO-O} & 7.1 hours & 2341 & 111002 & 21 mins \\
    \textbf{DBLP-O} & 10 mins & 145 & 1001 & 8 mins\\
    % \textbf{MAKG-O} & 12 mins  &  21&  68& \\
    % \textbf{MAKG-R} &  23 mins & 41 & 136& \\
    % \textbf{DBTune} & 40 mins & 30 & 627 &\\
  \bottomrule
 %\textbf{YAGO-O} & 427m51s & 2341 & 111002 & \\
 % \textbf{DBLP-O} & 10m13s & 145 & 1001 & \\
 % \textbf{MAKG-O} & 11m43s  &  21&  68& \\
 % \textbf{MAKG-R} &  23m4s & 41 & 136& \\
 % \textbf{DBTune} & 39m45s & 30 & 627 &\\
\end{tabular}
\end{table*}

==> tables/maestro_timev2.tex <==
\begin{table}[t]
\vspace*{-2ex}
  \caption{End to end time performance comparison between {\sysName} and Maestro in hours.}
  \label{tab:maestro_time}
  \vspace*{-3ex}
  \begin{tabular}{cccc}
    \toprule
    \textbf{KG (\# predicates)} & \textbf{Maestro} & \textbf{{\sysName}} \\
    \midrule
    \textbf{DBpedia (18211)} & 30.77 & 0.17 \\
    \textbf{YAGO (2809)} & 5.20  & 0.10 \\
    \textbf{MAG (130)} & 5.38 & 0.12\\
    \textbf{DBLP (131)} &  0.12  & 0.12\\
  \bottomrule
\end{tabular}
\vspace*{-1ex}
\end{table}

==> tables/open_llm.tex <==
\begin{table*}[t]
	 % \fontsize{5pt}{5pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|cccccc|cccccc}
		\toprule
		 & &  \multicolumn{6}{c|}{\textbf{YAGO}} & \multicolumn{6}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways} \textbf{Dialogue-E}\end{sideways} &\begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways}\\
		\midrule
	    \multirow{6}{*}{
            \textbf{Original}} 
            & \textbf{LLAMA-7b} & 11 & 62 & 165 &  0 & 500 & 1 & 20 & 17  &70& 0 & 500 & 0\\
            & \textbf{LLAMA-13b} & 3 & 4 & 30 & 0 & 500 & 1 & 5 & 8 &30& 0 & 500 & 0\\
            & \textbf{Mistral-7b-v0.1} & 8 & 6 &115&  0 & 152 & 20 & 66  & 36 &333 & 5 & 500 & 9\\
            & \textbf{CodeLLAMA-7b} & 30 & 83 & 189 & 32 & 306 & 20 & 220  & 8 & 258 & 5 & 500 & 5\\  
	    & \textbf{CodeLLAMA-13b} & 6 & 2 & 9 & 1 & 36 & 20& 25  & 0 & 28 & 0 & 68 & 20 \\
	    & \textbf{GPT-3.5} &  &  &   &  & &   &  &  &  & & &\\
	    \midrule
	    \multirow{6}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} & 19 & 11 & 73 & 0 & 91 & 0 & 6  & 3 &23& 0 & 42 & 0\\
            & \textbf{LLAMA-13b} & 46 & 54 &347&  5 & 374 & 12 & 88  & 91 &298& 3 & 320 & 2\\
            & \textbf{Mistral-7b-v0.1} & 14 & 7 &147&  1 & 171 & 4 & 34 & 15&192 & 1 & 216 & 10\\
            & \textbf{CodeLLAMA-7b} & 109 & 75 & 373 & 29 & 426 & 18 & 187  &45 & 297 & 8 & 327 & 15\\  
	    & \textbf{CodeLLAMA-13b} & 1 & 2 &10& 3 & 33 & 18 & 9 &3 &17 & 1 & 37 & 20\\
        & \textbf{GPT-3.5} &  &  &   &  & &   &  &  &  & & &\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/open_llm_june23.tex <==
\begin{table*}[t]
	 % \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results, Multi-LLM-1: (Question-triple and Dialogue Generation: LLLAMA-3-8b-inst + Answer Queries Generation: CodeLLAMA-13b), Multi-LLM-2: (Question-triple Generation: GPT-4, Dialogue Generation: LLAMA-3-8b-inst, + Answer Queries Generation: CodeLLAMA-13b)}
	\label{tab:openllm}
	\begin{tabular}{c|c|ccccccccc|ccccccccc}
		% \toprule
  \hline
		 & &  \multicolumn{9}{c|}{\textbf{YAGO}} & \multicolumn{9}{c}{\textbf{DBLP}} \\
   % \midrule
   \hline
		 \begin{sideways}\textbf{Approach}\end{sideways}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Success}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways}  & \begin{sideways}\textbf{Dialogue-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Success}\end{sideways} & 
        \begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways}  & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways}\\
		% \midrule
            \hline
	    \multirow{13}{*}{
            \rotatebox[origin=c]{90}{\textbf{Multi-stages (Ours)}}}
           % \textbf{\makecell{Multi-stages \\ (Ours)}}}
            & \textbf{GPT-4o} & 20 & 100 & 20 & 0 & 0 & 0 & 0 & 8 & 0.04(0.32) & 21 & 95 & 20 & 0 & 0 & 1& 0 & 6 & 0.05(0.38) \\
            & \textbf{GPT-4} & 21 & 95 & 20 & 0 & 0 & 1 & 0 & 13 & 0.05(0.71) & 20 & 100 & 20 & 0 & 0 & 0 & 0 & 11 & 0.05(0.78) \\
	    & \textbf{GPT-3.5} & 22 & 91 & 20 &  1 & 0 & 1 & 0 & 6 & 0.05(0.04) & 21 & 95 & 20 & 1 & 0 & 0 & 0 & 7 & 0.06(0.05) \\
            & \textbf{Gemini-1-pro} & 28 & 71 & 20 & 0 & 2 & 0 & 6 & 6 & 0.06(0.01) & 30 & 67 & 20 & 5 & 0 & 0 & 5 & 5.2 & 0.09(0.02)\\
            % & \textbf{\color{orange}{Gemini-pro-1.5-old}} & 179 & 20 & 0 & 0 & 157 & 34 & 0.25(0.48) & 146 & 20 & 0 & 0 & 123 & 50 & 0.30(0.59)\\
            & \textbf{Gemini-1.5-pro} & 92 & 22 & 20 & 0 & 1 & 0 & 71 & 20.5 & 0.18(0.35) & 49 & 41 & 20 & 0 & 0 & 1 & 28 & 14.5 & 0.12(0.24)\\
            \cline{2-20}
            & \textbf{{LLAMA-3-8b}} & 157 & 13 & 20 & 2 & 124 & 9 & 0 & 84 & 0.36 & 100 & 20 & 20 & 2 & 47 & 23 & 8 & 71 & 0.33 \\
            & \textbf{LLAMA-3-8b-inst} & 49 & 41 & 20 & 0 & 16 & 0 & 13 & 37 & 0.13 & 146 & 14 & 20 & 0 & 106 & 0 & 16 & 89 & 0.39 \\
            % & \textbf{LLAMA-2-7b} & 500 & 0 & 6 & 41 & &49 & 380 & 1.25 & 500 & 0 & 61 & 39 & & 167 & 353 & 1.45 \\
            & \textbf{LLAMA-2-13b} & 368 & 5 & 20 & 5 & 325 & 10 & 1 & 270 & 0.79 & 500 & 1 & 5 & 32 & 426 & 7 & 22 & 392 & 1.30 \\
            & \textbf{CodeLLAMA-7b} & 294 & 7 & 20 & 3 & 162 & 74 & 16 & 234 & 0.92 & 500 & 1 & 5 & 144 & 156 & 44 & 145 & 356 & 0.16 \\
	    & \textbf{CodeLLAMA-13b} & 24 & 83 & 20 & 0 & 0 & 4 & 0 & 31 & 0.08 & 32 & 63 & 20 & 3 & 5 & 2 & 1 & 37 & 0.01 \\
            & \textbf{Mistral-7b-v0.1} & 119 & 17 & 20 & 2 & 88 & 3 & 0 & 70 & 0.25 & 500 & 3 & 15 & 5 & 323 & 5 & 14 & 189 & 0.90 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 5 & 2 & 11 & 9 & 167 & 0.87 & 500 & 8 & 156 & 150 & 33 & 174 & 1.23 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 18 & 6 & 9 & 1 & 333 & 1.01 & 500 & 2 & 28 & 43 & 19 & 325 & 1.29 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 16 & 1 & 20 & 91 & 223 & 1.06 & 500 & 3 & 10 & 9 & 7 & 201 & 1.1 \\
            & \textbf{Multi-LLM-1} & 20 & 100 & 20 & 0 & 0 & 0 & 0 & 18 & 0.06 & 24 & 83 & 20 & 0 & 4 & 0 & 0 & 20 & 0.07\\
            & \textbf{Multi-LLM-2} & 22 & 91 & 20 & 0 & 0 & 0 & 2 & 18 & 0.06(0.28) & 28 
 & 71 & 20 & 2 & 4 & 0 & 2 & 23 & 0.10(0.82)\\
	    % \midrule
            \hline
	    \multirow{11}{*}{
            \rotatebox[origin=c]{90}{\textbf{One-stage}}}
            % \textbf{One-stage}}
            
             & \textbf{GPT-4o} & 52 & 38 & 20 & 11 & 0 & 5 & 15 & 9 & 0.03(0.32) & 242 & 8 & 20 & 52 & 0 & 8 & 144 & 59 & 0.15(1.30)\\
             % & \textbf{GPT-4o} & 52 & & 20 & 11 & 0 & 5 & 15 & 9 & 0.03(0.32) & 200 & & 14 & 45 & 0 & 4 & 123 & 47 & 0.12(1.05)\\
             & \textbf{GPT-4} & 50 & 40 & 20 & 5 & 1 & 1 & 23 & 17 & 0.04(0.73) & 96 & 21 & 20 & 5 & 1 & 2 & 66 & 46 & 0.09(1.86)\\
             & \textbf{GPT-3.5} & 407 & 5 & 19 & 2 & 0 & 8 & 242 & 53 & 0.36(0.32) & 240 & 8 & 20 & 25 & 0 & 5 & 119 & 50 & 0.25(0.24)\\
             % & \textbf{\color{red}{GPT-4o-dblp-1000}} & 52 & 20 & 11 & 0 & 5 & 15 & 9 & 0.03(0.32) & 76 & 20 & 4 & 0 & 4 & 44 & 25 & 0.02(0.19)\\
            % & \textbf{Gemini-1.5-pro} & 138 & 20 & 59 & 4 & 0 & 5 & 16 & 0.12(0.27) & 200 & 16 & 16 & 4 & 0 & 13 & 29 & 0.25(0.53)\\
            & \textbf{Gemini-1-pro} & 36 & 56 & 20 & 0 & 10 & 4 & 1 & 3 & 0.03(0.01) & 194 & 10 & 20 & 130 & 0 & 12 & 6 & 21 & 0.30(0.07)\\
            & \textbf{Gemini-1.5-pro} & 138 & 14 & 20 & 59 & 4 & 0 & 5 & 16 & 0.12(0.27) & 327 & 6 & 20 & 28 & 0 & 3 & 10 & 51.5 & 0.43(0.9)\\
            \cline{2-20}
            & \textbf{LLAMA-3-8b} & 1000 & 0 & 0 & 44 & 107 & 158 & 92 & 251 & 1 & 1000 & 0 & 2 & 170 & 23 & 55 & 452 & 286 & 1.23\\
            & \textbf{LLAMA-3-8b-inst} & 222 & 9 & 20 & 10 & 13 & 59 & 43 & 72 & 0.26 & 280 & 7 & 20 & 51 & 6 & 44 & 71 & 90 & 0.38\\
            % & \textbf{LLAMA-2-7b} & 1000 & 0 & 52 & 145 & 83 & 524 & 275 & 1.02 & 1000 & 0 & 183 & 33 & 16 & 632 & 286 & 1.20\\
            & \textbf{LLAMA-2-13b} & 1000 & 0 & 0 & 40 & 216 & 87 & 401 & 403 & 1 & 1000 & 0 & 0 & 53 & 39 & 18 & 827 & 479 & 1.22\\
            & \textbf{CodeLLAMA-7b} & 1000 & 0 & 0 & 72 & 87 & 196 & 344 & 314 & 1.07 & 1000 & 0 & 1 & 203 & 45 & 30 & 604 & 313 & 1.25\\
            & \textbf{CodeLLAMA-13b} & 1000 & 1 & 11 & 78 & 29 & 579 & 168 & 443 & 1.07 & 1000 & 1 & 5 & 188 & 11 & 91 & 677 & 459 & 1.26\\
            & \textbf{Mistral-7b-v0.1} & 1000 & 0 & 0 & 53 & 93 & 420 & 223 & 261 & 0.98 & 1000 & 0 & 1 & 208 & 34 & 118 & 528 & 257 & 1.20\\
            
            % & \textbf{LLAMA-3-8b} & 200 & 0 & 5 & 17 & 29 & 18 & 48 & 0.20 & 200 & 0 & 29 & 4 & 9 & 67 & 52 & 0.25\\
            % & \textbf{LLAMA-3-8b-inst} & 200 & 17 & 4 & 14 & 30 & 59 & 62 & 0.24 & 200 & 15 & 29 & 7 & 30 & 63 & 62 & 0.27\\
            % & \textbf{CodeLLAMA-13b} & 200 & 2 & 17 & 6 & 115 & 37 & 89 & 0.22 & 200 & 1 & 57 & 1 & 21 & 115 & 92 & 0.24\\
		% \bottomrule
            \hline
	\end{tabular}
\end{table*}
% Prompt Engineering
% LLM Capabilities
% instion-tuned models ? 



% & \textbf{\color{green}{GPT-4o}} & 38 & 20 & 0 & 0 & 4 & 14 & 24 & 0.04(0.37) & 66 & 20 & 5 & 0 &5 & 36 & 20 & 0.09(0.81) \\
            % & \textbf{GPT-4o}  & 52 & 20 & 0 & 0 & 5 & 27 & 13 & 0.03(0.30) & 73 & 20 & 1 & 1 &3 & 48 & 21 & 0.05(0.51)\\
            % & \textbf{GPT-4o}  & 52 & 20 & 0 & 0 & 5 & 27 & 13 & 0.03(0.30) & 73 & 20 & 1 & 1 &3 & 48 & 21 & 0.05(0.51)\\
            % & \textbf{GPT-4}  & 20 & 20 & 0 & 0 & & 0 & 21 & 0.03(0.53) & 22 & 20 & 1 & 0 & & 1 & 20 & 0.06(0.96) \\
            % & \textbf{GPT-3.5}  & 23 & 20 & 0 & 0 & & 0 & 5 & 0.04(0.04) & 26 & 20 & 2 & 1 & & 3 & 12 & 0.08(0.07) \\
            % & \textbf{Gemini-pro-1} & 39 & 20 & 0 & 0 & 13 & 6 & 0.11(0.02) & 56 & 20 & 6 & 0 & 0 & 8 & 0.13(0.02) \\
            % & \textbf{Gemini-pro-1.5} & 22 & 20 & 0 & 0 & 1 & 7 & 0.08(0.12) & 45 & 20 & 17 & 0 & 3 & 13.5 & 0.18(0.30)\\
            % & \textbf{LLAMA-3-8b} & 469 & 20 & 1 & 11 & 59 & 663 & 2.58 & 227 & 20 & 0 & 64 & 50 & 305 & 1.44 \\
            % & \textbf{LLAMA-3-8b-inst} & 104 & 20 & 0 & 0 & 18 & 199 & 0.63 & 500 & 15 & 0 & 4 & 115 & 895 & 3.4 \\
            % & \textbf{LLAMA-2-7b} & 487 & 0 & 0 & 45 & 158 & 910 & 2.85 & 500 & 0 & 89 & 16 & 277 & 752 & 2.80 \\
	    % & \textbf{\textcolor{orange}{LLAMA-2-13b}} & 462 & 16 & 0 & 14 & 119 & 909 & 2.39 & 456 & 7 & 10 & 41 & 106 & 910 & 2.94 \\
            % & \textbf{CodeLLAMA-7b} & 500 & 16 & 0 & 15 & 8 & 1048 & 3.35 & 500 & 2 & 37 & 14 & 86 & 1108 & 3.98 \\
            % & \textbf{CodeLLAMA-13b} & 26 & 20 & 0 & 0 & 0 & 83 & 0.18 & 42 & 20 & 2 & 0 & 2 & 122 & 0.30 \\
            % & \textbf{Mistral-7b-v0.1} & 213 & 20 & 0 & 2 & 5 & 243 & 0.10 & 500 & 12 & 6 & 72 & 35 & 429 & 2.66 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 0 & 1 & 1 & 404 & 155 & 1.6 & 500 & 2 & 80 & 13 & 318 & 151 & 1.84 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 17 & 0 & 20 & 13 & 582 & 2.5 & 500 & 3 & 11 & 119 & 27 & 449 & 2.66 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 13 & 1 & 11 & 265 & 439 & 1.89 & 500 & 2 & 4 & 14 & 252 & 250 & 1.97 \\
            % & \textbf{Multi-LLM-1} & 27 & 20 & 0 & 0 & 5 & 50 & 0.17 & 46 & 20 & 0 & 0 & 8 & 84 & 0.32\\
            % & \textbf{Multi-LLM-2} & 22 & 20 & 0 & 0 & 1 & 18 & 0.09 & 35 & 20 & 3 & 0 & 3 & 27 & 0.19\\

==> tables/open_llm_may12-simplified.tex <==
\begin{table*}[t]
	 % \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results, Multi-LLM-1: (Question-triple and Dialogue Generation: LLLAMA-3-8b-inst + Answer Queries Generation: CodeLLAMA-13b), Multi-LLM-2: (Question-triple Generation: GPT-4, Dialogue Generation: LLAMA-3-8b-inst, + Answer Queries Generation: CodeLLAMA-13b)}
	\label{tab:openllm}
	\begin{tabular}{c|c|ccccccc|ccccccc}
		\toprule
		 & &  \multicolumn{7}{c|}{\textbf{YAGO}} & \multicolumn{7}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways}  & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Complex}} 
            & \textbf{GPT-4o} & 20 & 20 & 0 & 0 & 0 & 8 & 0.04(0.32) & 21 & 20 & 0 & 0 & 0 & 6 & 0.05(0.38) \\
            & \textbf{GPT-4} & 21 & 20 & 0  & 0 & 0 & 13 & 0.05(0.71) & 20 & 20 & 0 & 0 & 0 & 11 & 0.05(0.78) \\
	    & \textbf{GPT-3.5} & 22 & 20 &  1 & 0 & 0 & 6 & 0.05(0.04) & 21 & 20 & 1 & 0 & 0 & 7 & 0.06(0.05) \\
            & \textbf{Gemini-pro-1} & 28 & 20 & 0 & 0 & 5 & 6 & 0.06(0.01) & 30 & 20 & 5 & 0 & 5 & 5.2 & 0.09(0.02)\\
            % & \textbf{\color{orange}{Gemini-pro-1.5-old}} & 179 & 20 & 0 & 0 & 157 & 34 & 0.25(0.48) & 146 & 20 & 0 & 0 & 123 & 50 & 0.30(0.59)\\
            & \textbf{Gemini-pro-1.5} & 92 & 20 & 0 & 0 & 71 & 20.5 & 0.18(0.35) & 49 & 20 & 0 & 0 & 28 & 14.5 & 0.12(0.24)\\
            & \textbf{{LLAMA-3-8b}} & 157 & 20 & 2 & 2 & 0 & 84 & 0.36 & 100 & 20 & 2 & 0 & 0 & 71 & 0.33 \\
            & \textbf{LLAMA-3-8b-inst} & 49 & 20 & 0 & 0 & 2 & 37 & 0.13 & 146 & 20 & 0 & 4 & 0 & 89 & 0.39 \\
            & \textbf{LLAMA-2-7b} & 500 & 0 & 6 & 41 & 49 & 380 & 1.25 & 500 & 0 & 61 & 39 & 167 & 353 & 1.45 \\
            & \textbf{LLAMA-2-13b} & 368 & 20 & 5 & 7 & 1 & 270 & 0.79 & 500 & 5 & 32 & 9 & 18 & 392 & 1.30 \\
            & \textbf{CodeLLAMA-7b} & 294 & 20 & 3 & 19 & 16 & 234 & 0.92 & 500 & 5 & 144 & 7 & 143 & 356 & 0.16 \\
	    & \textbf{CodeLLAMA-13b} & 24 & 20 & 0 & 0 & 0 & 31 & 0.083 & 32 & 20 & 3 & 1 & 1 & 37 & 0.011 \\
            & \textbf{Mistral-7b-v0.1} & 119 & 20 & 2 & 6 & 0 & 70 & 0.25 & 500 & 15 & 5 & 3 & 14 & 189 & 0.90 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 5 & 2 & 11 & 9 & 167 & 0.87 & 500 & 8 & 156 & 150 & 33 & 174 & 1.23 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 18 & 6 & 9 & 1 & 333 & 1.01 & 500 & 2 & 28 & 43 & 19 & 325 & 1.29 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 16 & 1 & 20 & 91 & 223 & 1.06 & 500 & 3 & 10 & 9 & 7 & 201 & 1.1 \\
            & \textbf{Multi-LLM-1} & 20 & 20 & 0 & 0 & 0 & 18 & 0.06 & 24 & 20 & 0 & 0 & 0 & 20 & 0.07\\
            & \textbf{Multi-LLM-2} & 22 & 20 & 0 & 0 & 0 & 18 & 0.06 & 28 & 20 & 2 & 0 & 2 & 23 & 0.10\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{GPT-4o} & 21 & 20 & 0 & 0 & 0 & 8 & 0.08(0.50) & 22 & 20 & 0 & 0 & 1 & 7 & 0.10(0.61)\\
            & \textbf{GPT-4}  & 22 & 20 & 0  & 0 &2 & 14 & 0.07(0.97) & 20 & 20 & 0 & 0 & 0 & 11 & 0.09(1.13) \\
            & \textbf{GPT-3.5}  & 24 & 20 & 0 & 1 & 1 & 7 & 0.08(0.06) & 24 & 20 & 0 & 0 & 2 & 7 & 0.10(0.07) \\
            & \textbf{Gemini-pro-1} & 39 & 20 & 0 & 0 & 13 & 6 & 0.11(0.02) & 56 & 20 & 6 & 0 & 0 & 8 & 0.13(0.02) \\
            & \textbf{Gemini-pro-1.5} & 22 & 20 & 0 & 0 & 1 & 7 & 0.08(0.12) & 45 & 20 & 17 & 0 & 3 & 13.5 & 0.18(0.30)\\
            & \textbf{LLAMA-3-8b} & 469 & 20 & 1 & 11 & 59 & 663 & 2.58 & 227 & 20 & 0 & 64 & 50 & 305 & 1.44 \\
            & \textbf{LLAMA-3-8b-inst} & 104 & 20 & 0 & 0 & 18 & 199 & 0.63 & 500 & 15 & 0 & 4 & 115 & 895 & 3.4 \\
            & \textbf{LLAMA-2-7b} & 487 & 0 & 0 & 45 & 158 & 910 & 2.85 & 500 & 0 & 89 & 16 & 277 & 752 & 2.80 \\
	    & \textbf{\textcolor{orange}{LLAMA-2-13b}} & 462 & 16 & 0 & 14 & 119 & 909 & 2.39 & 456 & 7 & 10 & 41 & 106 & 910 & 2.94 \\
            & \textbf{CodeLLAMA-7b} & 500 & 16 & 0 & 15 & 8 & 1048 & 3.35 & 500 & 2 & 37 & 14 & 86 & 1108 & 3.98 \\
            & \textbf{CodeLLAMA-13b} & 26 & 20 & 0 & 0 & 0 & 83 & 0.18 & 42 & 20 & 2 & 0 & 2 & 122 & 0.30 \\
            & \textbf{Mistral-7b-v0.1} & 213 & 20 & 0 & 2 & 5 & 243 & 0.10 & 500 & 12 & 6 & 72 & 35 & 429 & 2.66 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 0 & 1 & 1 & 404 & 155 & 1.6 & 500 & 2 & 80 & 13 & 318 & 151 & 1.84 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 17 & 0 & 20 & 13 & 582 & 2.5 & 500 & 3 & 11 & 119 & 27 & 449 & 2.66 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 13 & 1 & 11 & 265 & 439 & 1.89 & 500 & 2 & 4 & 14 & 252 & 250 & 1.97 \\
            & \textbf{Multi-LLM-1} & 27 & 20 & 0 & 0 & 5 & 50 & 0.17 & 46 & 20 & 0 & 0 & 8 & 84 & 0.32\\
            & \textbf{Multi-LLM-2} & 22 & 20 & 0 & 0 & 1 & 18 & 0.09 & 35 & 20 & 3 & 0 & 3 & 27 & 0.19\\
	    
		\bottomrule
	\end{tabular}
\end{table*}
% Prompt Engineering
% LLM Capabilities
% instion-tuned models ? 

==> tables/open_llm_may12.tex <==
\begin{table*}[t]
	 % \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results, Multi-LLM-1: (Question-triple and Dialogue Generation: LLLAMA-3-8b-inst + Answer Queries Generation: CodeLLAMA-13b), Multi-LLM-2: (Question-triple Generation: GPT-4, Dialogue Generation: LLAMA-3-8b-inst, + Answer Queries Generation: CodeLLAMA-13b)}
	\label{tab:openllm}
	\begin{tabular}{c|c|cccccccc|cccccccc}
		\toprule
		 & &  \multicolumn{8}{c|}{\textbf{YAGO}} & \multicolumn{8}{c}{\textbf{DBLP}} \\
   \midrule
		 \begin{sideways}\textbf{Approach}\end{sideways}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways}  & \begin{sideways}\textbf{Dialogue-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways}  & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens M (\$)}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
           \textbf{\makecell{Multi-stages \\ (Ours)}}}
            & \textbf{GPT-4o} & 20 & 20 & 0 & 0 & 0 & 0 & 8 & 0.04(0.32) & 21 & 20 & 0 & 0 & 1& 0 & 6 & 0.05(0.38) \\
            & \textbf{GPT-4} & 21 & 20 & 0  & 0 & & 0 & 13 & 0.05(0.71) & 20 & 20 & 0 & 0 & &0 & 11 & 0.05(0.78) \\
	    & \textbf{GPT-3.5} & 22 & 20 &  1 & 0 & & 0 & 6 & 0.05(0.04) & 21 & 20 & 1 & 0 & &0 & 7 & 0.06(0.05) \\
            & \textbf{Gemini-1-pro} & 28 & 20 & 0 & 0 & &5 & 6 & 0.06(0.01) & 30 & 20 & 5 & 0 & &5 & 5.2 & 0.09(0.02)\\
            % & \textbf{\color{orange}{Gemini-pro-1.5-old}} & 179 & 20 & 0 & 0 & 157 & 34 & 0.25(0.48) & 146 & 20 & 0 & 0 & 123 & 50 & 0.30(0.59)\\
            & \textbf{Gemini-1.5-pro} & 92 & 20 & 0 & 1 & 0 & 71 & 20.5 & 0.18(0.35) & 49 & 20 & 0 & 0 & 1 & 28 & 14.5 & 0.12(0.24)\\
            & \textbf{{LLAMA-3-8b}} & 157 & 20 & 2 & 2 & & 0 & 84 & 0.36 & 100 & 20 & 2 & 0 & &0 & 71 & 0.33 \\
            & \textbf{LLAMA-3-8b-inst} & 49 & 20 & 0 & 0 & & 2 & 37 & 0.13 & 146 & 20 & 0 & 4 & & 0 & 89 & 0.39 \\
            % & \textbf{LLAMA-2-7b} & 500 & 0 & 6 & 41 & &49 & 380 & 1.25 & 500 & 0 & 61 & 39 & & 167 & 353 & 1.45 \\
            & \textbf{LLAMA-2-13b} & 368 & 20 & 5 & 7 & & 1 & 270 & 0.79 & 500 & 5 & 32 & 9 & & 18 & 392 & 1.30 \\
            & \textbf{CodeLLAMA-7b} & 294 & 20 & 3 & 19 & & 16 & 234 & 0.92 & 500 & 5 & 144 & 7 & & 143 & 356 & 0.16 \\
	    & \textbf{CodeLLAMA-13b} & 24 & 20 & 0 & 0 & & 0 & 31 & 0.083 & 32 & 20 & 3 & 1 & & 1  & 37 & 0.011 \\
            & \textbf{Mistral-7b-v0.1} & 119 & 20 & 2 & 6 & & 0 & 70 & 0.25 & 500 & 15 & 5 & 3 & & 14 & 189 & 0.90 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 5 & 2 & 11 & 9 & 167 & 0.87 & 500 & 8 & 156 & 150 & 33 & 174 & 1.23 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 18 & 6 & 9 & 1 & 333 & 1.01 & 500 & 2 & 28 & 43 & 19 & 325 & 1.29 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 16 & 1 & 20 & 91 & 223 & 1.06 & 500 & 3 & 10 & 9 & 7 & 201 & 1.1 \\
            & \textbf{Multi-LLM-1} & 20 & 20 & 0 & 0 & & 0 & 18 & 0.06 & 24 & 20 & 0 & 0 & & 0 & 20 & 0.07\\
            & \textbf{Multi-LLM-2} & 22 & 20 & 0 & 0 & & 0 & 18 & 0.06 & 28 & 20 & 2 & 0 & & 2 & 23 & 0.10\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{One-stage}}
            
             & \textbf{GPT-4o} & 52 & 20 & 11 & 0 & 5 & 15 & 9 & 0.03(0.32) & 200 & 14 & 45 & 0 & 4 & 123 & 47 & 0.12(1.05)\\
             & \textbf{GPT-4} & 50 & 20 & 5 & 1 & 1 & 23 & 17 & 0.04(0.73) & 96 & 20 & 5 & 1 & 2 & 66 & 46 & 0.09(1.86)\\
             & \textbf{GPT-3.5} & 407 & 19 & 2 & 0 & 8 & 242 & 53 & 0.36(0.32) & 240 & 20 & 25 & 0 & 5 & 119 & 50 & 0.25(0.24)\\
             % & \textbf{\color{red}{GPT-4o-dblp-1000}} & 52 & 20 & 11 & 0 & 5 & 15 & 9 & 0.03(0.32) & 76 & 20 & 4 & 0 & 4 & 44 & 25 & 0.02(0.19)\\
            % & \textbf{Gemini-1.5-pro} & 138 & 20 & 59 & 4 & 0 & 5 & 16 & 0.12(0.27) & 200 & 16 & 16 & 4 & 0 & 13 & 29 & 0.25(0.53)\\
            & \textbf{Gemini-1-pro} & 36 & 20 & 0 & 10 & 4 & 1 & 3 & 0.03(0.01) & 194 & 20 & 130 & 0 & 12 & 6 & 21 & 0.30(0.07)\\
            & \textbf{Gemini-1.5-pro} & 138 & 20 & 59 & 4 & 0 & 5 & 16 & 0.12(0.27) & 327 & 20 & 28 & 0 & 3 & 10 & 51.5 & 0.43(0.9)\\
            & \textbf{LLAMA-3-8b} & 1000 & 0 & 44 & 107 & 158 & 92 & 251 & 1 & 1000 & 2 & 170 & 23 & 55 & 452 & 286 & 1.23\\
            & \textbf{LLAMA-3-8b-inst} & 222 & 20 & 10 & 13 & 59 & 43 & 72 & 0.26 & 280 & 20 & 51 & 6 & 44 & 71 & 90 & 0.38\\
            % & \textbf{LLAMA-2-7b} & 1000 & 0 & 52 & 145 & 83 & 524 & 275 & 1.02 & 1000 & 0 & 183 & 33 & 16 & 632 & 286 & 1.20\\
            & \textbf{LLAMA-2-13b} & 1000 & 0 & 40 & 216 & 87 & 401 & 403 & 1 & 1000 & 0 & 53 & 39 & 18 & 827 & 479 & 1.22\\
            & \textbf{CodeLLAMA-7b} & 1000 & 0 & 72 & 87 & 196 & 344 & 314 & 1.07 & 1000 & 1 & 203 & 45 & 30 & 604 & 313 & 1.25\\
            & \textbf{CodeLLAMA-13b} & 1000 & 11 & 78 & 29 & 579 & 168 & 443 & 1.07 & 1000 & 5 & 188 & 11 & 91 & 677 & 459 & 1.26\\
            & \textbf{Mistral-7b-v0.1} & 1000 & 0 & 53 & 93 & 420 & 223 & 261 & 0.98 & 1000 & 1 & 208 & 34 & 118 & 528 & 257 & 1.20\\
            
            % & \textbf{LLAMA-3-8b} & 200 & 0 & 5 & 17 & 29 & 18 & 48 & 0.20 & 200 & 0 & 29 & 4 & 9 & 67 & 52 & 0.25\\
            % & \textbf{LLAMA-3-8b-inst} & 200 & 17 & 4 & 14 & 30 & 59 & 62 & 0.24 & 200 & 15 & 29 & 7 & 30 & 63 & 62 & 0.27\\
            % & \textbf{CodeLLAMA-13b} & 200 & 2 & 17 & 6 & 115 & 37 & 89 & 0.22 & 200 & 1 & 57 & 1 & 21 & 115 & 92 & 0.24\\
		\bottomrule
	\end{tabular}
\end{table*}
% Prompt Engineering
% LLM Capabilities
% instion-tuned models ? 



% & \textbf{\color{green}{GPT-4o}} & 38 & 20 & 0 & 0 & 4 & 14 & 24 & 0.04(0.37) & 66 & 20 & 5 & 0 &5 & 36 & 20 & 0.09(0.81) \\
            % & \textbf{GPT-4o}  & 52 & 20 & 0 & 0 & 5 & 27 & 13 & 0.03(0.30) & 73 & 20 & 1 & 1 &3 & 48 & 21 & 0.05(0.51)\\
            % & \textbf{GPT-4o}  & 52 & 20 & 0 & 0 & 5 & 27 & 13 & 0.03(0.30) & 73 & 20 & 1 & 1 &3 & 48 & 21 & 0.05(0.51)\\
            % & \textbf{GPT-4}  & 20 & 20 & 0 & 0 & & 0 & 21 & 0.03(0.53) & 22 & 20 & 1 & 0 & & 1 & 20 & 0.06(0.96) \\
            % & \textbf{GPT-3.5}  & 23 & 20 & 0 & 0 & & 0 & 5 & 0.04(0.04) & 26 & 20 & 2 & 1 & & 3 & 12 & 0.08(0.07) \\
            % & \textbf{Gemini-pro-1} & 39 & 20 & 0 & 0 & 13 & 6 & 0.11(0.02) & 56 & 20 & 6 & 0 & 0 & 8 & 0.13(0.02) \\
            % & \textbf{Gemini-pro-1.5} & 22 & 20 & 0 & 0 & 1 & 7 & 0.08(0.12) & 45 & 20 & 17 & 0 & 3 & 13.5 & 0.18(0.30)\\
            % & \textbf{LLAMA-3-8b} & 469 & 20 & 1 & 11 & 59 & 663 & 2.58 & 227 & 20 & 0 & 64 & 50 & 305 & 1.44 \\
            % & \textbf{LLAMA-3-8b-inst} & 104 & 20 & 0 & 0 & 18 & 199 & 0.63 & 500 & 15 & 0 & 4 & 115 & 895 & 3.4 \\
            % & \textbf{LLAMA-2-7b} & 487 & 0 & 0 & 45 & 158 & 910 & 2.85 & 500 & 0 & 89 & 16 & 277 & 752 & 2.80 \\
	    % & \textbf{\textcolor{orange}{LLAMA-2-13b}} & 462 & 16 & 0 & 14 & 119 & 909 & 2.39 & 456 & 7 & 10 & 41 & 106 & 910 & 2.94 \\
            % & \textbf{CodeLLAMA-7b} & 500 & 16 & 0 & 15 & 8 & 1048 & 3.35 & 500 & 2 & 37 & 14 & 86 & 1108 & 3.98 \\
            % & \textbf{CodeLLAMA-13b} & 26 & 20 & 0 & 0 & 0 & 83 & 0.18 & 42 & 20 & 2 & 0 & 2 & 122 & 0.30 \\
            % & \textbf{Mistral-7b-v0.1} & 213 & 20 & 0 & 2 & 5 & 243 & 0.10 & 500 & 12 & 6 & 72 & 35 & 429 & 2.66 \\
            % & \textbf{Mistral-7b-v0.1-inst} & 500 & 0 & 1 & 1 & 404 & 155 & 1.6 & 500 & 2 & 80 & 13 & 318 & 151 & 1.84 \\
            % & \textbf{Mistral-7b-v0.2} & 500 & 17 & 0 & 20 & 13 & 582 & 2.5 & 500 & 3 & 11 & 119 & 27 & 449 & 2.66 \\
            % & \textbf{Mistral-7b-v0.2-inst} & 500 & 13 & 1 & 11 & 265 & 439 & 1.89 & 500 & 2 & 4 & 14 & 252 & 250 & 1.97 \\
            % & \textbf{Multi-LLM-1} & 27 & 20 & 0 & 0 & 5 & 50 & 0.17 & 46 & 20 & 0 & 0 & 8 & 84 & 0.32\\
            % & \textbf{Multi-LLM-2} & 22 & 20 & 0 & 0 & 1 & 18 & 0.09 & 35 & 20 & 3 & 0 & 3 & 27 & 0.19\\

==> tables/open_llm_prompt_updated.tex <==
\begin{table*}[t]
	 % \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|ccccccc|ccccccc}
		\toprule
		 & &  \multicolumn{7}{c|}{\textbf{YAGO}} & \multicolumn{7}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways}  & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Complex}} 
            & \textbf{LLAMA-7b} & 500 & 3 & 6 & 135 & 57 & 367 & 1.27M & 500 & 0 & 97 & 81 & 172 & 349 & 1.46M \\
            & \textbf{LLAMA-13b} & 213 & 20 & 0 & 8 & 0 & 151 & 475K & 500 & 5 & 48 & 30 & 23 & 378 & 1.37M\\
            & \textbf{Mistral-7b-v0.1} & 191 & 20 & 1 & 4 & 0 & 119 & 396K & 500 & 19 & 12 & 15 & 12 & 266 & 1.26M\\
            & \textbf{CodeLLAMA-7b} & 143 & 20 & 3 & 18 & 11 & 
123 & 481K &500 & 8 & 212 & 42 & 188 & 755 & 1.55M\\
	    & \textbf{CodeLLAMA-13b} & 34 & 20 & 1 & 10 & 0 & 44 & 110K & 47 & 20 & 9 & 9 & 3 & 58 & 161K\\
	    & \textbf{GPT-3.5} & 20 & 20 &  0 & 0 &0 & 5 & 42K & 22 & 20 & 0 & 0 & 1 & 6 & 56K\\
            & \textbf{GPT-4} & 24 & 20 & 0&1&0 & 13 &47K & 21 & 20 & 0 & 0 & 0& 13& 48K\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} & 500 & 0 & 1 & 53 & 163 & 843 & 2.74M & 500 & 0 & 93 & 13 & 300 & 736 & 2.89M\\
	    & \textbf{LLAMA-13b} & 495 & 15 & 0 & 38 & 138 & 932 & 2.62M & 500 & 2 & 8 & 197 & 113 & 893 & 3.05M\\
            & \textbf{Mistral-7b-v0.1} & 246 & 20 & 1 & 14 & 7 & 304 & 1.2M & 500 & 3 & 4 & 255 & 31 & 395 & 2.44M\\
            & \textbf{CodeLLAMA-7b} & 402 & 20 & 3 & 45 & 9 & 701 & 2.65M & 373 & 20 & 27 & 73 & 61 & 729 & 3.01M\\
            & \textbf{CodeLLAMA-13b} & 24 & 20 & 0 & 1 & 0 & 60 & 152K & 37 & 20 & 2 & 0 & 4 & 92 & 266K\\
            & \textbf{GPT-3.5} & 30 & 20 & 0 & 2 & 2 & 8 & 102K& 22 & 20& 0 & 1&0&8&94K\\
            & \textbf{GPT-4} & 21&20 & 0 & 0 & 1& 12& 72K & 20&20&0&0&0&13&89K\\
	    
		\bottomrule
	\end{tabular}
\end{table*}
% Prompt Engineering
% LLM Capabilities
% Instruction-tuned models ? 

==> tables/open_llm_v2.tex <==
\begin{table*}[t]
	 % \fontsize{5pt}{5pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|cccccccccc|cccccccccc}
		\toprule
		 & &  \multicolumn{10}{c|}{\textbf{YAGO}} & \multicolumn{10}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways}& \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways} \textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Original}} 
            & \textbf{LLAMA-7b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{LLAMA-13b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{Mistral-7b-v0.1} & 179 & 20 & 5 & 0 & 152 & 2 & 0 & 0 & 129 & &  &  & &&&&&&fix it\\
            & \textbf{CodeLLAMA-7b} & 169 & 20 & 13 & 17 & 71 & 41 & 0 & 7 & 158 & & &  & &&&&&&fix it\\
	    & \textbf{CodeLLAMA-13b} &  30 & 20 & 2 & 3 & 1 & 2 & 0  & 2 & 40 && 45 &  20 & 4 & 0 & 17 & 2 & 0 & 2 & 58\\
	    & \textbf{GPT-3.5} & 30 & 20 & 7  & 0 & 3 & 0 & 0 & 0 & 4  & 38& 23 & 20 &3&0&0&0&0&0& 4&47\\
            & \textbf{GPT-4} & 24  & 20 & 0  & 1 & 3 & 0  &0  &0  & 11 &39 &22 & 20& 0 &1&1& 0& 0& 0&12&44\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{LLAMA-13b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{Mistral-7b-v0.1} &  &  &  &   &  &  &  &   & running & & &  &&&& && &running \\
            & \textbf{CodeLLAMA-7b} & 307 & 20 & 6 & 38 & 93 & 32 & 0 & 118 & 537 &&  &   & \\
	    & \textbf{CodeLLAMA-13b} & 30 & 20 & 0 & 2 & 2 & 2 & 0 & 4 & 81 & &38 & 20 & 1 & 4 & 6 & 0 & 0 & 7 & 99\\
            & \textbf{GPT-3.5} & 21  & 20 & 1 & 0 & 0 & 0 & 0 & 0&4 &74 &26 & 20 & 3 & 0&0&0 &0&3& 5& 97\\
            & \textbf{GPT-4} & 21 & 20 & 0 & 0 & 0&  0 & 0 & 1 & 13 & 73 & 20 & 20 &0&0&0 &0&0 &0&11&93\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/open_llm_v3.tex <==
\begin{table*}[t]
	 % \fontsize{5pt}{5pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|cccccccccc|cccccccccc}
		\toprule
		 & &  \multicolumn{10}{c|}{\textbf{YAGO}} & \multicolumn{10}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways}& \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways} \textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Original}} 
            & \textbf{LLAMA-7b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{LLAMA-13b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{Mistral-7b-v0.1} & & &  &  & &&&&&&\\
            & \textbf{CodeLLAMA-7b} && & &  & &&&&&&\\
	    & \textbf{CodeLLAMA-13b} & &&  &  & &&&&&& \\
	    & \textbf{GPT-3.5} & 30 & 20 & 7  & 0 & 3 & 0 & 0 & 0 & 4  & 38& 23 & 20 &3&0&0&0&0&0& 4&47\\
            & \textbf{GPT-4} & 24  & 20 & 0  & 1 & 3 & 0  &0  &0  & 11 &39 &22 & 20& 0 &1&1& 0& 0& 0&12&44\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} &  &  &  &   &  &  &  &   &&  &  & \\
            & \textbf{\color{red}LLAMA-13b} & 501 & 10 & 1 & 40  & 172 & 5 & 0 & 273  & 898m & 2.529M & 501 & 2 & 25 & 87 & 167 & 2 & 0 & 218 & 892m & 3.092M\\
            & \textbf{Mistral-7b-v0.1} &  &  &  &   &  &  &  &   &  & & &  &&&& && & \\
            & \textbf{CodeLLAMA-7b} & &&  & &  & &&&&&&  & \\
	    & \textbf{CodeLLAMA-13b} &&  & &&&&&&&&\\
            & \textbf{GPT-3.5} & 21  & 20 & 1 & 0 & 0 & 0 & 0 & 0&4 &74 &26 & 20 & 3 & 0&0&0 &0&3& 5& 97\\
            & \textbf{GPT-4} & 21 & 20 & 0 & 0 & 0&  0 & 0 & 1 & 13 & 73 & 20 & 20 &0&0&0 &0&0 &0&11&93\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/open_llm_v4.tex <==
\begin{table*}[t]
	 \fontsize{7pt}{7pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|cccccccccc|cccccccccc}
		\toprule
		 & &  \multicolumn{10}{c|}{\textbf{YAGO}} & \multicolumn{10}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways}& \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways} \textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Context-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Original}} 
            & \textbf{LLAMA-7b} & 500 & 1 & 5 & 77 & 360 & 2 & 0 & 55 & 453 & 1.26M & 500 & 0 & 45 & 56 & 228 & 0 & 0 & 171 & 404 & 1.44M\\
            & \textbf{LLAMA-13b} & 283 & 20 & 11 & 3 & 237 & 11 & 0 & 1 & 238 & 619K & 500 & 7 & 40 & 21 & 366 & 13 & 0 & 53 & 495 & 1.3M\\
            & \textbf{Mistral-7b-v0.1} & 160 & 20 & 2 & 3 & 131 & 3 & 0 & 1 & 95 & 347K & 500 & 19 & 14 & 27 & 403 & 9 & 0 & 28 & 285 & 1.33M\\
            & \textbf{CodeLLAMA-7b} &166 & 20 & 19 & 22 & 65 & 28 & 0 & 12 & 136 & 503K & 500 & 5 & 269 & 21 & 34 & 6 & 0 & 165 & 365 & 1.54M\\
	    & \textbf{CodeLLAMA-13b} &58 & 20 & 5 & 27 & 1 & 5 & 0 & 0 & 73 & 184K & 78 & 20 & 20 & 12 & 14 & 3 & 0 & 9 & 95 & 265K\\
	    & \textbf{GPT-3.5} & 24 & 20 & 2 & 1 & 0 & 0 & 0 & 1 &  7 & 49K & 25 & 20 &3 &1&0&0&0&1& 9 & 69K\\
            & \textbf{GPT-4} & 21 & 20 & 0 & 1 & 0 & 0 & 0 & 0 & 14 & 45K& 21 & 20 &0&1&0 & 0&0&0 &16&52K\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} & 500 & 0 & 16 & 55 & 197 & 1 & 0 & 231 & 816 & 2.8M & 500 & 0 & 44 & 16 & 56 & 0 & 0 & 384 & 603 & 2.4M\\
	    & \textbf{LLAMA-13b} & 500 & 14 & 3 & 38 & 237 & 13 & 0 & 195 & 940 & 2.68M & 500 & 2 & 15 & 159 & 162 & 2 & 0 & 160 & 907 & 3.12M\\
            & \textbf{Mistral-7b-v0.1} &  264 & 20 & 11 & 15 & 209 & 5 & 0 & 4 & 315 & 1.39M & 500 & 11 & 8 & 94 & 362 & 5 & 0 & 20 & 794 & 2.85M \\
            & \textbf{CodeLLAMA-7b} & 248 & 20 & 8 & 40 & 141 & 33 & 0 & 6 & 485 & 1.7M & 500 & 9 & 182 & 62 & 173 & 16 & 0 & 58 & 743 & 2.8M\\
            & \textbf{CodeLLAMA-13b} & 28 & 20 & 1 & 1 & 0 & 5 & 0 & 1 & 80 & 185K & 32 & 20 & 1 & 0 & 11 & 0 & 0 & 0 & 92 & 248K\\
            & \textbf{GPT-3.5} & 24 & 20 & 0 & 1 & 1 &0 & 0 & 2& 8& 88K& 37 & 20 & 3 & 5 & 6& 0&0&3& 12 & 165K\\
            & \textbf{GPT-4} & 25 & 20 & 0 & 0 & 1& 0  & 0 & 4 & 15 & 87K & 20 & 20 &0&0&0 &0& 0&0&14&93K\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/open_llm_v5.tex <==
\begin{table*}[t]
	 \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|ccccccccc|ccccccccc}
		\toprule
		 & &  \multicolumn{9}{c|}{\textbf{YAGO}} & \multicolumn{9}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways}\textbf{Dialogue-E}\end{sideways} & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} & \begin{sideways}\textbf{SPARQL-E}\end{sideways} & \begin{sideways} \textbf{Dialogue-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Original}} 
            & \textbf{LLAMA-7b} & 500 & 1 & 5 & 77 & 360 & 2 & 55 & 453 & 1.26M & 500 & 0 & 45 & 56 & 228 & 0 & 171 & 404 & 1.44M\\
            & \textbf{LLAMA-13b} & 283 & 20 & 11 & 3 & 237 & 11 & 1 & 238 & 619K & 500 & 7 & 40 & 21 & 366 & 13 & 53 & 495 & 1.3M\\
            & \textbf{Mistral-7b-v0.1} & 160 & 20 & 2 & 3 & 131 & 3 & 1 & 95 & 347K & 500 & 19 & 14 & 27 & 403 & 9 & 28 & 285 & 1.33M\\
            & \textbf{CodeLLAMA-7b} &166 & 20 & 19 & 22 & 65 & 28  & 12 & 136 & 503K & 500 & 5 & 269 & 21 & 34 & 6 & 165 & 365 & 1.54M\\
	    & \textbf{CodeLLAMA-13b} &58 & 20 & 5 & 27 & 1 & 5 & 0 & 73 & 184K & 78 & 20 & 20 & 12 & 14 & 3 & 9 & 95 & 265K\\
	    & \textbf{GPT-3.5} & 24 & 20 & 2 & 1 & 0 & 0 & 1 &  7 & 49K & 25 & 20 &3 &1&0&0&1& 9 & 69K\\
            & \textbf{GPT-4} & 21 & 20 & 0 & 1 & 0 & 0 & 0 & 14 & 45K& 21 & 20 &0&1&0 & 0&0 &16&52K\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} & 500 & 0 & 16 & 55 & 197 & 1 & 231 & 816 & 2.8M & 500 & 0 & 44 & 16 & 56 & 0 & 384 & 603 & 2.4M\\
	    & \textbf{LLAMA-13b} & 500 & 14 & 3 & 38 & 237 & 13 & 195 & 940 & 2.68M & 500 & 2 & 15 & 159 & 162 & 2 & 160 & 907 & 3.12M\\
            & \textbf{Mistral-7b-v0.1} &  264 & 20 & 11 & 15 & 209 & 5 & 4 & 315 & 1.39M & 500 & 11 & 8 & 94 & 362 & 5 & 20 & 794 & 2.85M \\
            & \textbf{CodeLLAMA-7b} & 248 & 20 & 8 & 40 & 141 & 33 & 6 & 485 & 1.7M & 500 & 9 & 182 & 62 & 173 & 16  & 58 & 743 & 2.8M\\
            & \textbf{CodeLLAMA-13b} & 28 & 20 & 1 & 1 & 0 & 5 &  1 & 80 & 185K & 32 & 20 & 1 & 0 & 11 & 0 &  0 & 92 & 248K\\
            & \textbf{GPT-3.5} & 24 & 20 & 0 & 1 & 1 &0 & 2& 8& 88K& 37 & 20 & 3 & 5 & 6& 0&3& 12 & 165K\\
            & \textbf{GPT-4} & 25 & 20 & 0 & 0 & 1& 0  & 4 & 15 & 87K & 20 & 20 &0&0&0 &0&0&14&93K\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/open_llm_v6.tex <==
\begin{table*}[t]
	 % \fontsize{8pt}{8pt}\selectfont
	\caption{Evaluating the performance of openLLMs on the simplified and original pipeline for two KGs, DBLP and YAGO. E represents error and S represents successful results}
	\label{tab:openllm}
	\begin{tabular}{c|c|ccccccc|ccccccc}
		\toprule
		 & &  \multicolumn{7}{c|}{\textbf{YAGO}} & \multicolumn{7}{c}{\textbf{DBLP}} \\
   \midrule
		\textbf{Pipeline Type}& \textbf{LLM} & 
        
        \begin{sideways}\textbf{Num\_seeds}\end{sideways} & \begin{sideways}\textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways} &  \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways} &
        
        \begin{sideways} \textbf{Num\_seeds}\end{sideways} &\begin{sideways} \textbf{Dialogue-S}\end{sideways} & \begin{sideways}\textbf{Question-E}\end{sideways} & \begin{sideways}\textbf{Triples-E}\end{sideways}  & \begin{sideways}\textbf{Parsing-E}\end{sideways} & \begin{sideways}\textbf{Time(mins)}\end{sideways} & \begin{sideways}\textbf{\# Tokens}\end{sideways}\\
		\midrule
	    \multirow{7}{*}{
            \textbf{Complex}} 
            & \textbf{LLAMA-7b} & 500 & 1 & 5 & 77 & 55 & 453 & 1.26M & 500 & 0 & 45 & 56 & 171 & 404 & 1.44M\\
            & \textbf{LLAMA-13b} & 283 & 20 & 11 & 3 &  1 & 238 & 619K & 500 & 7 & 40 & 21 & 53 & 495 & 1.3M\\
            & \textbf{Mistral-7b-v0.1} & 160 & 20 & 2 & 3 & 1 & 95 & 347K & 500 & 19 & 14 & 27 & 28 & 285 & 1.33M\\
            & \textbf{CodeLLAMA-7b} &166 & 20 & 19 & 22 & 12 & 136 & 503K & 500 & 5 & 269 & 21 & 165 & 365 & 1.54M\\
	    & \textbf{CodeLLAMA-13b} &58 & 20 & 5 & 27 &  0 & 73 & 184K & 78 & 20 & 20 & 12 & 9 & 95 & 265K\\
	    & \textbf{GPT-3.5} & 24 & 20 & 2 & 1 & 1 &  7 & 49K & 25 & 20 &3 &1&1& 9 & 69K\\
            & \textbf{GPT-4} & 21 & 20 & 0 & 1 & 0 & 14 & 45K& 21 & 20 &0&1&0 &16&52K\\
	    \midrule
	    \multirow{7}{*}{
            \textbf{Simplified}} 
            & \textbf{LLAMA-7b} & 500 & 0 & 16 & 55 & 231 & 816 & 2.8M & 500 & 0 & 44 & 16 & 384 & 603 & 2.4M\\
	    & \textbf{LLAMA-13b} & 500 & 14 & 3 & 38 & 195 & 940 & 2.68M & 500 & 2 & 15 & 159 & 160 & 907 & 3.12M\\
            & \textbf{Mistral-7b-v0.1} &  264 & 20 & 11 & 15 & 4 & 315 & 1.39M & 500 & 11 & 8 & 94 & 20 & 794 & 2.85M \\
            & \textbf{CodeLLAMA-7b} & 248 & 20 & 8 & 40 & 6 & 485 & 1.7M & 500 & 9 & 182 & 62 & 58 & 743 & 2.8M\\
            & \textbf{CodeLLAMA-13b} & 28 & 20 & 1 & 1 & 1 & 80 & 185K & 32 & 20 & 1 & 0 &  0 & 92 & 248K\\
            & \textbf{GPT-3.5} & 24 & 20 & 0 & 1 & 2& 8& 88K& 37 & 20 & 3 & 5 &3& 12 & 165K\\
            & \textbf{GPT-4} & 25 & 20 & 0 & 0 & 4 & 15 & 87K & 20 & 20 &0&0&0&14&93K\\
	    
		\bottomrule
	\end{tabular}
\end{table*}

==> tables/question_quality.tex <==
\begin{table}[t]
  \caption{The number of Valid question for benchmarks generated by {\sysName} for 20 dialogues, with and without the entity representation module, and the number of skipped nodes to reach our target for different KGs.}
  \label{tab:quality}
  \begin{tabular}{ccc}
    \toprule
     & \textbf{{\sysName}} & \textbf{No Label} \\
    \midrule
    \textbf{DBLP-valid} & 52/81 & 63/87 \\
    \textbf{YAGO-valid} & 77/77 & 71/75 \\
    \textbf{DBpedia-valid} & 94/ 103& 93/97\\
    \midrule
    \textbf{DBLP-skip} & 3 & 7 \\
    \textbf{YAGO-skip} & 15 & 195 \\
    \textbf{DBpedia-skip} & 1 & 88 \\
  \bottomrule
    \end{tabular}
\end{table}

==> tables/subgraph_vs_summarized.tex <==
\begin{table*}[t]
\vspace*{-2ex}
  \caption{Cost comparison between the subgraph and summarized approaches in terms of the number of tokens needed to generate benchmarks, percentage of correct generated SPARQL queries, and the average time taken in seconds to generate one dialogue for a benchmark of 20 dialogues.}
  \vspace*{-3ex}
  \label{tab:comp}
  \begin{tabular}{cccccccc}
    \toprule
      & & \multicolumn{2}{c}{\textbf{DBLP}} & \multicolumn{2}{c}{\textbf{YAGO}} & \multicolumn{2}{c}{\textbf{DBpedia}} \\
     \midrule
     &   & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} & \textbf{Subgraph} & \textbf{{\sysName}} \\
    \midrule
    \multirow{4}{*}{\textbf{Cost}}
    & \textbf{Average} & 3090.9 & 2733.7 & 3153.8 & 2304.4 & 3438.15 & 2517.65 \\
    & \textbf{Minimum} & 1779 & 1910 & 1675 & 1362 & 1868 & 1808\\
    & \textbf{Maximum} & 5970 & 7104 & 9247 & 3397 & 10198 & 4179 \\
    & \textbf{Total} & 61818 & 54674 & 63076 & 46088 & 68763 & 50353\\
     \midrule
     \multirow{4}{*}{\textbf{SPARQL}}
     &\textbf{Correct} & 68 & 90 & 73 & 86 & 79 & 94\\
    &\textbf{Incorrect} & 14 & 6 & 9 & 5 & 18 & 5\\
    &\textbf{Correct \%} & 82.9\% & 93.8\% & 89.0\% & 94.5\% & 81.4\% & 94.9\%\\
    \midrule
    &\textbf{Time (Sec)} & 13.57 & 19.59 & 11.85 & 14.02 & 16.75 & 11.12\\
  \bottomrule
\end{tabular}
\end{table*}



==> tables/time.tex <==
% refer data at /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/subgraph/*
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/results/may12/dbpedia/original for dbpedia
% /dev/data/benchmark_generation/Chatbot-Resources/benchmark/gpt3.5_triple_update for yago and dblp - chatty-gen

\begin{table}[t]
  \caption{Comparison between {\sysName} and the subgraph approach with respect to the average time taken to generate the dialogue with all of its components KG. The times are in seconds}
  \label{tab:time}
  \begin{tabular}{ccc}
    \toprule
    \textbf{KG} & \textbf{Subgraph} & \textbf{{\sysName}} \\
    \midrule
    \textbf{DBLP} & 13.57 & 19.59\\
    \textbf{YAGO} & 11.85 & 14.02\\
    \textbf{DBpedia} & 16.75 & 11.12 \\
  \bottomrule
\end{tabular}
\end{table}


%% old table

% \begin{table}[t]
%   \caption{Comparison between {\sysName} and the subgraph approach with respect to the average time taken to generate the dialogue with all of its components KG. The times are in seconds}
%   \label{tab:time}
%   \begin{tabular}{ccc}
%     \toprule
%     \textbf{KG} & \textbf{Subgraph} & \textbf{{\sysName}} \\
%     \midrule
%     \textbf{DBLP} & 13.9 & 43.4\\
%     \textbf{YAGO} & 44.6 & 13.5\\
%     \textbf{DBpedia} & 12.4 & 21.9 \\
%   \bottomrule
% \end{tabular}
% \end{table}

==> tables/usecase_run2.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{cccc}
    \toprule
        \textbf{Model} &  \textbf{Tie} & \textbf{ConvQuestions} & \textbf{Chatty-Gen} \\
        \midrule
         \textbf{GPT-4o}& 70\% & 25\% & 5\%\\
         \textbf{Multi-LLM-1} & 58\% & 42\% & 0\\
         \textbf{CodeLLAMA-13b} & 25\% & 75\% & 0 \\
         \bottomrule
    \end{tabular}
    \caption{Comparison of question quality between human-generated questions from ConvQuestions and automatically generated questions by {\sysName} using different LLMs. 
    % Each value represents the result of two runs, with ties assigned when results differ. All values are percentages.
    }
    \label{tab:usecase}
\end{table}
% Values
% Gpt-4o:   "Tie": 14, "ConvQuestions": 5, "Chatty_Gen": 1
% Mulit-LLM1: Tie:  11, Chatty-Gen:  0, Conv-Questions:  8
% CodeLLAMA13b: Tie:  5, Chatty-Gen:  0, Conv-Questions:  15

==> tables/usecase_run3.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{cccc}
    \toprule
        \textbf{Model} &  \textbf{Tie} & \textbf{ConvQuestions} & \textbf{Chatty-Gen} \\
        \midrule
         \textbf{GPT-4o}& 70\% & 25\% & 5\%\\
         % \textbf{Multi-LLM-1} & 58\% & 42\% & 0\\
         \textbf{Multi-LLM-1} & 80\% & 15\% & 5\%\\
         % \textbf{CodeLLAMA-13b} & 20\% & 80\% & 0 \\
         \bottomrule
    \end{tabular}
    \caption{Comparison of question quality between human-generated questions from ConvQuestions and automatically generated questions by {\sysName} using different LLMs. 
    % Each value represents the result of two runs, with ties assigned when results differ. All values are percentages.
    }
    \label{tab:usecase}
\end{table}
% Values
% Gpt-4o:   "Tie": 14, "ConvQuestions": 5, "Chatty_Gen": 1
% Mulit-LLM1: Tie:  11, Chatty-Gen:  0, Conv-Questions:  8
% Multi-LLM1 - 7q: Tie:  16, Chatty-Gen:  1, Conv-Questions:  3
% CodeLLAMA13b: Tie:  4, Chatty-Gen:  0, Conv-Questions:  16
